SoK: Kicking CAN Down the Road. Systematizing CAN Security Knowledge

For decades, the Controller Area Network (CAN) has served as the primary in-vehicle bus (IVB), extending its use to many non-vehicular systems. In recent years, CAN security has been intensively scrutinized, yielding extensive research literature. Despite its wealth, the literature lacks structured systematization, complicating efforts to assess and compare attack severity, defense efficacy, security gaps, and root causes. This leaves many defenders uncertain about the relevance of specific attacks or defenses to their systems, and even whether CAN's security problems are truly CAN-specific. As newer IVBs emerge, this matters beyond CAN: if CAN's root causes are not CAN-specific, replacing CAN may only move its problems to a new standard. In this paper, we systematize CAN security knowledge, presenting a comprehensive taxonomy and assessment models of attackers, attacks, and defenses. We identify replicable attacks and defense gaps, and investigate their root causes to determine their exclusivity to the CAN standard. We then investigate whether those root causes appear in three emerging IVBs and assess their effectiveness in solving fundamental CAN security problems. Our findings challenge common perceptions: CAN is more securable than perceived, most of its insecurity root causes are shared across IVBs, and merely adopting newer IVB technology does not solve persistent security problems. We conclude by suggesting that securing future in-vehicle communication requires addressing shared root causes, and we propose four research directions with the most promising potential.

==> LLMs.tex <==
\section{LLM Usage Considerations}

LLMs were only used for grammar, punctuation, and redundancy checking purposes in this manuscript after having been originally written by the authors. All outputs were inspected by the authors to ensure accuracy and originality.

==> Tables/AttackRootCause.tex <==
\begin{table*}[t]
\caption{Root causes for CAN attacks.} 
\label{tbl:attack_root_cause}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{|c||c|c|c|c|c|c|c|c|}
        \hline
      %& R1: Attacker Access      & R2: Shared Media        & R3: Exploitable Priority  & R4: Error Handling        & R5: Layer-II            & R6: Vulnerable Higher-Layer & R7: Physical Layer       & DR1: Cryptography        & DR2: Costly Attacker Signal & DR3: Difficult Environment \\
      %& to Network (I)           & Properties (I)          & System (I)                & Properties (IU)           & Rule Violation          & Protocols                   & Properties (IU)          & Challenges  (I)             & Filtering and Disabling (I)     & Understanding              \\
& $\mathcal{R}$1 (I) & $\mathcal{R}$2 & $\mathcal{R}3$ (I) & $\mathcal{R}$4 (I) & $\mathcal{R}$5 (IU) & $\mathcal{R}$6 & $\mathcal{R}$7 & $\mathcal{R}$8 (IU)  \\
    \hline\hline
Communication surveillance (I) &\checkmark & &\checkmark & & & & & \\
\hline
\cellcolor{gray!25}Privacy leakage (I) &\checkmark & &\checkmark & & & & & \\
\hline
\cellcolor{gray!25}Sensitive information sniffing &\checkmark & &\checkmark & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Information and firmware dump &\checkmark & & & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Memory leakage &\checkmark & & & & & &\checkmark & \\
\hline
Error-based network reconnaissance (IU) &\checkmark & &\checkmark &\checkmark &\checkmark & & & \\
\hline
\cellcolor{gray!25}Skew network mapping (I) &\checkmark & &\checkmark & & & & & \\
\hline
\cellcolor{gray!25}Signal and hardware profiling &\checkmark &\checkmark &\checkmark & & & & & \\
\hline
\cellcolor{gray!25}Topology intelligence &\checkmark &\checkmark &\checkmark & & & & & \\
\hline
\cellcolor{gray!25}Electromagnetic emission &\checkmark &\checkmark & & & & & & \\
\hline
Fake data fabrication (I) &\checkmark & & & & & & & \\
\hline
\cellcolor{gray!25}Memory and firmware manipulation &\checkmark & & & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Bypassing diagnostic authentication &\checkmark & & & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Session-based buffer overflow &\checkmark & & & & & &\checkmark & \\
\hline
Impersonation and replay (I) &\checkmark & &\checkmark & & & & & \\
\hline
\cellcolor{gray!25}Poly-semantic frames (U) &\checkmark & &\checkmark & & &\checkmark & &\checkmark \\
\hline
\cellcolor{gray!25}Double receive (U) &\checkmark & &\checkmark & &\checkmark &\checkmark & & \\
\hline
Frame hijacking (IU) &\checkmark & &\checkmark &\checkmark &\checkmark & & & \\
\hline
\cellcolor{gray!25}Polyglot frames (U) &\checkmark & & & & &\checkmark & &\checkmark \\
\hline
\cellcolor{gray!25}Frame tampering (U) &\checkmark & &\checkmark & & &\checkmark & &\checkmark \\
\hline
\cellcolor{gray!25}Unorthodox frames (U) &\checkmark & & & &\checkmark &\checkmark & & \\
\hline
Physical fingerprint distortion (IU) &\checkmark & &\checkmark &\checkmark &\checkmark & & & \\
\hline
\cellcolor{gray!25}Physical architecture manipulation &\checkmark &\checkmark & & & & & & \\
\hline
\cellcolor{gray!25}ECU functionality disabling &\checkmark & & & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Request overwhelming &\checkmark & & & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Sybil exhaustion &\checkmark & & & & & &\checkmark & \\
\hline
\cellcolor{gray!25}Synchronization disruption (U) &\checkmark & &\checkmark & & &\checkmark & &\checkmark \\
\hline
Error injection (IU) &\checkmark & &\checkmark &\checkmark &\checkmark & & & \\
\hline
Error state manipulation (IU) &\checkmark & &\checkmark &\checkmark &\checkmark & & & \\
\hline
Bus access denial (I) &\checkmark & &\checkmark &\checkmark & & & & \\
\hline
\cellcolor{gray!25}Signal attenuation (U) &\checkmark & &\checkmark & & &\checkmark & &\checkmark \\
\hline
\cellcolor{gray!25}Vandalism &\checkmark &\checkmark & & & & & & \\
\hline
  \end{tabular}}
\end{table*}


==> Tables/AttackerAbility.tex <==
\begin{table}[t]
\centering
\caption{CAN attacker models.}
\label{tbl:attacker_ability}
\resizebox{\columnwidth}{!}{
\arrayrulecolor{black}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Bus Access Level} & \textbf{Equipment} & \textbf{Layer Dominance}\\
\hline\hline
By-the-Rules & Remote & Generic & Higher Layer \\
\hline
Bit-Banger & Remote & Generic & Controller Layer \\
\hline
Down-to-Earth & Physical & Special & Transwire Layer \\
\hline

\end{tabular}
}
\end{table}

==> Tables/Attacks.backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
Attacker\textbackslash{}Complexity                          & Prevalence                       & Easy                                                                                                                                                                                                        & Intermediate                                                                                                                                                     & Complex                                                                                                                               \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                    & Standard                         & \begin{tabular}[c]{@{}l@{}}Error-Based reconnaissance (C), \\ Impersonation and Replay (I), \\ Frame Hijacking (I), Error State Mnipulation (A), \\ Error Injection (A), Bus access denial (A)\end{tabular} & \cellcolor[HTML]{F1F1F1}\begin{tabular}[c]{@{}l@{}}Communication Surveillance (C), \\ Fake Data Fabrication (I)\end{tabular}                                     & \cellcolor[HTML]{B5B5B5}Physical Fingerprint Spoofing (I)                                                                             \\ \cline{2-5} 
\cellcolor[HTML]{FFFFFF}                                    & \cellcolor[HTML]{FFFFC7}Wide     & \cellcolor[HTML]{FFFFC7}\begin{tabular}[c]{@{}l@{}}Higher-layer Sybil Exhaustion (A), \\ Request Overwhelming (A)\end{tabular}                                                                              & \cellcolor[HTML]{F1F1BD}\begin{tabular}[c]{@{}l@{}}Privacy Leakage (C),  Clock-Skew Mapping(C), \\ ECU Functionality Disabling (A)\end{tabular}                  & \cellcolor[HTML]{C0C095}                                                                                                              \\ \cline{2-5} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}By-the-rules}      & \cellcolor[HTML]{FFFC9E}Specific & \cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}l@{}}Memory Leakage (C), \\ Session Based Buffer Overflow\end{tabular}                                                                                        & \cellcolor[HTML]{F3F097}\begin{tabular}[c]{@{}l@{}}Sensetive Info Sniffing (C),  \\ Bypassing Diagnostic Authentication (I), \\ Clock-skew Spoofing\end{tabular} & \cellcolor[HTML]{AAA868}\begin{tabular}[c]{@{}l@{}}Info and Firmware Dump (C),  \\ memory and Firmware Manipulation (I),\end{tabular} \\ \hline
\rowcolor[HTML]{FFE8CD} 
\cellcolor[HTML]{FFE8CD}                                    & Standard                         & Double Receive (I),                                                                                                                                                                                         & \cellcolor[HTML]{EED7BE}Polyglot Frames (I),                                                                                                                     & \cellcolor[HTML]{C8B6A0}Frame Tampering (I), Signal Attenuation (A)                                                                   \\ \cline{2-5} 
\cellcolor[HTML]{FFE8CD}                                    & \cellcolor[HTML]{FFCE93}Wide     & \cellcolor[HTML]{FFCE93}                                                                                                                                                                                    & \cellcolor[HTML]{EEBF87}Polysemantic Frames (I),                                                                                                                 & \cellcolor[HTML]{C8A274}                                                                                                              \\ \cline{2-5} 
\multirow{-3}{*}{\cellcolor[HTML]{FFE8CD}Bit-banger}        & \cellcolor[HTML]{FE996B}Specific & \cellcolor[HTML]{FE996B}                                                                                                                                                                                    & \cellcolor[HTML]{F39063}                                                                                                                                         & \cellcolor[HTML]{AC6646}                                                                                                              \\ \hline
\rowcolor[HTML]{FFE2E0} 
\cellcolor[HTML]{FFE2E0}                                    & Standard                         &                                                                                                                                                                                                             & \cellcolor[HTML]{F5D9D7}\begin{tabular}[c]{@{}l@{}}Signal and Hardware Profiling (C),  \\ Electromagnetic Emissions (C),\end{tabular}                            & \cellcolor[HTML]{B69F9D}                                                                                                              \\ \cline{2-5} 
\cellcolor[HTML]{FFE2E0}                                    & \cellcolor[HTML]{FFCCC9}Wide     & \cellcolor[HTML]{FFCCC9}                                                                                                                                                                                    & \cellcolor[HTML]{EEBBB8}                                                                                                                                         & \cellcolor[HTML]{BA9290}                                                                                                              \\ \cline{2-5} 
\multirow{-3}{*}{\cellcolor[HTML]{FFE2E0}Down-to-earth (L)} & \cellcolor[HTML]{FD6864}Specific & \cellcolor[HTML]{FD6864}                                                                                                                                                                                    & \cellcolor[HTML]{EE615D}                                                                                                                                         & \cellcolor[HTML]{B04845}                                                                                                              \\ \hline
\rowcolor[HTML]{9A0000} 
Down-to-earth (P)                                           & Standard                         & Physical Architecture Manipulation (I)                                                                                                                                                                      & \cellcolor[HTML]{820000}Location Identification (C),                                                                                                             & \cellcolor[HTML]{430000}                                                                                                              \\ \hline
\end{tabular}
}
\end{table*}

==> Tables/Attacks.old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
Attacker\textbackslash{}Complexity                          & Prevalence                       & Easy                                                                                                                                                                                                        & Intermediate                                                                                                                                                     & Complex                                                                                                                               \\ \hline
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                    & Standard                         & \begin{tabular}[c]{@{}l@{}}Error-Based reconnaissance (C), \\ Impersonation and Replay (I), \\ Frame Hijacking (I), Error State Mnipulation (A), \\ Error Injection (A), Bus access denial (A)\end{tabular} & \cellcolor[HTML]{F1F1F1}\begin{tabular}[c]{@{}l@{}}Communication Surveillance (C), \\ Fake Data Fabrication (I)\end{tabular}                                     & \cellcolor[HTML]{B5B5B5}Physical Fingerprint Spoofing (I)                                                                             \\ \cline{2-5} 
\cellcolor[HTML]{FFFFFF}                                    & \cellcolor[HTML]{FFFFC7}Wide     & \cellcolor[HTML]{FFFFC7}\begin{tabular}[c]{@{}l@{}}Higher-layer Sybil Exhaustion (A), \\ Request Overwhelming (A)\end{tabular}                                                                              & \cellcolor[HTML]{F1F1BD}\begin{tabular}[c]{@{}l@{}}Privacy Leakage (C),  Clock-Skew Mapping(C), \\ ECU Functionality Disabling (A)\end{tabular}                  & \cellcolor[HTML]{C0C095}                                                                                                              \\ \cline{2-5} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}By-the-rules}      & \cellcolor[HTML]{FFFC9E}Specific & \cellcolor[HTML]{FFFC9E}\begin{tabular}[c]{@{}l@{}}Memory Leakage (C), \\ Session Based Buffer Overflow\end{tabular}                                                                                        & \cellcolor[HTML]{F3F097}\begin{tabular}[c]{@{}l@{}}Sensetive Info Sniffing (C),  \\ Bypassing Diagnostic Authentication (I), \\ Clock-skew Spoofing\end{tabular} & \cellcolor[HTML]{AAA868}\begin{tabular}[c]{@{}l@{}}Info and Firmware Dump (C),  \\ memory and Firmware Manipulation (I),\end{tabular} \\ \hline
\rowcolor[HTML]{FFE8CD} 
\cellcolor[HTML]{FFE8CD}                                    & Standard                         & Double Receive (I),                                                                                                                                                                                         & \cellcolor[HTML]{EED7BE}Polyglot Frames (I),                                                                                                                     & \cellcolor[HTML]{C8B6A0}Frame Tampering (I), Signal Attenuation (A)                                                                   \\ \cline{2-5} 
\cellcolor[HTML]{FFE8CD}                                    & \cellcolor[HTML]{FFCE93}Wide     & \cellcolor[HTML]{FFCE93}                                                                                                                                                                                    & \cellcolor[HTML]{EEBF87}Polysemantic Frames (I),                                                                                                                 & \cellcolor[HTML]{C8A274}                                                                                                              \\ \cline{2-5} 
\multirow{-3}{*}{\cellcolor[HTML]{FFE8CD}Bit-banger}        & \cellcolor[HTML]{FE996B}Specific & \cellcolor[HTML]{FE996B}                                                                                                                                                                                    & \cellcolor[HTML]{F39063}                                                                                                                                         & \cellcolor[HTML]{AC6646}                                                                                                              \\ \hline
\rowcolor[HTML]{FFE2E0} 
\cellcolor[HTML]{FFE2E0}                                    & Standard                         &                                                                                                                                                                                                             & \cellcolor[HTML]{F5D9D7}\begin{tabular}[c]{@{}l@{}}Signal and Hardware Profiling (C),  \\ Electromagnetic Emissions (C),\end{tabular}                            & \cellcolor[HTML]{B69F9D}                                                                                                              \\ \cline{2-5} 
\cellcolor[HTML]{FFE2E0}                                    & \cellcolor[HTML]{FFCCC9}Wide     & \cellcolor[HTML]{FFCCC9}                                                                                                                                                                                    & \cellcolor[HTML]{EEBBB8}                                                                                                                                         & \cellcolor[HTML]{BA9290}                                                                                                              \\ \cline{2-5} 
\multirow{-3}{*}{\cellcolor[HTML]{FFE2E0}Down-to-earth (L)} & \cellcolor[HTML]{FD6864}Specific & \cellcolor[HTML]{FD6864}                                                                                                                                                                                    & \cellcolor[HTML]{EE615D}                                                                                                                                         & \cellcolor[HTML]{B04845}                                                                                                              \\ \hline
\rowcolor[HTML]{9A0000} 
Down-to-earth (P)                                           & Standard                         & Physical Architecture Manipulation (I)                                                                                                                                                                      & \cellcolor[HTML]{820000}Location Identification (C),                                                                                                             & \cellcolor[HTML]{430000}                                                                                                              \\ \hline
\end{tabular}
}
\end{table*}

==> Tables/Attacks.old2.tex <==
\begin{table*}[]
\centering
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|ll|l|l|l|l|} 
\hline
\multicolumn{4}{|c|}{\multirow{2}{*}{Attacker Model}}                                                                                                                                                                                        & \multicolumn{1}{c|}{\multirow{2}{*}{Prevlance}} & \multicolumn{1}{l}{}                                                                                                                                                                                                                                                                                                                                                                        & \multicolumn{1}{l}{Exploit Complexity}                                                                                                                                                                             &                                                                                                                   \\ 
\cline{6-8}
\multicolumn{4}{|c|}{}                                                                                                                                                                                                                       & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{Easy ($\Circle$)}                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{1}{c|}{Intermediate ($\LEFTcircle$)}                                                                                                                                                                & \multicolumn{1}{c|}{Complex ($\CIRCLE$)}                                                                        \\ 
\hline
{\cellcolor[rgb]{0.749,0.749,0.749}}                                   & {\cellcolor[rgb]{0.831,0.831,0.831}} & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.914,0.914,0.914}}} & \multirow{3}{*}{By-the-rules}                                    & Standard ($\CIRCLE$)                          &                                                                                                                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}\underline{Communication Surveillance (C),}\\\underline{Fake Data Fabrication (I)}\end{tabular}                                                                                                 &                                                                                                                   \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~>{\arrayrulecolor{black}}----|}
{\cellcolor[rgb]{0.749,0.749,0.749}}                                   & {\cellcolor[rgb]{0.831,0.831,0.831}} & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.914,0.914,0.914}}} &                                                                  & Wide ($\LEFTcircle$)                          & \begin{tabular}[c]{@{}l@{}}\underline{\textbf{Higher-Layer Sybil Exhaustion (A),}}\\\underline{\textbf{Request Overwhelming (A)}}\end{tabular}                                                                                                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}\underline{Privacy Leakage (C),}\\\underline{ECU Functionality Disabling (A)}\end{tabular}                                                                                                      &                                                                                                                   \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~>{\arrayrulecolor{black}}----|}
{\cellcolor[rgb]{0.749,0.749,0.749}}                                   & {\cellcolor[rgb]{0.831,0.831,0.831}} & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.914,0.914,0.914}}} &                                                                  & Specific ($\Circle$)                          & \begin{tabular}[c]{@{}l@{}}\underline{\textbf{Memory Leakage (C),}}\\\underline{\textbf{Session-Based Buffer Overflow (I)}}\end{tabular}                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}\underline{Memory Leakage (C),}\\\underline{Bypassing Diagnostic Authentication (I)}\end{tabular}                                                                                               & \begin{tabular}[c]{@{}l@{}}Information and Firmware Dump (C),\\Memory and Firmware Manipulation (I)\end{tabular}  \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}->{\arrayrulecolor{black}}-----|}
\rowcolor[rgb]{0.914,0.914,0.914} {\cellcolor[rgb]{0.749,0.749,0.749}} & {\cellcolor[rgb]{0.831,0.831,0.831}} &                                                           & {\cellcolor[rgb]{0.914,0.914,0.914}}                             & Standard ($\CIRCLE$)                          & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.914,0.914,0.914}}l@{}}\underline{\textbf{Error-based Reconnaissance (C),}}\\\underline{\textbf{Impersonation and Replay (I),}}\\\underline{\textbf{Double Receive (I),}}\\\underline{\textbf{Unorthodox Frames (I),}}\\\underline{\textbf{Error State Manipulation (A),}}\\\underline{\textbf{Error-Injection (A),}}\\\underline{\textbf{Bus Access Denial (A)}}\end{tabular} &                                                                                                                                                                                                                    &                                                                                                                   \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-->{\arrayrulecolor{black}}----|}
\rowcolor[rgb]{0.914,0.914,0.914} {\cellcolor[rgb]{0.749,0.749,0.749}} & {\cellcolor[rgb]{0.831,0.831,0.831}} &                                                           & {\cellcolor[rgb]{0.914,0.914,0.914}}                             & Wide ($\LEFTcircle$)                          &                                                                                                                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.914,0.914,0.914}}l@{}}\underline{Clock-Skew Network Mapping (C),}\\\underline{Poly-semantic Frames (I),}\\\underline{Frame Tampering (I),}\\\underline{Polyglot Frames (I)}\end{tabular} &                                                                                                                   \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-->{\arrayrulecolor{black}}----|}
\rowcolor[rgb]{0.914,0.914,0.914} {\cellcolor[rgb]{0.749,0.749,0.749}} & {\cellcolor[rgb]{0.831,0.831,0.831}} &                                                           & \multirow{-3}{*}{{\cellcolor[rgb]{0.914,0.914,0.914}}Bit-banger} & Specific ($\Circle$)                          &                                                                                                                                                                                                                                                                                                                                                                                             & \underline{Clock-Skew Spoofing (I)}                                                                                                                                                                                    &                                                                                                                   \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor{black}}------|}
\rowcolor[rgb]{0.831,0.831,0.831} {\cellcolor[rgb]{0.749,0.749,0.749}} & \multicolumn{1}{l}{}                 &                                                           & Down-to-earth (L)                                                & Standard ($\CIRCLE$)                          & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.831,0.831,0.831}}l@{}}\underline{\textbf{Physical-Fingerprint Distortion (I),}}\\\underline{\textbf{Physical Architecture Manipulation (I),}}\\\underline{\textbf{Synchronization Disruption (A)}}\end{tabular}                                                                                                                                               & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.831,0.831,0.831}}l@{}}\underline{Signal and Hardware Profiling (C),}\\\underline{Location Identification (C),}\\\underline{Electromagnetic Emissions (C)}\end{tabular}               & Signal Attenuation (A)                                                                                            \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.749,0.749,0.749}}->{\arrayrulecolor{black}}-------|}
\rowcolor[rgb]{0.749,0.749,0.749} \multicolumn{1}{|l}{}                & \multicolumn{1}{l}{}                 &                                                           & Down-to-earth (P)                                                & Standard ($\CIRCLE$)                          &                                                                                                                                                                                                                                                                                                                                                                                             &                                                                                                                                                                                                                    & Physical Vandalism (A)                                                                                            \\
\hline
\end{tabular}
}
\end{table*}

==> Tables/Attacks.tex <==
\begin{table}[]
\centering
\arrayrulecolor{black}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{|l|l|c|c|c|l|} 
\hline
\multicolumn{3}{|c|}{Attacker Model}                                                                                                                                                                                                                                                                                                                                     & Prevlance                                                                  & Exploit Complexity                                & \multicolumn{1}{c|}{Attack}                                                                                                                                                                                                               \\ 
\hline
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                 & \multirow{11}{*}{\begin{sideways}By-the-rules ($\CIRCLE$)\end{sideways}}                                                                                                                             & \multirow{2}{*}{Standard ($\CIRCLE$)}                                      & Easy ($\Circle$)                                  & \begin{tabular}[c]{@{}l@{}}Error-Based Reconnaissance (C)\\Impersonation and Replay (I)\\Frame Hijacking (I)\\Physical-Fingerprint Distortion (I)\\Error State Manipulation (A)\\Error-Injection (A)\\Bus Access Denial (A)\end{tabular}  \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~~>{\arrayrulecolor{black}}--|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                 &                                                                                                                                                                                                     &                                                                            & \multicolumn{1}{l|}{Intermediate ($\LEFTcircle$)} & \begin{tabular}[c]{@{}l@{}}Communication Surveillance (C)\\Fake Data Fabrication (I)\end{tabular}                                                                                                                                         \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~>{\arrayrulecolor{black}}---|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                 &                                                                                                                                                                                                     & \multirow{2}{*}{Wide ($\LEFTcircle$)}                                      & Easy ($\Circle$)                                  & \begin{tabular}[c]{@{}l@{}}Higher-Layer Sybil Exhaustion (A)\\Request Overwhelming (A)\end{tabular}                                                                                                                                       \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~~>{\arrayrulecolor{black}}--|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                 &                                                                                                                                                                                                     &                                                                            & Intermediate ($\LEFTcircle$)                      & \begin{tabular}[c]{@{}l@{}}Privacy Leakage (C)\\Clock-Skew Network Mapping (C)\\ECU Functionality Disabling (A)\end{tabular}                                                                                                              \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~>{\arrayrulecolor{black}}---|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                 &                                                                                                                                                                                                     & \multirow{3}{*}{Specific ($\Circle$)}                                      & Easy ($\Circle$)                                  & \begin{tabular}[c]{@{}l@{}}Memory Leakage (C)\\Session-Based Buffer Overflow (I)\end{tabular}                                                                                                                                             \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~~>{\arrayrulecolor{black}}--|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                 &                                                                                                                                                                                                     &                                                                            & Intermediate ($\LEFTcircle$)                      & \begin{tabular}[c]{@{}l@{}}Sensitive Information Sniffing (C)\\Bypassing Diagnostic Authentication (I)\end{tabular}                                                                                                                       \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-~~>{\arrayrulecolor{black}}--|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & \multirow{-7}{*}{{\cellcolor[rgb]{0.914,0.914,0.914}}}                               &                                                                                                                                                                                                     &                                                                            & Complex ($\CIRCLE$)                               & \begin{tabular}[c]{@{}l@{}}Information and Firmware Dump (C)\\Memory and Firmware Manipulation (I)\end{tabular}                                                                                                                           \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}->{\arrayrulecolor{black}}----|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & \multicolumn{1}{l}{{\cellcolor[rgb]{0.914,0.914,0.914}}}                             & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                                                                                                                                & {\cellcolor[rgb]{0.914,0.914,0.914}}                                       & Easy ($\Circle$)                                  & \begin{tabular}[c]{@{}l@{}}Double Receive (I)\\Unorthodox Frames (I)\\Synchronization Disruption (A)\end{tabular}                                                                                                                         \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}--->{\arrayrulecolor{black}}--|}
{\cellcolor[rgb]{0.831,0.831,0.831}}                                        & \multicolumn{1}{l}{{\cellcolor[rgb]{0.914,0.914,0.914}}}                             & {\cellcolor[rgb]{0.914,0.914,0.914}}                                                                                                                                                                & \multirow{-2}{*}{{\cellcolor[rgb]{0.914,0.914,0.914}}Standard ($\CIRCLE$)} & \multicolumn{1}{l|}{Complex ($\CIRCLE$)}          & \begin{tabular}[c]{@{}l@{}}Signal Attenuation (A)\\Physical Vandalism (A)\end{tabular}                                                                                                                                                    \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor[rgb]{0.914,0.914,0.914}}-->{\arrayrulecolor{black}}---|}
\multirow{-10}{*}{{\cellcolor[rgb]{0.831,0.831,0.831}}}                     & \multicolumn{1}{l}{\multirow{-3}{*}{{\cellcolor[rgb]{0.914,0.914,0.914}}}}           & \multirow{-7}{*}{{\cellcolor[rgb]{0.914,0.914,0.914}}\begin{sideways}Bit-banger($\LEFTcircle$) \end{sideways}}                                                                                      & {\cellcolor[rgb]{0.914,0.914,0.914}}Wide ($\LEFTcircle$)                   & \multicolumn{1}{l|}{Intermediate ($\LEFTcircle$)} & \begin{tabular}[c]{@{}l@{}}Poly-semantic Frames (I)\\Frame Tampering (I)\\Polyglot Frames (I)\end{tabular}                                                                                                                                \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}->{\arrayrulecolor{black}}-----|}
\multicolumn{1}{|l}{{\cellcolor[rgb]{0.831,0.831,0.831}}}                   & \multicolumn{1}{l}{{\cellcolor[rgb]{0.831,0.831,0.831}}}                             & {\cellcolor[rgb]{0.831,0.831,0.831}}                                                                                                                                                                & {\cellcolor[rgb]{0.831,0.831,0.831}}                                       & Easy ($\Circle$)                                  & Physical Architecture Manipulation (I)                                                                                                                                                                                                    \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.831,0.831,0.831}}---->{\arrayrulecolor{black}}--|}
\multicolumn{1}{|l}{\multirow{-2}{*}{{\cellcolor[rgb]{0.831,0.831,0.831}}}} & \multicolumn{1}{l}{\multirow{-2}{*}{{\cellcolor[rgb]{0.831,0.831,0.831}}\rotcell{}}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.831,0.831,0.831}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.831,0.831,0.831}}c@{}}Down-\\to-earth($\Circle$)\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.831,0.831,0.831}}Standard ($\CIRCLE$)} & Intermediate ($\LEFTcircle$)                      & \begin{tabular}[c]{@{}l@{}}Clock-Skew Network Mapping (C)\\Topology Intelligence (C)\\Electromagnetic Emissions (C)\end{tabular}                                                                                                          \\
\hline
\end{tabular}
}
\end{table}

==> Tables/Attacks_Only.tex <==
\begin{table*}
\centering
\begin{tabular}{ccc}
Target: Higher                      & Target: Controller                  & Target: Transwire                    \\
Communication Surveillance          & Error Based Reconnaissance          & Signal and Hardware Profiling        \\
Privacy Leakage                     & Clock-Skew Network Mapping          & Topology Intelligence                \\
Sensitivwe Information Sniffing     & Impersonation and Replay            & Electromagnetic Emissions            \\
Memiory Leakage                     & Poly-Semantic Frames                & Signal Attenuation                   \\
Information and Firmware Dump       & Frame Tampering                     & Physical Vandalism                   \\
Fake Data Fabrication               & Double Receive                      & Physical-Fingerprint \`{}distortion  \\
Memory and Firmware Manipulation    & Polyglot Frames                     & Physical Architecture Manipulation   \\
Bypassing Diagnostic Authentication & Unorthodox Frames                   &                                      \\
Session-Based Buffer Overflow       & Frame Hijacking                     &                                      \\
ECU Function Disabling              & Physical-Fingerprint \`{}distortion &                                      \\
Higher-Level Sybil Exhaustion       & Physical Architecture Manipulation  &                                      \\
Request Overwhelming                &                                     &                                     
\end{tabular}
\end{table*}

==> Tables/Attacks_Taxonomized.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\definecolor{MonaLisa}{rgb}{1,0.592,0.592}
\definecolor{Melrose}{rgb}{0.741,0.741,1}
\definecolor{Silver}{rgb}{0.752,0.752,0.752}
\begin{table}
\centering
\caption{Attacks Taxonomized}
\label{tbl:CANRC}
\resizebox*{\columnwidth}{!}{
\begin{tblr}{
  column{3} = {c},
  cell{1}{2} = {c},
  cell{1}{4} = {c},
  cell{2}{2} = {MonaLisa,c},
  cell{2}{3} = {MonaLisa},
  cell{2}{4} = {MonaLisa,c},
  cell{3}{2} = {MonaLisa,c},
  cell{3}{3} = {MonaLisa},
  cell{3}{4} = {MonaLisa,c},
  cell{4}{2} = {MonaLisa,c},
  cell{4}{3} = {Melrose},
  cell{4}{4} = {MonaLisa,c},
  cell{5}{2} = {MonaLisa,c},
  cell{5}{3} = {Melrose},
  cell{5}{4} = {Melrose,c},
  cell{6}{2} = {MonaLisa,c},
  cell{6}{3} = {Melrose},
  cell{6}{4} = {Melrose,c},
  cell{7}{2} = {Melrose,c},
  cell{7}{3} = {Melrose},
  cell{7}{4} = {Silver,c},
  cell{8}{2} = {Melrose,c},
  cell{8}{3} = {Melrose},
  cell{8}{4} = {Silver,c},
  cell{9}{2} = {Melrose,c},
  cell{9}{3} = {Melrose},
  cell{9}{4} = {Silver,c},
  cell{10}{2} = {Melrose,c},
  cell{10}{3} = {Melrose},
  cell{10}{4} = {Silver,c},
  cell{11}{2} = {Silver,c},
  cell{11}{3} = {Silver},
  cell{11}{4} = {Silver,c},
  cell{12}{2} = {Silver,c},
  cell{12}{3} = {Silver},
  cell{12}{4} = {Silver,c},
  cell{13}{2} = {Silver,c},
  cell{13}{3} = {Silver},
  cell{13}{4} = {Silver,c},
  cell{14}{2} = {Silver},
  cell{14}{3} = {Silver},
  cell{14}{4} = {Silver},
}
Security Element & Target: Higher                      & Target: Controller         & Target: Transwire                   \\
Confidentiality  & Communication Surveillance          & Error Based Reconnaissance & Signal and Hardware Profiling       \\
                 & Privacy Leakage                     & Clock-Skew Network Mapping & Topology Intelligence               \\
                 & Sensitive Information Sniffing     & Impersonation and Replay   & Electromagnetic Emissions           \\
                 & Memory Leakage                     & Poly-Semantic Frames       & Physical-Fingerprint Distortion~   \\
                 & Information and Firmware Dump       & Frame Tampering            & Physical Architecture Manipulation~ \\
Integrity        & Fake Data Fabrication               & Double Receive             & Signal Attenuation                  \\
                 & Memory and Firmware Manipulation    & Polyglot Frames            & Physical Vandalism                  \\
                 & Bypassing Diagnostic Authentication & Unorthodox Frames          &                                     \\
                 & Session-Based Buffer Overflow       & Frame Hijacking            &                                     \\
Availability     & ECU Function Disabling              & Synch Disruption           &                                     \\
                 & Higher-Level Sybil Exhaustion       & Error Injection            &                                     \\
                 & Request Overwhelming                & Error State Manipulation   &                                     \\
                 &                                     & Bus Access Denial          &                                     
\end{tblr}
}
\end{table}

==> Tables/CANAlts.tex <==
% \usepackage{rotating}
% \usepackage{tabularray}
\begin{table}[h]
\label{tbl:altperf}
\centering
\caption{Emerging IVBs and their features}
\resizebox{\columnwidth}{!}{
\begin{tblr}{
  column{odd} = {c},
  column{2} = {c},
  column{4} = {c},
  column{8} = {c},
  column{10} = {c},
  column{12} = {c},
  hlines,
  vlines,
}
           & \begin{sideways}Real-Time\end{sideways} & \begin{sideways}Atomic-Broadcast\end{sideways} & \begin{sideways}Max Baudrate\end{sideways} & \begin{sideways}Equipment Cost\end{sideways}         & \begin{sideways}Wiring Cost\end{sideways} & \begin{sideways}Flexible Topology\end{sideways} & \begin{sideways}Longest Payload\end{sideways} & \begin{sideways}Error-Handling\end{sideways} & \begin{sideways}Bus Master\end{sideways} & \begin{sideways}Zonal Compatible\end{sideways} & \begin{sideways}Validity\end{sideways} \\
CAN        & $\checkmark$           & $\checkmark$                  & 1 Mb/s                                     & $\downarrow$                        & $\downarrow$             & $\LEFTcircle$                  & 64 b                                          & $\CIRCLE$                   & X                                        & $\Circle$                     & $\CIRCLE$                               \\
CANFD      & $\checkmark$           & $\checkmark$                  & 8* Mb/s                                    & $\downarrow$                        & $\downarrow$             & $\LEFTcircle$                  & 64 B                                          & $\CIRCLE$                   & X                                        & $\Circle$                     & $\CIRCLE$                               \\
CANXL      & $\checkmark$           & $\checkmark$                  & 20* Mb/s                                   & $\downarrow$                        & $\downarrow$             & $\CIRCLE$                      & 2048 B                                        & $\CIRCLE$                   & X                                        & $\CIRCLE$                     & $\Circle$                          \\
10BASE-T1S & $\checkmark$           & X                                              & 10 Mb/s                                    & $\uparrow\downarrow$ & $\downarrow$             & $\LEFTcircle$                  & 1520 B                                        & $\LEFTcircle$               & $\checkmark$            & $\CIRCLE$                     & $\LEFTcircle$                            
\end{tblr}
}
\end{table}


%* Means that it is the data section only
%validity: CAN and FD are widely used. CANXL is not used, only standardized. 10base has some controllers and has been probably been used in some limited use cases but I am not sure. I think you may need to add electromagnetic interference. You may need to remove schedulability if you made it a standard for exclusion

==> Tables/CANAlts_Sec.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\begin{table}[h]
\caption{Change this. Make it  RC1, 2, etc and then list what each attack checks, then what each other bus checks. In text say what is highly likely}
\label{tbl:altsec}
\centering
\resizebox{\columnwidth}{!}{
% \usepackage{rotating}
% \usepackage{color}

\centering
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c|c|c|} 
\hline
           & \multicolumn{5}{c||}{Insecurity Root-Cause}                                                                                                                                                                                                                                                  & \multicolumn{8}{c|}{Attack}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ 
\hline
           & \begin{sideways}Native Confidentiality\end{sideways} & \begin{sideways}Native Authentication\end{sideways} & \begin{sideways}Priority Assignment\end{sideways} & \begin{sideways}Transmission Control\end{sideways} & \begin{sideways}Obs. State Behavior\end{sideways} & \begin{sideways}Com. Surveillance\end{sideways}                                           & \begin{sideways}Error Injection\end{sideways}                                            & \begin{sideways}State Manipulation\end{sideways}                                   & \begin{sideways}Bus Reconnaissance\end{sideways}                                         & \begin{sideways}Impersonation \& Rep.\end{sideways}                                   & \begin{sideways}Data Fabrication\end{sideways}                                           & \begin{sideways}Frame Hijacking\end{sideways}                                            & \begin{sideways}Flooding\end{sideways}                                                    \\ 
\hline
CAN        & $\Circle$                           & $\Circle$                          & $\CIRCLE$                               & $\CIRCLE$                               & $\CIRCLE$                                & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}} & \textcolor[rgb]{0.047,0.051,0.055}{\textcolor{black}{$\checkmark$}}  \\ 
\hline
CANFD      & $\Circle$                           & $\Circle$                          & $\CIRCLE$                               & $\CIRCLE$                               & $\CIRCLE$                                & $\uparrow$                                                            & $\uparrow$                                                            & $\uparrow$                                                            & $\uparrow$                                                            & $\uparrow$                                                            & $\checkmark$                                                        & $\uparrow$                                                            & $\uparrow$                                                             \\ 
\hline
CANXL      & $\LEFTcircle$                           & $\LEFTcircle$                          & $\CIRCLE$                               & $\CIRCLE$                               & $\uparrow\downarrow$                                                         & $\uparrow\downarrow$                                      & $\uparrow$                                                            & $\uparrow\downarrow$                                      & $\uparrow\downarrow$                                      & $\uparrow\downarrow$                                      & $\checkmark$                                                        & $\downarrow$                                                                & $\uparrow$                                                             \\ 
\hline
10Base-T1S & $\LEFTcircle$                           & $\LEFTcircle$                          & $\CIRCLE$                               & $\LEFTcircle$                               & --                                                        & $\uparrow\downarrow$                                      & $\uparrow\downarrow$                                      & --                                                                                       & $\checkmark$                                                        & $\uparrow\downarrow$                                      & $\checkmark$                                                        & $\downarrow$                                                                & $\uparrow$                                                             \\
\hline
\end{tabular}
}
\end{table}

==> Tables/CANsec.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}%[h]%[th!]
\centering
\caption{Formally analyzing IVB security protocols.}
\label{tbl:CANsec}
\resizebox{\columnwidth}{!}{
\arrayrulecolor{black}
\begin{tabular}{|c|c||c|c|c|}
\hline
\multicolumn{2}{|c||}{} & $\mathcal{P}_{a}: \mathtt{Authenticity}$ & $\mathcal{P}_{f}: \mathtt{Freshness}$ & $\mathcal{P}_{c}: \mathtt{Confidentiality}$ \\
\hline\hline
CANsec& E & \checkmark & \checkmark & \checkmark\\
\cline{2-5}
(w. MKA/IKA) & I & X & X & X\\
\hline
CANsec+& E & \checkmark & \checkmark & \checkmark\\
\cline{2-5}
(w. Revocation) & I & \checkmark & \checkmark & \checkmark\\
\hline
MACsec& E & \checkmark & \checkmark & \checkmark\\
\cline{2-5}
(w. MKA) & I & X & X & X\\
\hline
MACsec+& E & \checkmark & \checkmark & \checkmark\\
\cline{2-5}
(w. Revocation) & I & \checkmark & \checkmark &\checkmark\\
\hline

\end{tabular}
}
\end{table}

==> Tables/CANsec2.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}%[h]%[th!]
\centering
\caption{Formally verifying security properties for CANsec}
\label{tbl:CANsec}
\resizebox{\columnwidth}{!}{
\arrayrulecolor{black}
\begin{tabular}{|l||cc|cc||cc|} 
\hline
\multicolumn{1}{|c||}{\multirow{2}{*}{Property $\mathcal{P}$}}                       & \multicolumn{2}{c|}{CANsec}          & \multicolumn{2}{c||}{CANsec+}        & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.854,0.854,0.854}}CKA}                       \\ 
\hhline{|~||----||--|}
                                                              & E            & I                     & E            & I                     & {\cellcolor[rgb]{0.854,0.854,0.854}}IKA & {\cellcolor[rgb]{0.854,0.854,0.854}}MKA  \\ 
\hline
$\mathcal{P}_{a}: Authenticity$                                  & $\checkmark$ & X                     & $\checkmark$ & $\checkmark$          & {\cellcolor[rgb]{0.854,0.854,0.854}}$-$ & {\cellcolor[rgb]{0.854,0.854,0.854}}$-$  \\ 
\hline
$\mathcal{P}_{f}: Freshness$                                    & $\checkmark$ & X                     & $\checkmark$ & $\checkmark$          & {\cellcolor[rgb]{0.854,0.854,0.854}}$-$ & {\cellcolor[rgb]{0.854,0.854,0.854}}$-$  \\ 
\hline
$\mathcal{P}_{c}: Confidentiality$                              & $\checkmark$ & X                     & $\checkmark$ & $\checkmark$          & {\cellcolor[rgb]{0.854,0.854,0.854}}$-$ & {\cellcolor[rgb]{0.854,0.854,0.854}}$-$  \\ 
\hhline{|=::====:b|>{\arrayrulecolor[rgb]{0.854,0.854,0.854}\doublerulesepcolor[rgb]{0.854,0.854,0.854}}==>{\arrayrulecolor{black}}|}\doublerulesepcolor{white}
\rowcolor[rgb]{0.854,0.854,0.854} $\mathcal{P}_{r}: Revocation$ & $-$          & \multicolumn{1}{c}{-} & $-$          & \multicolumn{1}{c}{-} & X                                       & X                                        \\
\hline
\end{tabular}
}
\end{table}

==> Tables/CANsec3.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}%[h]%[th!]
\centering
\caption{Formally Verifying IVB Security Protocols \kha{are we really showing thst cansec+ and macsec+ have revocation? In our formal verification, what do we verify? that they have revocation or that this revocation closes the internal attacker issue}}
\label{tbl:CANsec}
\resizebox{0.75\columnwidth}{!}{
\arrayrulecolor{black}
\begin{tabular}{|c||cc|cc|}
\hhline{-----}
\multirow{2}{*}{\textbf{Property}} & \multicolumn{2}{c|}{\textbf{CANsec/CKA}} & \multicolumn{2}{c|}{\textbf{MACsec/MKA}} \\
%& \multicolumn{2}{c|}{(w. CKA)} & \multicolumn{2}{c|}{(w. Revocation)} & \multicolumn{2}{c|}{(w. MKA)} & \multicolumn{2}{c|}{(w. Revocation)} \\
\hhline{|~||----}
& \textit{E} & \textit{I} & \textit{E} & \textit{I} \\
\hhline{|=::====|}
$\mathcal{P}_{a}: Authenticity$  & \checkmark & X & \checkmark & X  \\
\hhline{|-||----|}
$\mathcal{P}_{f}: Freshness$  & \checkmark & X & \checkmark & X  \\
\hhline{|-||----|}
$\mathcal{P}_{c}: Confidentiality$  & \checkmark & X & \checkmark & X \\
\hhline{|-||----|}

%& & & & & \\


\end{tabular}
}
\end{table}

==> Tables/Collective.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.945,0.752,0.752}
\definecolor{Grenadier}{rgb}{0.85,0.313,0}
\definecolor{Manhattan}{rgb}{0.945,0.733,0.611}
\begin{table*}
\centering
\caption{Juxtaposition of CAN attack and defense categories along with their severity and efficacy assessments.\kha{old}}
\label{tbl:bigtable}
\resizebox{\textwidth}{!}{

\begin{tblr}{
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  row{5} = {c},
  row{6} = {c},
  row{7} = {c},
  row{8} = {c},
  row{9} = {c},
  row{11} = {c},
  row{12} = {c},
  row{13} = {c},
  row{14} = {c},
  row{15} = {c},
  row{16} = {c},
  row{17} = {c},
  row{18} = {c},
  row{19} = {c},
  row{20} = {c},
  row{21} = {c},
  row{22} = {c},
  row{23} = {Manhattan,c},
  row{24} = {c},
  row{26} = {c},
  row{27} = {c},
  row{28} = {c},
  row{29} = {c},
  row{30} = {c},
  row{31} = {c},
  row{32} = {c},
  row{33} = {Manhattan,c},
  row{35} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=6}{},
  cell{1}{9} = {c=7}{},
  cell{3}{1} = {r=11}{},
  cell{3}{2} = {r=5}{},
  cell{3}{3} = {Matrix,fg=white},
  cell{3}{4} = {BeautyBush},
  cell{3}{5} = {BeautyBush},
  cell{3}{6} = {BeautyBush},
  cell{3}{7} = {BeautyBush},
  cell{3}{8} = {BeautyBush},
  cell{3}{9} = {r=2}{},
  cell{3}{10} = {r=2}{},
  cell{3}{11} = {r=2}{},
  cell{3}{12} = {r=2}{},
  cell{3}{13} = {r=2}{},
  cell{3}{14} = {r=2}{},
  cell{3}{15} = {r=2}{},
  cell{6}{9} = {r=2}{},
  cell{6}{10} = {r=2}{},
  cell{6}{11} = {r=2}{},
  cell{6}{12} = {r=2}{},
  cell{6}{13} = {r=2}{},
  cell{6}{14} = {r=2}{},
  cell{6}{15} = {r=2}{},
  cell{8}{2} = {r=3}{},
  cell{8}{3} = {BeautyBush},
  cell{8}{4} = {BeautyBush},
  cell{8}{5} = {BeautyBush},
  cell{8}{6} = {BeautyBush},
  cell{8}{7} = {BeautyBush},
  cell{8}{8} = {BeautyBush},
  cell{10}{3} = {r=2}{c},
  cell{10}{4} = {r=2}{c},
  cell{10}{5} = {r=2}{c},
  cell{10}{6} = {r=2}{c},
  cell{10}{7} = {r=2}{c},
  cell{10}{8} = {r=2}{},
  cell{10}{9} = {r=3}{c},
  cell{10}{10} = {r=3}{c},
  cell{10}{11} = {r=3}{c},
  cell{10}{12} = {r=3}{c},
  cell{10}{13} = {r=3}{c},
  cell{10}{14} = {r=3}{c},
  cell{10}{15} = {r=3}{c},
  cell{11}{2} = {r=3}{},
  cell{14}{1} = {r=13}{},
  cell{14}{2} = {r=4}{},
  cell{14}{3} = {Matrix,fg=white},
  cell{14}{4} = {BeautyBush},
  cell{14}{5} = {BeautyBush},
  cell{14}{6} = {BeautyBush},
  cell{14}{7} = {BeautyBush},
  cell{14}{8} = {BeautyBush},
  cell{18}{2} = {r=7}{},
  cell{18}{3} = {BeautyBush},
  cell{18}{4} = {BeautyBush},
  cell{18}{5} = {BeautyBush},
  cell{18}{6} = {BeautyBush},
  cell{18}{7} = {BeautyBush},
  cell{18}{8} = {BeautyBush},
  cell{19}{9} = {r=2}{},
  cell{19}{10} = {r=2}{},
  cell{19}{11} = {r=2}{},
  cell{19}{12} = {r=2}{},
  cell{19}{13} = {r=2}{},
  cell{19}{14} = {r=2}{},
  cell{19}{15} = {r=2}{},
  cell{21}{3} = {Grenadier,fg=white},
  cell{21}{4} = {Manhattan},
  cell{21}{5} = {Manhattan},
  cell{21}{6} = {Manhattan},
  cell{21}{7} = {Manhattan},
  cell{21}{8} = {Manhattan},
  cell{21}{9} = {r=3}{},
  cell{21}{10} = {r=3}{},
  cell{21}{11} = {r=3}{},
  cell{21}{12} = {r=3}{},
  cell{21}{13} = {r=3}{},
  cell{21}{14} = {r=3}{},
  cell{21}{15} = {r=3}{},
  cell{24}{3} = {BeautyBush},
  cell{24}{4} = {BeautyBush},
  cell{24}{5} = {BeautyBush},
  cell{24}{6} = {BeautyBush},
  cell{24}{7} = {BeautyBush},
  cell{24}{8} = {BeautyBush},
  cell{25}{2} = {r=2}{},
  cell{25}{3} = {c},
  cell{25}{4} = {c},
  cell{25}{5} = {c},
  cell{25}{6} = {c},
  cell{25}{7} = {c},
  cell{25}{8} = {c},
  cell{25}{9} = {c},
  cell{25}{10} = {c},
  cell{25}{11} = {c},
  cell{25}{12} = {c},
  cell{25}{13} = {c},
  cell{25}{14} = {c},
  cell{25}{15} = {c},
  cell{27}{1} = {r=8}{},
  cell{27}{2} = {r=3}{},
  cell{27}{9} = {r=3}{},
  cell{27}{10} = {r=3}{},
  cell{27}{11} = {r=3}{},
  cell{27}{12} = {r=3}{},
  cell{27}{13} = {r=3}{},
  cell{27}{14} = {r=3}{},
  cell{27}{15} = {r=3}{},
  cell{30}{2} = {r=4}{},
  cell{30}{3} = {Grenadier,fg=white},
  cell{30}{4} = {BeautyBush},
  cell{30}{5} = {BeautyBush},
  cell{30}{6} = {BeautyBush},
  cell{30}{7} = {BeautyBush},
  cell{30}{8} = {BeautyBush},
  cell{31}{3} = {Grenadier,fg=white},
  cell{31}{4} = {BeautyBush},
  cell{31}{5} = {BeautyBush},
  cell{31}{6} = {BeautyBush},
  cell{31}{7} = {BeautyBush},
  cell{31}{8} = {BeautyBush},
  cell{32}{3} = {Grenadier,fg=white},
  cell{32}{4} = {BeautyBush},
  cell{32}{5} = {BeautyBush},
  cell{32}{6} = {BeautyBush},
  cell{32}{7} = {BeautyBush},
  cell{32}{8} = {BeautyBush},
  cell{32}{9} = {r=2}{},
  cell{32}{10} = {r=2}{},
  cell{32}{11} = {r=2}{},
  cell{32}{12} = {r=2}{},
  cell{32}{13} = {r=2}{},
  cell{32}{14} = {r=2}{},
  cell{32}{15} = {r=2}{},
  cell{33}{3} = {Grenadier,fg=white},
  cell{34}{2} = {r=2}{},
  cell{34}{3} = {c},
  cell{34}{4} = {c},
  cell{34}{5} = {c},
  cell{34}{6} = {c},
  cell{34}{7} = {c},
  cell{34}{8} = {c},
  cell{34}{9} = {c},
  cell{34}{10} = {c},
  cell{34}{11} = {c},
  cell{34}{12} = {c},
  cell{34}{13} = {c},
  cell{34}{14} = {c},
  cell{34}{15} = {c},
  vlines,
  vline{4} = {4}{dotted},
  hline{1,3,14,27,36} = {-}{},
  hline{2,5-6,9-10,13,15,17,19,26} = {3-15}{},
  hline{4,7,12,16,20-23,28-29,31-33} = {3-8}{},
  hline{8,34} = {2-8}{},
  hline{11} = {2}{},
  hline{16,21,31-32} = {9-15}{dotted},
  hline{18,25,30} = {2-15}{},
  hline{24} = {3-7}{},
  hline{24} = {8-15}{dashed},
  hline{34} = {9-15}{dashed},
  hline{35} = {1,3-15}{},
}
\begin{sideways}\end{sideways}       & \begin{sideways}Layer\end{sideways}      & Attack                              &                                       &                                        &                                      &                                          &                                          & Defense                                                                                                                                                 &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Category                            & $\mathcal{B}$ & $\mathcal{Q}$ & $\mathcal{X}$ & $\mathcal{V}$ & $\mathcal{D}$ & Category                                                                                                                                                & $\mathcal{I}$ & $\Lambda$                                                           & $\mathcal{E}$                                                         & $\beta$                                                             & $\mathcal{F}$                                                 & $\vartheta$                                                   \\
\begin{sideways}Confidentiality\end{sideways} & \begin{sideways}Higher\end{sideways}     & Communication Surveillance          & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\LEFTcircle$                            & Message Obfuscation                                                                                                                                     & P                                        & $\LEFTcircle$                                                                                    & $\CIRCLE$                                                                                        & $\CIRCLE$                                                                                            & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Privacy Leakage                     & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\LEFTcircle$                            &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Sensitive Information Sniffing      & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\Circle$                                & $\LEFTcircle$                            & {Better Implementation  Patching\\Message Obfuscation}                                                                                                  & {P\\P}                                   & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\Circle$\\$\Circle$}                                                                           & {$\Circle$\\$\Circle$}                                                                               & {$\Circle$\\$\Circle$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              &                                          & Memory Leakage                      & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\Circle$                                & $\Circle$                                & {Memory and Firmware Concealment\\Better Implementation Patching}                                                                                       & {P\\P}                                   & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\LEFTcircle$\\$\Circle$}                                                                       & {$\Circle$\\$\Circle$}                                                                               & {$\LEFTcircle$\\$\Circle$}                                                                   & {$\LEFTcircle$\\$\CIRCLE$}                                                               \\
                                              &                                          & Information and Firmware Dump       & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\Circle$                                & $\CIRCLE$                                &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error-Based Reconnaissance          & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & {One-Shot Mode\\lnterframe-Spacing Anonymization\\ID Anonymization}                                                                                     & {P\\P\\P}                                & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\Circle$\\$\LEFTcircle$\\$\Circle$}                                                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$}                                                            & {$\Circle$\\$\Circle$\\$\Circle$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & Clock-Skew Network Mapping          & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\LEFTcircle$                            & Skew Cloaking                                                                                                                                           & P                                        & $\CIRCLE$                                                                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                            & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Signal and Hardware Profiling       & $\CIRCLE$                             & $\CIRCLE$                              & $\LEFTcircle$                        & $\CIRCLE$                                & $\LEFTcircle$                            & –                                                                                                                                                       & –                                        & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        \\
                                              & \begin{sideways}Transwire\end{sideways}  &                                     &                                       &                                        &                                      &                                          &                                          &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Topology Intelligence               & $\CIRCLE$                             & $\CIRCLE$                              & $\CIRCLE$                            & $\CIRCLE$                                & $\LEFTcircle$                            &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Electromagnetic Emissions           & $\CIRCLE$                             & $\CIRCLE$                              & $\LEFTcircle$                        & $\CIRCLE$                                & $\LEFTcircle$                            & Shielding and Signal Slope Control                                                                                                                      & P                                        & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & $\Circle$                                                                                \\
\begin{sideways}Integrity\end{sideways}       & \begin{sideways}Higher\end{sideways}     & Fake Data Fabrication               & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\LEFTcircle$                            & Content Inspection                                                                                                                                      & D                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Memory and Firmware Manipulation    & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\Circle$                                & $\CIRCLE$                                & Firmware Attestation                                                                                                                                    & D,P                                      & $\CIRCLE$                                                                                        & $\Circle$                                                                                        & $\Circle$                                                                                            & $\CIRCLE$                                                                                    & $\LEFTcircle$                                                                            \\
                                              &                                          & Bypassing Diagnostic Authentication & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\Circle$                                & $\LEFTcircle$                            & {Diagnostic Session Authentication\\Control Flow Integrity}                                                                                             & {P\\P}                                   & {$\CIRCLE$\\$\LEFTcircle$}                                                                       & {$\Circle$\\$\LEFTcircle$}                                                                       & {$\Circle$\\$\Circle$}                                                                               & {$\Circle$\\$\CIRCLE$}                                                                       & {$\CIRCLE$\\$\LEFTcircle$}                                                               \\
                                              &                                          & Session-Based Buffer Overflow       & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\Circle$                                & $\Circle$                                & {Better Implementation Patching\\ECU Guardian\\Content Inspection}                                                                                      & {P\\P\\~D,P*}                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                            & {$\Circle$\\$\Circle$\\$\Circle$}                                            & {$\Circle$\\$\Circle$\\$\Circle$}                                                & {$\Circle$\\$\CIRCLE$\\$\Circle$}                                        & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                                \\
                                              & \begin{sideways}Controller\end{sideways} & Impersonation and Replay            & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & {Content Inspection\\PIDS\\Per-ECU Authentication\\Centralized Authentication\\Time IFS Anonymization\\Bit-Banger IDS\\Victim Resistance\\ECU Guardian} & {D\\D,P*\\D,P\\D,P*\\D,P*\\D,P*\\P\\P}   & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} & {$\Circle$\\$\Circle$\\$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$} & {$\Circle$\\$\Circle$\\$\LEFTcircle$\\$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$} & {$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\LEFTcircle$\\$\CIRCLE$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} \\
                                              &                                          & Poly-semantic Frames                & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\LEFTcircle$                            & Unifying Sampling Points                                                                                                                                & P                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\LEFTcircle$                                                                                & $\LEFTcircle$                                                                            \\
                                              &                                          & Frame Tampering~                    & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\LEFTcircle$                            &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Double Receive                      & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & {ECU Guardian\\Bit-Banger IDS\\Dynamic Fragmentation}                                                                                                   & {P\\D,P*\\P*}                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\Circle$\\$\Circle$\\$\Circle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                    & {$\CIRCLE$\\$\Circle$\\$\CIRCLE$}                                                            & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$}                                                \\
                                              &                                          & Polyglot Frames                     & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\LEFTcircle$                            &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Unorthodox Frames                   & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Frame Hijacking                     & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & {ID Anonymization\\Interframe-Spacing Anonymization}                                                                                                    & {P\\P}                                   & {$\LEFTcircle$\\$\LEFTcircle$}                                                                   & {$\Circle$\\$\LEFTcircle$}                                                                       & {$\Circle$\\$\LEFTcircle$}                                                                           & {$\Circle$\\$\Circle$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              & \begin{sideways}Transwire\end{sideways}  & Physical-Fingerprint Distortion     & $\Circle$                             & ~$\Circle$                             & ~$\Circle$                           & $\CIRCLE$                                & $\Circle$                                & {Bit-Banger IDS \\ID Anonymization\\Interframe-Spacing Anonymization}                                                                                   & {D,P*\\P\\P}                             & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                            & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & Physical Architecture Manipulation  & $\CIRCLE$                             & $\CIRCLE$                              & $\CIRCLE$                            & $\CIRCLE$                                & $\Circle$                                & PIDS (Locator)                                                                                                                                          & D                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\CIRCLE$                                                                                    & $\CIRCLE$                                                                                \\
\begin{sideways}Availability\end{sideways}    & \begin{sideways}Higher\end{sideways}     & ECU Functionality Disabling         & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\LEFTcircle$                            & {Better Implementation  Patching\\Content Inspection \\ECU Guardian}                                                                                    & {P\\D\\P}                                & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                    & {$\Circle$\\$\Circle$\\$\CIRCLE$}                                                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                \\
                                              &                                          & Higher-Layer Sybil Exhaustion       & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\Circle$                                &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Request Overwhelming                & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\LEFTcircle$                            & $\Circle$                                &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error State Manipulation            & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & One-Shot Mode                                                                                                                                           & S                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\LEFTcircle$                                                                                        & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Error-Injection                     & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & {Error Handling IDS\\ID Anonymization\\Interframe-Spacing Anonymization}                                                                                & {D\\P\\D,P}                              & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                            & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                            & {$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$}                                                    \\
                                              &                                          & Bus Access Denial                   & $\Circle$                             & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                & {Layer-II Node Suspension\\ID Priority Dissociation\\Dynamic Fragmentation \\ECU Guardian\\Bit-Banger IDS}                                              & {P\\P\\P*\\P\\D}                         & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                              & {$\Circle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$}                                      & {$\Circle$\\$\CIRCLE$\\$\Circle$\\$\Circle$\\$\Circle$}                                              & {$\Circle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\Circle$}                                      & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                              \\
                                              &                                          & Synchronization Disruption          & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\Circle$                                &                                                                                                                                                         &                                          &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Transwire\end{sideways}  & Signal Attenuation                  & $\LEFTcircle$                         & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\CIRCLE$                                & PIDS                                                                                                                                                    & D                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\Circle$                                                                                    & $\LEFTcircle$                                                                            \\
                                              &                                          & Physical Vandalism                  & $\CIRCLE$                         & $\Circle$                              & $\Circle$                            & $\CIRCLE$                                & $\CIRCLE$                                & –                                                                                                                                                       & –                                        & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        
\end{tblr}
}
\end{table*}

==> Tables/Collective2.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.90,0.70,0.60}
\definecolor{Manhattan}{rgb}{0.7600,0.7955,0.8992}
\definecolor{BurntOrange}{rgb}{0.3373, 0.4353, 0.7216}

\definecolor{Bobo}{RGB}{176,145,122}
% \definecolor{BurntOrange}{rgb}{0.807,0.298,0}
% \definecolor{Manhattan}{rgb}{0.945,0.733,0.611}
% \definecolor{Alto}{rgb}{0.854,0.854,0.854}
% \definecolor{SilverChalice}{rgb}{0.678,0.678,0.678}
%\definecolor{Bobo}{rgb}{0.945,0.752,0.752}
%try this pink {1,0.9,0.86}
\begin{table*}
\centering
\caption{Juxtaposing Each CAN Attack Category Against Possible Defense Categories with Severity and Efficacy Assessments}
\label{tbl:bigtable}
\resizebox*{0.96\textwidth}{0.96\textheight}{
% \setlength\extrarowheight{-5pt}
\small
\begin{tblr}{
  rows = {valign = m},
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  row{5} = {c},
  row{6} = {c},
  row{7} = {c},
  row{8} = {c},
  row{9} = {c},
  row{11} = {c},
  row{12} = {c},
  row{13} = {c},
  row{14} = {c},
  row{15} = {c},
  row{16} = {c},
  row{17} = {c},
  row{18} = {c},
  row{19} = {c},
  row{20} = {c},
  row{21} = {c},
  row{22} = {c},
  %row{23} = {Manhattan,c},
  row{24} = {c},
  row{26} = {c},
  row{27} = {c},
  row{28} = {c},
  row{29} = {c},
  row{30} = {c},
  row{31} = {c},
  row{32} = {c},
  row{33} = {c},
  row{35} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=6}{},
  cell{1}{9} = {c=7}{},
  cell{3}{1} = {r=11}{},
  cell{3}{2} = {r=5}{},
  cell{3}{3} = {Matrix,fg=white,halign=c},
  cell{3}{4} = {Bobo},
  cell{3}{5} = {Bobo},
  cell{3}{6} = {Bobo},
  cell{3}{7} = {Bobo},
  cell{3}{8} = {Bobo},
  cell{3}{9} = {r=2}{c},
  cell{3}{10} = {r=2}{},
  cell{3}{11} = {r=2}{},
  cell{3}{12} = {r=2}{},
  cell{3}{13} = {r=2}{},
  cell{3}{14} = {r=2}{},
  cell{3}{15} = {r=2}{},
  cell{4}{3} = {halign=c},
  cell{5}{3} = {halign=c},
  cell{5}{9} = {halign=c},
  cell{6}{3} = {halign=c},
  cell{6}{9} = {r=2}{c},
  cell{6}{10} = {r=2}{},
  cell{6}{11} = {r=2}{},
  cell{6}{12} = {r=2}{},
  cell{6}{13} = {r=2}{},
  cell{6}{14} = {r=2}{},
  cell{6}{15} = {r=2}{},
  cell{7}{3} = {halign=c},
  cell{7}{9} = {halign=c},
  cell{8}{2} = {r=2}{},
  cell{8}{3} = {BurntOrange,fg=white,halign=c},
  cell{8}{4} = {Bobo},
  cell{8}{5} = {Bobo},
  cell{8}{6} = {Bobo},
  cell{8}{7} = {Bobo},
  cell{8}{8} = {Bobo},
  cell{8}{9} = {halign=c},
  cell{9}{3} = {halign=c},
  cell{9}{9} = {halign=c},
  cell{10}{2} = {r=4}{},
  cell{10}{3} = {r=2}{c},
  cell{10}{4} = {r=2}{c},
  cell{10}{5} = {r=2}{c},
  cell{10}{6} = {r=2}{c},
  cell{10}{7} = {r=2}{c},
  cell{10}{8} = {r=2}{},
  cell{10}{9} = {r=3}{c},
  cell{10}{10} = {r=3}{c},
  cell{10}{11} = {r=3}{c},
  cell{10}{12} = {r=3}{c},
  cell{10}{13} = {r=3}{c},
  cell{10}{14} = {r=3}{c},
  cell{10}{15} = {r=3}{c},
  %cell{11}{2} = {r=3}{},
  cell{11}{3} = {halign=c},
  cell{11}{9} = {halign=c},
  cell{12}{3} = {halign=c},
  cell{12}{9} = {halign=c},
  cell{13}{3} = {halign=c},
  cell{13}{9} = {halign=c},
  cell{14}{1} = {r=13}{},
  cell{14}{2} = {r=4}{},
  cell{14}{3} = {Matrix,fg=white,halign=c},
  cell{14}{4} = {Bobo},
  cell{14}{5} = {Bobo},
  cell{14}{6} = {Bobo},
  cell{14}{7} = {Bobo},
  cell{14}{8} = {Bobo},
  cell{14}{9} = {halign=c},
  cell{15}{3} = {halign=c},
  cell{15}{9} = {r=2}{c},
  cell{15}{10} = {r=2}{},
  cell{15}{11} = {r=2}{},
  cell{15}{12} = {r=2}{},
  cell{15}{13} = {r=2}{},
  cell{15}{14} = {r=2}{},
  cell{15}{15} = {r=2}{},
  cell{16}{3} = {halign=c},
  cell{16}{9} = {halign=c},
  cell{17}{3} = {halign=c},
  cell{17}{9} = {halign=c},
  cell{18}{2} = {r=7}{},
  cell{18}{3} = {Bobo,halign=c},
  cell{18}{4} = {Bobo},
  cell{18}{5} = {Bobo},
  cell{18}{6} = {Bobo},
  cell{18}{7} = {Bobo},
  cell{18}{8} = {Bobo},
  cell{18}{9} = {halign=c},
  %cell{19}{9} = {r=2}{},
  %cell{19}{10} = {r=2}{},
  %cell{19}{11} = {r=2}{},
  %cell{19}{12} = {r=2}{},
  %cell{19}{13} = {r=2}{},
  %cell{19}{14} = {r=2}{},
  %cell{19}{15} = {r=2}{},
  cell{19}{3} = {halign=c},
  cell{19}{9} = {halign=c},
  cell{20}{3} = {halign=c},
  cell{20}{9} = {halign=c},
  cell{21}{3} = {BurntOrange,fg=white,halign=c},
  cell{21}{4} = {Manhattan},
  cell{21}{5} = {Manhattan},
  cell{21}{6} = {Manhattan},
  cell{21}{7} = {Manhattan},
  cell{21}{8} = {Manhattan},
  cell{21}{9} = {r=3}{c},
  cell{21}{10} = {r=3}{},
  cell{21}{11} = {r=3}{},
  cell{21}{12} = {r=3}{},
  cell{21}{13} = {r=3}{},
  cell{21}{14} = {r=3}{},
  cell{21}{15} = {r=3}{},
  cell{22}{3} = {Manhattan,halign=c},
  cell{22}{4} = {Manhattan},
  cell{22}{5} = {Manhattan},
  cell{22}{6} = {Manhattan},
  cell{22}{7} = {Manhattan},
  cell{22}{8} = {Manhattan},
  %cell{22}{3} = {halign=c},
  cell{22}{9} = {halign=c},
  cell{23}{3} = {halign=c},
  cell{23}{3} = {halign=c},
  cell{23}{4} = {halign=c},
  cell{23}{5} = {halign=c},
  cell{23}{6} = {halign=c},
  cell{23}{7} = {halign=c},
  cell{23}{8} = {halign=c},
  cell{23}{9} = {halign=c},
  cell{24}{3} = {Bobo,halign=c},
  cell{24}{4} = {Bobo},
  cell{24}{5} = {Bobo},
  cell{24}{6} = {Bobo},
  cell{24}{7} = {Bobo},
  cell{24}{8} = {Bobo},
  cell{24}{9} = {halign=c},
  cell{25}{2} = {r=2}{},
  cell{25}{3} = {Bobo,c},
  cell{25}{4} = {Bobo,c},
  cell{25}{5} = {Bobo,c},
  cell{25}{6} = {Bobo,c},
  cell{25}{7} = {Bobo,c},
  cell{25}{8} = {Bobo,c},
  cell{25}{9} = {c},
  cell{25}{10} = {c},
  cell{25}{11} = {c},
  cell{25}{12} = {c},
  cell{25}{13} = {c},
  cell{25}{14} = {c},
  cell{25}{15} = {c},
  cell{26}{3} = {halign=c},
  cell{26}{9} = {halign=c},
  cell{27}{1} = {r=9}{},
  cell{27}{2} = {r=3}{},
  cell{27}{3} = {halign=c},
  cell{27}{9} = {r=3}{c},
  cell{27}{10} = {r=3}{},
  cell{27}{11} = {r=3}{},
  cell{27}{12} = {r=3}{},
  cell{27}{13} = {r=3}{},
  cell{27}{14} = {r=3}{},
  cell{27}{15} = {r=3}{},
  cell{28}{3} = {halign=c},
  cell{28}{9} = {halign=c},
  cell{29}{3} = {halign=c},
  cell{29}{9} = {halign=c},
  cell{30}{2} = {r=4}{},
  cell{30}{3} = {BurntOrange,fg=white,halign=c},
  cell{30}{4} = {Bobo},
  cell{30}{5} = {Bobo},
  cell{30}{6} = {Bobo},
  cell{30}{7} = {Bobo},
  cell{30}{8} = {Bobo},
  cell{30}{9} = {halign=c},
  cell{31}{3} = {BurntOrange,fg=white,halign=c},
  cell{31}{4} = {Bobo},
  cell{31}{5} = {Bobo},
  cell{31}{6} = {Bobo},
  cell{31}{7} = {Bobo},
  cell{31}{8} = {Bobo},
  cell{31}{9} = {halign=c},
  cell{32}{3} = {BurntOrange,fg=white,halign=c},
  cell{32}{4} = {Bobo},
  cell{32}{5} = {Bobo},
  cell{32}{6} = {Bobo},
  cell{32}{7} = {Bobo},
  cell{32}{8} = {Bobo},
  cell{32}{9} = {halign=c},
  cell{33}{3} = {BurntOrange,fg=white,halign=c},
  cell{33}{4} = {Manhattan},
  cell{33}{5} = {Manhattan},
  cell{33}{6} = {Manhattan},
  cell{33}{7} = {Manhattan},
  cell{33}{8} = {Manhattan},
  cell{33}{9} = {halign=c},
  %cell{34}{9} = {c},
  %cell{34}{10} = {c},
  %cell{34}{11} = {c},
  %cell{34}{12} = {c},
  %cell{34}{13} = {c},
  %cell{34}{14} = {c},
  %cell{34}{15} = {c},
  cell{34}{2} = {r=2}{},
  cell{34}{3} = {c},
  cell{34}{4} = {c},
  cell{34}{5} = {c},
  cell{34}{6} = {c},
  cell{34}{7} = {c},
  cell{34}{8} = {c},
  cell{34}{9} = {c},
  cell{34}{10} = {c},
  cell{34}{11} = {c},
  cell{34}{12} = {c},
  cell{34}{13} = {c},
  cell{34}{14} = {c},
  cell{34}{15} = {c},
  cell{35}{3} = {c},
  cell{35}{4} = {c},
  cell{35}{5} = {c},
  cell{35}{6} = {c},
  cell{35}{7} = {c},
  cell{35}{8} = {c},
  cell{35}{9} = {c},
  cell{35}{10} = {c},
  cell{35}{11} = {c},
  cell{35}{12} = {c},
  cell{35}{13} = {c},
  cell{35}{14} = {c},
  cell{35}{15} = {c},
  vlines,
  %vline{4} = {4}{dotted},
  hline{1,3,14,27,36} = {-}{},
  hline{2,5-6,9-10,13,15,17,19,26,35,36} = {3-15}{},
  hline{4,7,20-24,28-29,31-33} = {3-8}{},
  hline{4,7,16,20-24,28-29,31-33} = {3-8}{},
  hline{8, 10, 18,25,30,34} = {2-15}{},
  %hline{11} = {2}{},
  hline{20,21,31-33} = {9-15}{dotted},
  hline{24} = {9-15}{dashed},
  hline{35} = {2-8}{},
}
\begin{sideways}\end{sideways}                & \begin{sideways}Layer\end{sideways}      & Attack &               &               &               &               &               & Defense                                                                                                                                                 &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
& & Category & \abl & \eqp & \ax  & \prev & \diff & Category & \ins &
\cov & \ecu & \bus & \infra & \val \\
\begin{sideways}Confidentiality\end{sideways} & \begin{sideways}Higher\end{sideways}     & Communication Surveillance (\Ca)          & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\LEFTcircle$ & Message Obfuscation (\DCa)                                                                                                                                    & P                                      & $\LEFTcircle$                                                                                    & $\low$                                                                                        & $\low$                                                                                            & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Privacy Leakage (\Cb)                     & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Sensitive Information Sniffing (\Cc)      & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\LEFTcircle$ & {Message Obfuscation (\DCa)\\Better Implementation \&  Patching (\DIc)}                                                                                                  & {P\\P}                                 & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\high$\\$\high$}                                                                           & {$\high$\\$\high$}                                                                               & {$\high$\\$\high$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              &                                          & Information and Firmware Dump (\Cd)                     & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\CIRCLE$     & {Better Implementation Patching (\DIc)\\ECU Firmware Hardening (\DId)}                                                                                       & {P\\P}                                 & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\high$\\$\moderate$}                                                                       & {$\high$\\$\high$}                                                                               & {$\high$\\$\moderate$}                                                                   & {$\CIRCLE$\\$\LEFTcircle$}                                                               \\
                                              &                                          & Memory Leakage (\Ce)       & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error-Based Reconnaissance (\Cf) & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {ID Anonymization (\DCc) \\Interframe-Spacing Anonymization (\DIh)\\One-Shot Mode (\DAb)}                                                                                     & {P\\P\\P}                              & {$\LEFTcircle$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\high$\\$\moderate$\\$\high$}                                                            & {$\high$\\$\moderate$\\$\moderate$}                                                            & {$\high$\\$\high$\\$\high$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & Clock-Skew Network Mapping (\Cg)          & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & Skew Cloaking (\DCb)                                                                                                                                           & P                                      & $\CIRCLE$                                                                                        & $\moderate$                                                                                    & $\high$                                                                                            & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              & \begin{sideways}Transwire\end{sideways}                                         & Signal and Hardware Profiling (\Ch)       & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$ & \standard     & ~$\LEFTcircle$ & –                                                                                                                                                       & –                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        \\
                                              &   &                                     &               &               &               &               &               &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Topology Intelligence (\Ci)               & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & \standard     & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Electromagnetic Emissions (\Cj)           & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$ & \standard     & $\LEFTcircle$ & Shielding and Signal Slope Control (\DCd)                                                                                                                    & P                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & $\Circle$                                                                                \\
\begin{sideways}Integrity\end{sideways}       & \begin{sideways}Higher\end{sideways}     & Fake Data Fabrication (\Ia)               & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\LEFTcircle$ & Content Inspection (\DIb)                                                                                                                                    & D                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Memory and Firmware Manipulation (\Ib)    & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\CIRCLE$     & {ECU Firmware Hardening (\DId)\\Diagnostic Session Authentication (\DIa)}                                                                                                                                  & {D,P\\P}                                   & {$\CIRCLE$\\$\CIRCLE$}                                                                                        & {$\high$\\$\high$}                                                                                        & {$\high$\\$\high$}                                                                                           & {$\moderate$\\$\high$}                                                                                   & {$\LEFTcircle$\\$\CIRCLE$}                                                                            \\
                                              &                                          & Bypassing Diagnostic Authentication (\Ic) & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\LEFTcircle$ &                                                                                              &                                 &                                                                        &                                                                        &                                                                                &                                                                        &                                                                \\
                                              &                                          & Session-Based Buffer Overflow (\Id)       & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\Circle$     & {Content Inspection (\DIb)\\Better Implementation Patching (\DIc)\\ECU Guardian (\DIk)}                                                                                      & {~D,P*\\P\\P}                          & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                                    & {$\high$\\$\high$\\$\low$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\LEFTcircle$}                                                    \\
                                              & \begin{sideways}Controller\end{sideways} & Impersonation and Replay (\Ie)            & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {Per-ECU Authentication (\DIa)\\Centralized Authentication (\DIa)\\Victim Resistance (\DIF)\\Time IFS Anonymization (\DIh)\\ PIDS (\DIi)\\Bit-Banger IDS (\DIj)\\ECU Guardian (\DIk)} & {D,P\\D,P*\\P\\D,P*\\D,P*\\D,P\\P} & {$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} & {$\low$\\$\moderate$\\$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$} & {$\moderate$\\$\moderate$\\$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$} & {$\high$\\$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$\\$\low$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} \\
                                              &                                          & Frame Tampering (\Ij)                & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & VIDS (\DIi)                                                                                                                                & D                                     & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\high$                                                                                & $\CIRCLE$                                                                            \\
                                              &                                          & Poly-semantic Frames (\Ii)~                    & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & Unifying Sampling Points (\DIg)                                                                                                                                                        &  P                                      &    $\LEFTcircle$                                                                                              &  \high                                                                                                &   \high                                                                                                   &     \moderate                                                                                         &       $\LEFTcircle$                                                                                   \\
                                              &                                          & Double Receive (\Ig)                      & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {Bit-Banger IDS (\DIj)\\ECU Guardian (\DIk)\\ Dynamic Fragmentation (\DAe)}                                                                                                   & {D,P*\\P\\P*}                          & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                                    & {$\high$\\$\low$\\$\low$}                                                            & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                \\
                                              &                                          & Unorthodox Frames (\Ih)                    & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \standard & $\Circle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Polyglot Frames (\Ik)                   & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \widespread     & $\LEFTcircle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Frame Hijacking (\IF)                     & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {ID Anonymization (\DCc)\\ Interframe-Spacing Anonymization (\DIh)}                                                                                                    & {P\\P}                                 & {$\LEFTcircle$\\$\LEFTcircle$}                                                                   & {$\high$\\$\moderate$}                                                                       & {$\high$\\$\moderate$}                                                                           & {$\high$\\$\high$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              & \begin{sideways}Transwire\end{sideways}  & Physical-Fingerprint Distortion (\Il)     & $\Circle$     & ~$\Circle$    & ~$\Circle$    & \standard     & $\Circle$     & {ID Anonymization (\DCc)\\ Interframe-Spacing Anonymization (\DIh)\\Bit-Banger IDS (\DIj)\\ECU Guardian (\DIk)\\ Dynamic Fragmentation (\DAe)}                                                                                   & {P\\P\\D,P*\\P\\P*}                           & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$}                                                            & {$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$\\$\low$\\$\low$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        \\
                                              &                                          & Physical Architecture Manipulation (\IM)  & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & \standard     & $\CIRCLE$     & PIDS (Locator) (\DIi)                                                                                                                                         & D                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\low$                                                                                    & $\CIRCLE$                                                                                \\
\begin{sideways}Availability\end{sideways}    & \begin{sideways}Higher\end{sideways}     & ECU Functionality Disabling (\Aa)         & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & {Content Inspection (\DIb) \\Better Implementation  Patching (\DIc)\\ECU Guardian (\DIk)}                                                                                    & {D\\P\\P}                              & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                                    & {$\high$\\$\high$\\$\low$}                                                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                \\
                                              &                                          & Request Overwhelming (\Ab)       & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Higher-Layer Sybil Exhaustion (\Ac)               & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error State Manipulation (\Ae)            & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & One-Shot Mode (\DAb)                                                                                                                                          & S                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\moderate$                                                                                        & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Error-Injection (\Ad)                     & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {ID Anonymization (\DCc)\\ Interframe-Spacing Anonymization (\DIh)\\Error Handling IDS (\DAc)}                                                                                & {P\\D,P\\D}                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\high$\\$\moderate$\\$\high$}                                                            & {$\high$\\$\moderate$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\LEFTcircle$}                                                    \\
                                              &                                          & Bus Access Denial (\Af)                   & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {ID Priority Dissociation (\DAa)\\Layer-II Node Suspension (\DAd)}                                              & {P\\P}                      & {$\LEFTcircle$\\$\LEFTcircle$}                              & {$\moderate$\\$\high$}                                      & {$\low$\\$\high$}                                              & {$\low$\\$\high$}                                      & {$\LEFTcircle$\\$\CIRCLE$}                              \\
                                              & & Synchronization Disruption (\Ag) & $\LEFTcircle$ & $\Circle$ & $\Circle$ & \standard & $\Circle$ & {Bit-Banger IDS (\DIj)\\ECU Guardian (\DIk)\\Dynamic Fragmentation (\DAe)} & {D\\P\\P*} & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$} & {$\high$\\$\high$\\$\high$} & {$\high$\\$\high$\\$\high$} & {$\high$\\$\low$\\$\low$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}  \\
                                              %&                                          &      &  &      &    &     &     & {\DIk. ECU Guardian\kha{??}\\\DAe. Dynamic Fragmentation}                                                                                                                                                         &  {P\\P*}                                        &  {$\LEFTcircle$\\$\CIRCLE$}                                                                                                    & {$\high$\\$\high$}                                                                                                 & 
                                              %{$\high$\\$\high$}                                                                                                    &   {$\low$\\$\low$}                                                       &             {$\CIRCLE$\\$\CIRCLE$}                                                                             \\
                                              & \begin{sideways}Transwire\end{sideways}  & Signal Attenuation (\Ah)                  & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \standard     & $\CIRCLE$     & {PIDS (\DIi)\\Dynamic Fragmentation (\DAe)}                                                                                                                                                   & {D\\P*}                                      & {$\LEFTcircle$\\$\CIRCLE$}                                                                                    & {$\high$\\$\high$}                                                                                      & {$\high$\\$\high$}                                                                                          &{$\high$\\$\low$}                                                                                     & {$\LEFTcircle$\\$\LEFTcircle$}                                                                           \\
                                              &                                          & Physical Vandalism (\Ai)                  & $\CIRCLE$     & $\Circle$     & $\CIRCLE$     & \standard     & $\CIRCLE$     & –                                                                                                                                                       & –                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        
\end{tblr}
}
\end{table*}

==> Tables/CollectiveNew.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{1,0.9,0.86}
\definecolor{BurntOrange}{rgb}{0.5,0.5,0.5}
\definecolor{Manhattan}{rgb}{0.854,0.854,0.854}
% \definecolor{BurntOrange}{rgb}{0.807,0.298,0}
% \definecolor{Manhattan}{rgb}{0.945,0.733,0.611}
% \definecolor{Alto}{rgb}{0.854,0.854,0.854}
% \definecolor{SilverChalice}{rgb}{0.678,0.678,0.678}
%\definecolor{BeautyBush}{rgb}{0.945,0.752,0.752}
%try this pink {1,0.9,0.86}
\begin{table*}
\centering
\caption{Juxtaposing each CAN attack category against possible defense categories with severity and efficacy assessments.}
\label{tbl:bigtable}
\resizebox*{0.96\textwidth}{0.96\textheight}{
% \setlength\extrarowheight{-5pt}
\small
\begin{tblr}{
  rows = {valign = m},
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  row{5} = {c},
  row{6} = {c},
  row{7} = {c},
  row{8} = {c},
  row{9} = {c},
  row{11} = {c},
  row{12} = {c},
  row{13} = {c},
  row{14} = {c},
  row{15} = {c},
  row{16} = {c},
  row{17} = {c},
  row{18} = {c},
  row{19} = {c},
  row{20} = {c},
  row{21} = {c},
  row{22} = {c},
  row{23} = {Manhattan,c},
  row{24} = {c},
  row{26} = {c},
  row{27} = {c},
  row{28} = {c},
  row{29} = {c},
  row{30} = {c},
  row{31} = {c},
  row{32} = {c},
  row{33} = {c},
  row{35} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=6}{},
  cell{1}{9} = {c=7}{},
  cell{3}{1} = {r=11}{},
  cell{3}{2} = {r=5}{},
  cell{3}{3} = {Matrix,fg=white,halign=l},
  cell{3}{4} = {BeautyBush},
  cell{3}{5} = {BeautyBush},
  cell{3}{6} = {BeautyBush},
  cell{3}{7} = {BeautyBush},
  cell{3}{8} = {BeautyBush},
  cell{3}{9} = {r=2}{l},
  cell{3}{10} = {r=2}{},
  cell{3}{11} = {r=2}{},
  cell{3}{12} = {r=2}{},
  cell{3}{13} = {r=2}{},
  cell{3}{14} = {r=2}{},
  cell{3}{15} = {r=2}{},
  cell{4}{3} = {halign=l},
  cell{5}{3} = {halign=l},
  cell{5}{9} = {halign=l},
  cell{6}{3} = {halign=l},
  cell{6}{9} = {r=2}{l},
  cell{6}{10} = {r=2}{},
  cell{6}{11} = {r=2}{},
  cell{6}{12} = {r=2}{},
  cell{6}{13} = {r=2}{},
  cell{6}{14} = {r=2}{},
  cell{6}{15} = {r=2}{},
  cell{7}{3} = {halign=l},
  cell{7}{9} = {halign=l},
  cell{8}{2} = {r=2}{},
  cell{8}{3} = {BurntOrange,fg=white,halign=l},
  cell{8}{4} = {BeautyBush},
  cell{8}{5} = {BeautyBush},
  cell{8}{6} = {BeautyBush},
  cell{8}{7} = {BeautyBush},
  cell{8}{8} = {BeautyBush},
  cell{8}{9} = {halign=l},
  cell{9}{3} = {halign=l},
  cell{9}{9} = {halign=l},
  cell{10}{2} = {r=4}{},
  cell{10}{3} = {r=2}{l},
  cell{10}{4} = {r=2}{c},
  cell{10}{5} = {r=2}{c},
  cell{10}{6} = {r=2}{c},
  cell{10}{7} = {r=2}{c},
  cell{10}{8} = {r=2}{},
  cell{10}{9} = {r=3}{c},
  cell{10}{10} = {r=3}{c},
  cell{10}{11} = {r=3}{c},
  cell{10}{12} = {r=3}{c},
  cell{10}{13} = {r=3}{c},
  cell{10}{14} = {r=3}{c},
  cell{10}{15} = {r=3}{c},
  %cell{11}{2} = {r=3}{},
  cell{11}{3} = {halign=l},
  cell{11}{9} = {halign=l},
  cell{12}{3} = {halign=l},
  cell{12}{9} = {halign=l},
  cell{13}{3} = {halign=l},
  cell{13}{9} = {halign=l},
  cell{14}{1} = {r=13}{},
  cell{14}{2} = {r=4}{},
  cell{14}{3} = {Matrix,fg=white,halign=l},
  cell{14}{4} = {BeautyBush},
  cell{14}{5} = {BeautyBush},
  cell{14}{6} = {BeautyBush},
  cell{14}{7} = {BeautyBush},
  cell{14}{8} = {BeautyBush},
  cell{14}{9} = {halign=l},
  cell{15}{3} = {halign=l},
  cell{15}{9} = {r=2}{l},
  cell{15}{10} = {r=2}{},
  cell{15}{11} = {r=2}{},
  cell{15}{12} = {r=2}{},
  cell{15}{13} = {r=2}{},
  cell{15}{14} = {r=2}{},
  cell{15}{15} = {r=2}{},
  cell{16}{3} = {halign=l},
  cell{16}{9} = {halign=l},
  cell{17}{3} = {halign=l},
  cell{17}{9} = {halign=l},
  cell{18}{2} = {r=7}{},
  cell{18}{3} = {BeautyBush,halign=l},
  cell{18}{4} = {BeautyBush},
  cell{18}{5} = {BeautyBush},
  cell{18}{6} = {BeautyBush},
  cell{18}{7} = {BeautyBush},
  cell{18}{8} = {BeautyBush},
  cell{18}{9} = {halign=l},
  %cell{19}{9} = {r=2}{},
  %cell{19}{10} = {r=2}{},
  %cell{19}{11} = {r=2}{},
  %cell{19}{12} = {r=2}{},
  %cell{19}{13} = {r=2}{},
  %cell{19}{14} = {r=2}{},
  %cell{19}{15} = {r=2}{},
  cell{19}{3} = {halign=l},
  cell{19}{9} = {halign=l},
  cell{20}{3} = {halign=l},
  cell{20}{9} = {halign=l},
  cell{21}{3} = {BurntOrange,fg=white,halign=l},
  cell{21}{4} = {Manhattan},
  cell{21}{5} = {Manhattan},
  cell{21}{6} = {Manhattan},
  cell{21}{7} = {Manhattan},
  cell{21}{8} = {Manhattan},
  cell{21}{9} = {r=3}{l},
  cell{21}{10} = {r=3}{},
  cell{21}{11} = {r=3}{},
  cell{21}{12} = {r=3}{},
  cell{21}{13} = {r=3}{},
  cell{21}{14} = {r=3}{},
  cell{21}{15} = {r=3}{},
  cell{22}{3} = {halign=l},
  cell{22}{9} = {halign=l},
  cell{23}{3} = {halign=l},
  cell{23}{9} = {halign=l},
  cell{24}{3} = {BeautyBush,halign=l},
  cell{24}{4} = {BeautyBush},
  cell{24}{5} = {BeautyBush},
  cell{24}{6} = {BeautyBush},
  cell{24}{7} = {BeautyBush},
  cell{24}{8} = {BeautyBush},
  cell{24}{9} = {halign=l},
  cell{25}{2} = {r=2}{},
  cell{25}{3} = {BeautyBush,l},
  cell{25}{4} = {BeautyBush,c},
  cell{25}{5} = {BeautyBush,c},
  cell{25}{6} = {BeautyBush,c},
  cell{25}{7} = {BeautyBush,c},
  cell{25}{8} = {BeautyBush,c},
  cell{25}{9} = {l},
  cell{25}{10} = {c},
  cell{25}{11} = {c},
  cell{25}{12} = {c},
  cell{25}{13} = {c},
  cell{25}{14} = {c},
  cell{25}{15} = {c},
  cell{26}{3} = {halign=l},
  cell{26}{9} = {halign=l},
  cell{27}{1} = {r=9}{},
  cell{27}{2} = {r=3}{},
  cell{27}{3} = {halign=l},
  cell{27}{9} = {r=3}{l},
  cell{27}{10} = {r=3}{},
  cell{27}{11} = {r=3}{},
  cell{27}{12} = {r=3}{},
  cell{27}{13} = {r=3}{},
  cell{27}{14} = {r=3}{},
  cell{27}{15} = {r=3}{},
  cell{28}{3} = {halign=l},
  cell{28}{9} = {halign=l},
  cell{29}{3} = {halign=l},
  cell{29}{9} = {halign=l},
  cell{30}{2} = {r=4}{},
  cell{30}{3} = {BurntOrange,fg=white,halign=l},
  cell{30}{4} = {BeautyBush},
  cell{30}{5} = {BeautyBush},
  cell{30}{6} = {BeautyBush},
  cell{30}{7} = {BeautyBush},
  cell{30}{8} = {BeautyBush},
  cell{30}{9} = {halign=l},
  cell{31}{3} = {BurntOrange,fg=white,halign=l},
  cell{31}{4} = {BeautyBush},
  cell{31}{5} = {BeautyBush},
  cell{31}{6} = {BeautyBush},
  cell{31}{7} = {BeautyBush},
  cell{31}{8} = {BeautyBush},
  cell{31}{9} = {halign=l},
  cell{32}{3} = {BurntOrange,fg=white,halign=l},
  cell{32}{4} = {BeautyBush},
  cell{32}{5} = {BeautyBush},
  cell{32}{6} = {BeautyBush},
  cell{32}{7} = {BeautyBush},
  cell{32}{8} = {BeautyBush},
  cell{32}{9} = {halign=l},
  cell{33}{3} = {BurntOrange,fg=white,halign=l},
  cell{33}{4} = {Manhattan},
  cell{33}{5} = {Manhattan},
  cell{33}{6} = {Manhattan},
  cell{33}{7} = {Manhattan},
  cell{33}{8} = {Manhattan},
  cell{33}{9} = {halign=l},
  %cell{34}{9} = {l},
  %cell{34}{10} = {c},
  %cell{34}{11} = {c},
  %cell{34}{12} = {c},
  %cell{34}{13} = {c},
  %cell{34}{14} = {c},
  %cell{34}{15} = {c},
  cell{34}{2} = {r=2}{},
  cell{34}{3} = {l},
  cell{34}{4} = {c},
  cell{34}{5} = {c},
  cell{34}{6} = {c},
  cell{34}{7} = {c},
  cell{34}{8} = {c},
  cell{34}{9} = {l},
  cell{34}{10} = {c},
  cell{34}{11} = {c},
  cell{34}{12} = {c},
  cell{34}{13} = {c},
  cell{34}{14} = {c},
  cell{34}{15} = {c},
  cell{35}{3} = {l},
  cell{35}{4} = {c},
  cell{35}{5} = {c},
  cell{35}{6} = {c},
  cell{35}{7} = {c},
  cell{35}{8} = {c},
  cell{35}{9} = {c},
  cell{35}{10} = {c},
  cell{35}{11} = {c},
  cell{35}{12} = {c},
  cell{35}{13} = {c},
  cell{35}{14} = {c},
  cell{35}{15} = {c},
  vlines,
  %vline{4} = {4}{dotted},
  hline{1,3,14,27,36} = {-}{},
  hline{2,5-6,9-10,13,15,17,19,26,35,36} = {3-15}{},
  hline{4,7,20-24,28-29,31-33} = {3-8}{},
  hline{4,7,16,20-24,28-29,31-33} = {3-8}{},
  hline{8, 10, 18,25,30,34} = {2-15}{},
  %hline{11} = {2}{},
  hline{20,21,31-33} = {9-15}{dotted},
  hline{24} = {9-15}{dashed},
  hline{35} = {2-8}{},
}
\begin{sideways}\end{sideways}                & \begin{sideways}Layer\end{sideways}      & Attack &               &               &               &               &               & Defense                                                                                                                                                 &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
& & Category & \abl & \eqp & \ax  & \prev & \diff & Category & \ins &
\cov & \ecu & \bus & \infra & \val \\
\begin{sideways}Confidentiality\end{sideways} & \begin{sideways}Higher\end{sideways}     & \Ca. Communication Surveillance          & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\LEFTcircle$ & \DCa. Message Obfuscation                                                                                                                                     & P                                      & $\LEFTcircle$                                                                                    & $\low$                                                                                        & $\low$                                                                                            & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & \Cb. Privacy Leakage                     & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & \Cc. Sensitive Information Sniffing      & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\LEFTcircle$ & {\DCa. Message Obfuscation\\\DIc. Better Implementation \&  Patching}                                                                                                  & {P\\P}                                 & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\high$\\$\high$}                                                                           & {$\high$\\$\high$}                                                                               & {$\high$\\$\high$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              &                                          & \Cd. Information and Firmware Dump                      & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\CIRCLE$     & {\DIc. Better Implementation Patching\\\DId. ECU Firmware Hardening}                                                                                       & {P\\P}                                 & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\high$\\$\moderate$}                                                                       & {$\high$\\$\high$}                                                                               & {$\high$\\$\moderate$}                                                                   & {$\CIRCLE$\\$\LEFTcircle$}                                                               \\
                                              &                                          & \Ce. Memory Leakage       & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & \Cf. Error-Based Reconnaissance & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {\DCc. ID Anonymization\\\DIh. Interframe-Spacing Anonymization\\\DAb. One-Shot Mode}                                                                                     & {P\\P\\P}                              & {$\LEFTcircle$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\high$\\$\moderate$\\$\high$}                                                            & {$\high$\\$\moderate$\\$\moderate$}                                                            & {$\high$\\$\high$\\$\high$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & \Cg. Clock-Skew Network Mapping          & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & \DCb. Skew Cloaking                                                                                                                                           & P                                      & $\CIRCLE$                                                                                        & $\moderate$                                                                                    & $\high$                                                                                            & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              & \begin{sideways}Transwire\end{sideways}                                         & \Ch. Signal and Hardware Profiling       & $\CIRCLE$     & $\CIRCLE$     & $\LEFTcircle$ & \standard     & ~$\LEFTcircle$ & –                                                                                                                                                       & –                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        \\
                                              &   &                                     &               &               &               &               &               &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & \Ci. Topology Intelligence               & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & \standard     & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & \Cj. Electromagnetic Emissions           & $\CIRCLE$     & $\CIRCLE$     & $\LEFTcircle$ & \standard     & $\LEFTcircle$ & \DCd. Shielding and Signal Slope Control                                                                                                                      & P                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & $\Circle$                                                                                \\
\begin{sideways}Integrity\end{sideways}       & \begin{sideways}Higher\end{sideways}     & \Ia. Fake Data Fabrication               & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\LEFTcircle$ & \DIb. Content Inspection                                                                                                                                      & D                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & \Ib. Memory and Firmware Manipulation    & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\CIRCLE$     & {\DIa. Diagnostic Session Authentication\\\DId. ECU Firmware Hardening}                                                                                                                                  & {P\\D,P}                                   & {$\CIRCLE$\\$\CIRCLE$}                                                                                        & {$\high$\\$\high$}                                                                                        & {$\high$\\$\high$}                                                                                           & {$\high$\\$\moderate$}                                                                                   & {$\CIRCLE$\\$\LEFTcircle$}                                                                            \\
                                              &                                          & \Ic. Bypassing Diagnostic Authentication & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\LEFTcircle$ &                                                                                              &                                 &                                                                        &                                                                        &                                                                                &                                                                        &                                                                \\
                                              &                                          & \Id. Session-Based Buffer Overflow       & $\Circle$     & $\Circle$     & $\Circle$     & \specific     & $\Circle$     & {\DIb. Content Inspection\\\DIc. Better Implementation Patching\\\DIk. ECU Guardian}                                                                                      & {~D,P*\\P\\P}                          & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                                    & {$\high$\\$\high$\\$\low$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\LEFTcircle$}                                                    \\
                                              & \begin{sideways}Controller\end{sideways} & \Ie. Impersonation and Replay            & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {\DIa. Per-ECU Authentication\\\DIa. Centralized Authentication\\\DIb. Content Inspection\\\DIF. Victim Resistance\\\DIh. Time IFS Anonymization\\\DIi. PIDS\\\DIj. Bit-Banger IDS\\\DIk. ECU Guardian} & {D,P\\D,P*\\D\\P\\D,P*\\D,P*\\D,P\\P} & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} & {$\low$\\$\moderate$\\$\high$\\$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$} & {$\moderate$\\$\moderate$\\$\high$\\$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$} & {$\high$\\$\high$\\$\high$\\$\moderate$\\$\high$\\$\high$\\$\high$\\$\low$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} \\
                                              &                                          & \Ij. Frame Tampering                & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & \DIi. VIDS                                                                                                                                & D                                     & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\high$                                                                                & $\CIRCLE$                                                                            \\
                                              &                                          & \Ii. Poly-semantic Frames~                    & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & \DIg. Unifying Sampling Points                                                                                                                                                         &  P                                      &    $\LEFTcircle$                                                                                              &  \high                                                                                                &   \high                                                                                                   &     \moderate                                                                                         &       $\LEFTcircle$                                                                                   \\
                                              &                                          & \Ig. Double Receive                      & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {\DIj. Bit-Banger IDS\\\DIk. ECU Guardian\DAe. Dynamic Fragmentation}                                                                                                   & {D,P*\\P\\P*}                          & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                                    & {$\high$\\$\low$\\$\low$}                                                            & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                \\
                                              &                                          & \Ik. Polyglot Frames                     & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & \Ih. Unorthodox Frames                   & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \standard     & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & \IF. Frame Hijacking                     & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {\DCc. ID Anonymization\\\DIh. Interframe-Spacing Anonymization}                                                                                                    & {P\\P}                                 & {$\LEFTcircle$\\$\LEFTcircle$}                                                                   & {$\high$\\$\moderate$}                                                                       & {$\high$\\$\moderate$}                                                                           & {$\high$\\$\high$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              & \begin{sideways}Transwire\end{sideways}  & \Il. Physical-Fingerprint Distortion     & $\Circle$     & ~$\Circle$    & ~$\Circle$    & \standard     & $\Circle$     & {\DCc. ID Anonymization\\\DIh. Interframe-Spacing Anonymization\\\DIj. Bit-Banger IDS}                                                                                   & {P\\D,P*\\P}                           & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$}                                                        & {$\high$\\$\moderate$\\$\high$}                                                            & {$\high$\\$\moderate$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & \IM. Physical Architecture Manipulation  & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & \standard     & $\CIRCLE$     & \DIi. PIDS (Locator)                                                                                                                                          & D                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\low$                                                                                    & $\CIRCLE$                                                                                \\
\begin{sideways}Availability\end{sideways}    & \begin{sideways}Higher\end{sideways}     & \Aa. ECU Functionality Disabling         & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\LEFTcircle$ & {\DIb. Content Inspection \\\DIc. Better Implementation  Patching\\\DIk. ECU Guardian}                                                                                    & {D\\P\\P}                              & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\high$\\$\high$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                                    & {$\high$\\$\high$\\$\low$}                                                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                \\
                                              &                                          & \Ab. Request Overwhelming       & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & \Ac. Higher-Layer Sybil Exhaustion               & $\Circle$     & $\Circle$     & $\Circle$     & \widespread & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & \Ae. Error State Manipulation            & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & \DAb. One-Shot Mode                                                                                                                                           & S                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\moderate$                                                                                        & $\high$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & \Ad. Error-Injection                     & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {\DCc. ID Anonymization\\\DIh. Interframe-Spacing Anonymization\\\DAc. Error Handling IDS}                                                                                & {P\\D,P\\D}                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\high$\\$\moderate$\\$\high$}                                                            & {$\high$\\$\moderate$\\$\high$}                                                                & {$\high$\\$\high$\\$\high$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\LEFTcircle$}                                                    \\
                                              &                                          & \Af. Bus Access Denial                   & $\Circle$     & $\Circle$     & $\Circle$     & \standard     & $\Circle$     & {\DAa. ID Priority Dissociation\\\DAd. Layer-II Node Suspension}                                              & {P\\P}                      & {$\LEFTcircle$\\$\LEFTcircle$}                              & {$\moderate$\\$\high$}                                      & {$\low$\\$\high$}                                              & {$\low$\\$\high$}                                      & {$\LEFTcircle$\\$\CIRCLE$}                              \\
                                              & & \Ag. Synchronization Disruption & $\LEFTcircle$ & $\Circle$ & $\Circle$ & \standard & $\Circle$ & {\DIj. Bit-Banger IDS\\\DIk. ECU Guardian\\\DAe. Dynamic Fragmentation} & {D\\P\\P*} & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$} & {$\high$\\$\high$\\$\high$} & {$\high$\\$\high$\\$\high$} & {$\high$\\$\low$\\$\low$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}  \\
                                              %&                                          &      &  &      &    &     &     & {\DIk. ECU Guardian\kha{??}\\\DAe. Dynamic Fragmentation}                                                                                                                                                         &  {P\\P*}                                        &  {$\LEFTcircle$\\$\CIRCLE$}                                                                                                    & {$\high$\\$\high$}                                                                                                 & 
                                              %{$\high$\\$\high$}                                                                                                    &   {$\low$\\$\low$}                                                       &             {$\CIRCLE$\\$\CIRCLE$}                                                                             \\
                                              & \begin{sideways}Transwire\end{sideways}  & \Ah. Signal Attenuation                  & $\LEFTcircle$ & $\Circle$     & $\Circle$     & \standard     & $\CIRCLE$     & \DIi. PIDS                                                                                                                                                    & D                                      & $\LEFTcircle$                                                                                    & $\high$                                                                                        & $\high$                                                                                            & $\high$                                                                                    & $\LEFTcircle$                                                                            \\
                                              &                                          & \Ai. Physical Vandalism                  & $\CIRCLE$     & $\Circle$     & $\CIRCLE$     & \standard     & $\CIRCLE$     & –                                                                                                                                                       & –                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        
\end{tblr}
}
\end{table*}

==> Tables/Collective_In_Progress.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.945,0.752,0.752}
\begin{table*}
\caption{Juxtaposition of CAN attack and defense categories along with their severity and efficacy assessments. \kha{vary gap colors}}
\centering
\label{tbl:bigtable}
\resizebox{\textwidth}{!}{
\footnotesize
\begin{tblr}{
  row{odd} = {c},
  row{2} = {c},
  row{4} = {c},
  row{6} = {c},
  row{8} = {c},
  row{12} = {c},
  row{14} = {c},
  row{16} = {c},
  row{18} = {c},
  row{20} = {c},
  row{22} = {c},
  row{24} = {BeautyBush,c},
  row{26} = {c},
  row{28} = {c},
  row{30} = {c},
  row{32} = {c},
  row{34} = {c},
  row{36} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=6}{},
  cell{1}{9} = {c=7}{},
  cell{3}{1} = {r=11}{},
  cell{3}{2} = {r=5}{},
  cell{3}{3} = {Matrix,fg=white},
  cell{3}{4} = {BeautyBush},
  cell{3}{5} = {BeautyBush},
  cell{3}{6} = {BeautyBush},
  cell{3}{7} = {BeautyBush},
  cell{3}{8} = {BeautyBush},
  cell{6}{9} = {r=2}{},
  cell{6}{10} = {r=2}{},
  cell{6}{11} = {r=2}{},
  cell{6}{12} = {r=2}{},
  cell{6}{13} = {r=2}{},
  cell{6}{14} = {r=2}{},
  cell{6}{15} = {r=2}{},
  cell{8}{2} = {r=3}{},
  cell{8}{3} = {BeautyBush},
  cell{8}{4} = {BeautyBush},
  cell{8}{5} = {BeautyBush},
  cell{8}{6} = {BeautyBush},
  cell{8}{7} = {BeautyBush},
  cell{8}{8} = {BeautyBush},
  cell{10}{3} = {r=2}{c},
  cell{10}{4} = {r=2}{c},
  cell{10}{5} = {r=2}{c},
  cell{10}{6} = {r=2}{c},
  cell{10}{7} = {r=2}{c},
  cell{10}{8} = {r=2}{},
  cell{10}{9} = {r=3}{c},
  cell{10}{10} = {r=3}{c},
  cell{10}{11} = {r=3}{c},
  cell{10}{12} = {r=3}{c},
  cell{10}{13} = {r=3}{c},
  cell{10}{14} = {r=3}{c},
  cell{10}{15} = {r=3}{c},
  cell{11}{2} = {r=3}{},
  cell{14}{1} = {r=15}{},
  cell{14}{2} = {r=4}{},
  cell{14}{3} = {BeautyBush},
  cell{14}{4} = {BeautyBush},
  cell{14}{5} = {BeautyBush},
  cell{14}{6} = {BeautyBush},
  cell{14}{7} = {BeautyBush},
  cell{14}{8} = {BeautyBush},
  cell{18}{2} = {r=9}{},
  cell{18}{3} = {BeautyBush},
  cell{18}{4} = {BeautyBush},
  cell{18}{5} = {BeautyBush},
  cell{18}{6} = {BeautyBush},
  cell{18}{7} = {BeautyBush},
  cell{18}{8} = {BeautyBush},
  cell{19}{9} = {r=2}{},
  cell{19}{10} = {r=2}{},
  cell{19}{11} = {r=2}{},
  cell{19}{12} = {r=2}{},
  cell{19}{13} = {r=2}{},
  cell{19}{14} = {r=2}{},
  cell{19}{15} = {r=2}{},
  cell{21}{3} = {Matrix,fg=white},
  cell{21}{4} = {BeautyBush},
  cell{21}{5} = {BeautyBush},
  cell{21}{6} = {BeautyBush},
  cell{21}{7} = {BeautyBush},
  cell{21}{8} = {BeautyBush},
  cell{21}{9} = {r=4}{},
  cell{21}{10} = {r=4}{},
  cell{21}{11} = {r=4}{},
  cell{21}{12} = {r=4}{},
  cell{21}{13} = {r=4}{},
  cell{21}{14} = {r=4}{},
  cell{21}{15} = {r=4}{},
  cell{25}{3} = {BeautyBush},
  cell{25}{4} = {BeautyBush},
  cell{25}{5} = {BeautyBush},
  cell{25}{6} = {BeautyBush},
  cell{25}{7} = {BeautyBush},
  cell{25}{8} = {BeautyBush},
  cell{27}{2} = {r=2}{},
  cell{27}{3} = {BeautyBush},
  cell{27}{4} = {BeautyBush},
  cell{27}{5} = {BeautyBush},
  cell{27}{6} = {BeautyBush},
  cell{27}{7} = {BeautyBush},
  cell{27}{8} = {BeautyBush},
  cell{29}{1} = {r=8}{},
  cell{29}{2} = {r=3}{},
  cell{29}{9} = {r=3}{},
  cell{29}{10} = {r=3}{},
  cell{29}{11} = {r=3}{},
  cell{29}{12} = {r=3}{},
  cell{29}{13} = {r=3}{},
  cell{29}{14} = {r=3}{},
  cell{29}{15} = {r=3}{},
  cell{32}{2} = {r=3}{},
  cell{32}{3} = {Matrix,fg=white},
  cell{32}{4} = {BeautyBush},
  cell{32}{5} = {BeautyBush},
  cell{32}{6} = {BeautyBush},
  cell{32}{7} = {BeautyBush},
  cell{32}{8} = {BeautyBush},
  cell{33}{3} = {Matrix,fg=white},
  cell{33}{4} = {BeautyBush},
  cell{33}{5} = {BeautyBush},
  cell{33}{6} = {BeautyBush},
  cell{33}{7} = {BeautyBush},
  cell{33}{8} = {BeautyBush},
  cell{34}{3} = {Matrix,fg=white},
  cell{34}{4} = {BeautyBush},
  cell{34}{5} = {BeautyBush},
  cell{34}{6} = {BeautyBush},
  cell{34}{7} = {BeautyBush},
  cell{34}{8} = {BeautyBush},
  cell{34}{9} = {r=2}{},
  cell{34}{10} = {r=2}{},
  cell{34}{11} = {r=2}{},
  cell{34}{12} = {r=2}{},
  cell{34}{13} = {r=2}{},
  cell{34}{14} = {r=2}{},
  cell{34}{15} = {r=2}{},
  cell{35}{2} = {r=2}{},
  cell{35}{3} = {Matrix,fg=white},
  cell{35}{4} = {BeautyBush},
  cell{35}{5} = {BeautyBush},
  cell{35}{6} = {BeautyBush},
  cell{35}{7} = {BeautyBush},
  cell{35}{8} = {BeautyBush},
  vlines,
  hline{1,3,14,29,37} = {-}{},
  hline{2,5-6,9-10,13,15,17,19,26,28} = {3-15}{},
  hline{4,7,12,16,20-25,30-31,33-34,36} = {3-8}{},
  hline{4,25,27,36} = {9-15}{dashed},
  hline{8,18,32} = {2-15}{},
  hline{11} = {2}{},
  hline{16,21,33-34} = {9-15}{dotted},
  hline{27,35} = {2-8}{},
}
\begin{sideways}Component\end{sideways}       & \begin{sideways}Layer\end{sideways}      & Attack                              &                                       &                                        &                                      &                                          &                                          & Defense                                                                                                                              &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Category                            & \begin{sideways}Ability\end{sideways} & \begin{sideways}Hardware\end{sideways} & \begin{sideways}Access\end{sideways} & \begin{sideways}Prevalence\end{sideways} & \begin{sideways}Complexity\end{sideways} & Category                                                                                                                             & \begin{sideways}Protection\end{sideways} & \begin{sideways}Coverage\end{sideways}                                                                                                                                       & \begin{sideways}ECU Impact\end{sideways}                                                                                                                                         & \begin{sideways}Bus Impact\end{sideways}                                                                                                                                             & \begin{sideways}Infrastructure\end{sideways}                                                                                                                                 & \begin{sideways}Validity\end{sideways}                                                                                                                                   \\
\begin{sideways}Confidentiality\end{sideways} & \begin{sideways}Higher\end{sideways}     & \hyperref[subsubsec:reveng]{Communication Surveillance}          & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\LEFTcircle$               & Message Obfuscation                                                                                                                  & P                                        & $\LEFTcircle$                                                                                                                                                   & $\CIRCLE$                                                                                                                                                           & $\CIRCLE$                                                                                                                                                               & $\Circle$                                                                                                                                                       & $\CIRCLE$                                                                                                                                                   \\
                                              &                                          & Privacy Leakage                     & $\Circle$                & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               & Privacy-preserving Transformations (remove)                                                                                                  & P                                        & $\LEFTcircle$                                                                                                                                                   & –                                                                                                                                                                                & –                                                                                                                                                                                    & $\Circle$                                                                                                                                                       & $\Circle$                                                                                                                                                   \\
                                              &                                          & Sensitive Information Sniffing      & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\LEFTcircle$               & {Better Implementation \& Patching\\Message Obfuscation}                                                                                & {P\\P}                                   & {$\CIRCLE$\\$\CIRCLE$}                                                                                                                             & {$\Circle$\\$\Circle$}                                                                                                                                 & {$\Circle$\\$\Circle$}                                                                                                                                     & {$\Circle$\\$\Circle$}                                                                                                                             & {$\CIRCLE$\\$\CIRCLE$}                                                                                                                         \\
                                              &                                          & Memory Leakage                      & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\Circle$                   & {Memory and Firmware Concealment\\Better Implementation \& Patching\\Diagnostic Session Authentication (remove?will you put auth at ll?)}                                 & {P\\P\\P}                                & {$\CIRCLE$\\$\CIRCLE$\\$\LEFTcircle$}                                                                                                 & {$\LEFTcircle$\\$\Circle$\\$\Circle$}                                                                                                     & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                             & {$\LEFTcircle$\\$\Circle$\\$\Circle$}                                                                                                 & {$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$}                                                                                             \\
                                              &                                          & Information and Firmware Dump       & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\CIRCLE$                   &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error-Based Reconnaissance          & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {One-Shot Mode\\lnterframe-Spacing Anonymization\\ID Anonymization}                                            & {P\\P\\P}                                & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                                                             & {$\Circle$\\$\LEFTcircle$\\$\Circle$}                                                                                                     & {$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$}                                                                                                     & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                     & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                                                 \\
                                              &                                          & Clock-Skew Network Mapping          & $\Circle$                & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               & Skew Cloaking                                                                                                                        & P                                        & $\CIRCLE$                                                                                                                                                       & $\LEFTcircle$                                                                                                                                                       & $\Circle$                                                                                                                                                               & $\Circle$                                                                                                                                                       & $\CIRCLE$                                                                                                                                                   \\
                                              &                                          & Signal and Hardware Profiling       & $\CIRCLE$                & $\CIRCLE$                 & $\LEFTcircle$           & $\CIRCLE$                   & $\LEFTcircle$               & –                                                                                                                                    & –                                        & –                                                                                                                                                                            & –                                                                                                                                                                                & –                                                                                                                                                                                    & –                                                                                                                                                                            & –                                                                                                                                                                        \\
                                              & \begin{sideways}Transwire\end{sideways}  &                                     &                                       &                                        &                                      &                                          &                                          &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Topology Intelligence             & $\CIRCLE$                & $\CIRCLE$                 & $\CIRCLE$               & $\CIRCLE$                   & $\LEFTcircle$               &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Electromagnetic Emissions           & $\CIRCLE$                & $\CIRCLE$                 & $\LEFTcircle$           & $\CIRCLE$                   & $\LEFTcircle$               & Shielding and Signal Slope Control                                                                                                   & P                                        & –                                                                                                                                                                            & –                                                                                                                                                                                & –                                                                                                                                                                                    & –                                                                                                                                                                            & $\Circle$                                                                                                                                                   \\
\begin{sideways}Integrity\end{sideways}       & \begin{sideways}Higher\end{sideways}     & Fake Data Fabrication  (Gapify)             & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\LEFTcircle$               & Content Inspection                                                                                                                   & D,P*                                     & $\LEFTcircle$                                                                                                                                                       & $\Circle$                                                                                                                                                           & $\Circle$                                                                                                                                                               & $\Circle$                                                                                                                                                       & $\CIRCLE$                                                                                                                                                   \\
                                              &                                          &   Memory and Firmware Manipulation    & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\CIRCLE$                   & Firmware Attestation                                                                                                                 & D,P                                      & $\CIRCLE$                                                                                                                                                       & $\Circle$                                                                                                                                                           & $\Circle$                                                                                                                                                               & $\CIRCLE$                                                                                                                                                       & $\LEFTcircle$                                                                                                                                               \\
                                              &                                          & Bypassing Diagnostic Authentication & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\LEFTcircle$               & {Diagnostic Session Authentication\\ECU Hardening (Change)}                                                                                   & {P\\P}                                   & {$\CIRCLE$\\$\LEFTcircle$}                                                                                                                         & {$\Circle$\\$\LEFTcircle$}                                                                                                                             & {$\Circle$\\$\Circle$}                                                                                                                                     & {$\Circle$\\$\CIRCLE$}                                                                                                                             & {$\CIRCLE$\\$\LEFTcircle$}                                                                                                                     \\
                                              &                                          & Session-Based Buffer Overflow       & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\Circle$                   & {Content Inspection (move below?)\\ECU Guardian (Review Coverage?)\\Better Implementation \& Patching (Review Validation?}                                                                   & {D\\P\\P}                                & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                                                                                                 & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                         & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                             & {$\Circle$\\$\CIRCLE$\\$\Circle$}                                                                                                     & {$\CIRCLE$\\$\LEFTcircle$\\$\Circle$}                                                                                             \\
                                              & \begin{sideways}Controller\end{sideways} & Impersonation and Replay            & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {PIDS\\Per-ECU Authentication\\Centralized Authentication (fit criterea)\\Time  IFS Anonymization\\Bit-Banger IDS\\Victim Resistance\\ECU Guardian} & {D,P*\\D,P\\D,P*\\D,P*\\D,P*\\P\\P}       & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} & {$\Circle$\\$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$} & {$\Circle$\\$\LEFTcircle$\\$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$} & {$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\LEFTcircle$\\$\CIRCLE$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} \\
                                              &                                          & Poly-semantic Frames                & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               & {Unifying Sampling Points\\PIDS(remove?)}                                                                                                     & {P\\D,P*}                                & {$\LEFTcircle$\\–}                                                                                                                                              & {$\Circle$\\$\Circle$}                                                                                                                                 & {$\Circle$\\$\Circle$}                                                                                                                                     & {$\LEFTcircle$\\$\Circle$}                                                                                                                         & {$\LEFTcircle$\\$\Circle$}                                                                                                                     \\
                                              &                                          & Frame Tampering (two tamper)                     & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Double Receive                      & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {ECU Guardian\\~Bit-Banger IDS\\Dynamic Fragmentation}                                                                               & {P\\D,P*\\P*}                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                                                             & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                         & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                             & {$\CIRCLE$\\$\Circle$\\$\CIRCLE$}                                                                                                     & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$}                                                                                         \\
                                              &                                          & Polyglot Frames                     & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Frame Tampering                     & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Unorthodox Frames                   & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Frame Hijacking                     & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {ID Anonymization\\Interframe-Spacing Anonymization}                                                                                 & {P\\P}                                   & {$\LEFTcircle$\\$\LEFTcircle$}                                                                                                                     & {$\Circle$\\$\LEFTcircle$}                                                                                                                             & {$\Circle$\\$\LEFTcircle$}                                                                                                                                 & {$\Circle$\\$\Circle$}                                                                                                                             & {$\CIRCLE$\\$\CIRCLE$}                                                                                                                         \\
                                              &                                          & Clock-Skew Spoofing  (remove)               & $\Circle$                & $\Circle$                 & $\Circle$               & $\Circle$                   & $\LEFTcircle$               & {Other PIDS (remove)\\Bit-Banger IDS}                                                                                                         & {D,P*\\D,P*}                             & {$\CIRCLE$\\$\CIRCLE$}                                                                                                                             & {$\Circle$\\$\Circle$}                                                                                                                                 & {$\Circle$\\$\Circle$}                                                                                                                                     & {$\Circle$\\$\Circle$}                                                                                                                             & {$\CIRCLE$\\$\CIRCLE$}                                                                                                                         \\
                                              & \begin{sideways}Transwire\end{sideways}  & Physical-Fingerprint Distortion     & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {ID Anonymization\\Interframe-Spacing Anonymization}                                                                                 & {P\\P}                                   & {$\LEFTcircle$\\$\LEFTcircle$}                                                                                                                     & {$\Circle$\\$\LEFTcircle$}                                                                                                                             & {$\Circle$\\$\LEFTcircle$}                                                                                                                                 & {$\Circle$\\$\Circle$}                                                                                                                             & {$\CIRCLE$\\$\CIRCLE$}                                                                                                                         \\
                                              &                                          & Physical Architecture Manipulation  & $\CIRCLE$                & $\CIRCLE$                 & $\CIRCLE$               & $\CIRCLE$                   & $\Circle$                   & PIDS (Locator)                                                                                                                       & D                                        & $\LEFTcircle$                                                                                                                                                   & $\Circle$                                                                                                                                                           & $\Circle$                                                                                                                                                               & $\CIRCLE$                                                                                                                                                       & $\CIRCLE$                                                                                                                                                   \\
\begin{sideways}Availability\end{sideways}    & \begin{sideways}Higher\end{sideways}     & ECU Functionality Disabling         & $\Circle$                & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\LEFTcircle$               & {Better Implementation \& Patching\\Content Inspection \\ECU Guardian}                                                                  & {P\\D\\P}                                & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                                                     & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                         & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                             & {$\Circle$\\$\Circle$\\$\CIRCLE$}                                                                                                     & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                                                         \\
                                              &                                          & Higher-Layer Sybil Exhaustion       & $\Circle$                & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\Circle$                   &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Request Overwhelming                & $\Circle$                & $\Circle$                 & $\Circle$               & $\LEFTcircle$               & $\Circle$                   &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error State Manipulation            & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & One-Shot Mode                                                                                                  & S                                        & $\LEFTcircle$                                                                                                                                                   & $\Circle$                                                                                                                                                           & $\LEFTcircle$                                                                                                                                                           & $\Circle$                                                                                                                                                       & $\CIRCLE$                                                                                                                                                   \\
                                              &                                          & Error-Injection                     & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {Error Handling IDS\\ID Anonymization\\Interframe-Spacing Anonymization}                                                             & {D\\P\\D,P}                              & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                                                             & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                                                                     & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                                                                         & {$\Circle$\\$\Circle$\\$\Circle$}                                                                                                     & {$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$}                                                                                             \\
                                              &                                          & Bus Access Denial                   & $\Circle$                & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   & {Layer-II Node Suspension\\ID Priority Dissociation\\Dynamic Fragmentation \\ECU Guardian\\Bit-Banger IDS}                           & {P\\P\\P*\\P\\D}                         & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                        & {$\Circle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$}                                                     & {$\Circle$\\$\CIRCLE$\\$\Circle$\\$\Circle$\\$\Circle$}                                            & {$\Circle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\Circle$}                                                     & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                             \\
                                              & \begin{sideways}Transwire\end{sideways}  & Synchronization Disruption          & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\Circle$                   &                                                                                                                                      &                                          &                                                                                                                                                                              &                                                                                                                                                                                  &                                                                                                                                                                                      &                                                                                                                                                                              &                                                                                                                                                                          \\
                                              &                                          & Signal Attenuation  (vandal?)                & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\CIRCLE$                & PIDS                                                                                                                                 & D                                        & $\LEFTcircle$                                                                                                                                                   & $\Circle$                                                                                                                                                           & $\Circle$                                                                                                                                                               & $\Circle$                                                                                                                                                       & $\LEFTcircle$      \\
                                              &                                          & Physical Vandalism                & $\LEFTcircle$            & $\Circle$                 & $\Circle$               & $\CIRCLE$                   & $\CIRCLE$  & --                                                                                                                                 & --                                        & --                                                                                                                                                   & --                                                                                                                                                           & --                                                                                                                                                               & --                                                                                                                                                       & --                                                                                                                                       
\end{tblr}
}
\end{table*}

==> Tables/Collective_S.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{1,0.9,0.86}
\definecolor{BurntOrange}{rgb}{0.5,0.5,0.5}
\definecolor{Manhattan}{rgb}{0.854,0.854,0.854}
% \definecolor{BurntOrange}{rgb}{0.807,0.298,0}
% \definecolor{Manhattan}{rgb}{0.945,0.733,0.611}
% \definecolor{Alto}{rgb}{0.854,0.854,0.854}
% \definecolor{SilverChalice}{rgb}{0.678,0.678,0.678}
%\definecolor{BeautyBush}{rgb}{0.945,0.752,0.752}
%try this pink {1,0.9,0.86}
\begin{table*}
\centering
\caption{Juxtaposing each CAN attack category against possible defense categories with severity and efficacy assessments}
\label{tbl:bigtable}
\resizebox*{0.96\textwidth}{0.96\textheight}{
% \setlength\extrarowheight{-5pt}
\small
\begin{tblr}{
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  row{5} = {c},
  row{6} = {c},
  row{7} = {c},
  row{8} = {c},
  row{9} = {c},
  row{11} = {c},
  row{12} = {c},
  row{13} = {c},
  row{14} = {c},
  row{15} = {c},
  row{16} = {c},
  row{17} = {c},
  row{18} = {c},
  row{19} = {c},
  row{20} = {c},
  row{21} = {c},
  row{22} = {c},
  row{23} = {Manhattan,c},
  row{24} = {c},
  row{26} = {c},
  row{27} = {c},
  row{28} = {c},
  row{29} = {c},
  row{30} = {c},
  row{31} = {c},
  row{32} = {c},
  row{33} = {Manhattan,c},
  row{35} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=6}{},
  cell{1}{9} = {c=7}{},
  cell{3}{1} = {r=11}{},
  cell{3}{2} = {r=5}{},
  cell{3}{3} = {Matrix,fg=white},
  cell{3}{4} = {BeautyBush},
  cell{3}{5} = {BeautyBush},
  cell{3}{6} = {BeautyBush},
  cell{3}{7} = {BeautyBush},
  cell{3}{8} = {BeautyBush},
  cell{3}{9} = {r=2}{},
  cell{3}{10} = {r=2}{},
  cell{3}{11} = {r=2}{},
  cell{3}{12} = {r=2}{},
  cell{3}{13} = {r=2}{},
  cell{3}{14} = {r=2}{},
  cell{3}{15} = {r=2}{},
  cell{6}{9} = {r=2}{},
  cell{6}{10} = {r=2}{},
  cell{6}{11} = {r=2}{},
  cell{6}{12} = {r=2}{},
  cell{6}{13} = {r=2}{},
  cell{6}{14} = {r=2}{},
  cell{6}{15} = {r=2}{},
  cell{8}{2} = {r=3}{},
  cell{8}{3} = {BeautyBush},
  cell{8}{4} = {BeautyBush},
  cell{8}{5} = {BeautyBush},
  cell{8}{6} = {BeautyBush},
  cell{8}{7} = {BeautyBush},
  cell{8}{8} = {BeautyBush},
  cell{10}{3} = {r=2}{c},
  cell{10}{4} = {r=2}{c},
  cell{10}{5} = {r=2}{c},
  cell{10}{6} = {r=2}{c},
  cell{10}{7} = {r=2}{c},
  cell{10}{8} = {r=2}{},
  cell{10}{9} = {r=3}{c},
  cell{10}{10} = {r=3}{c},
  cell{10}{11} = {r=3}{c},
  cell{10}{12} = {r=3}{c},
  cell{10}{13} = {r=3}{c},
  cell{10}{14} = {r=3}{c},
  cell{10}{15} = {r=3}{c},
  cell{11}{2} = {r=3}{},
  cell{14}{1} = {r=13}{},
  cell{14}{2} = {r=4}{},
  cell{14}{3} = {Matrix,fg=white},
  cell{14}{4} = {BeautyBush},
  cell{14}{5} = {BeautyBush},
  cell{14}{6} = {BeautyBush},
  cell{14}{7} = {BeautyBush},
  cell{14}{8} = {BeautyBush},
  cell{18}{2} = {r=7}{},
  cell{18}{3} = {BeautyBush},
  cell{18}{4} = {BeautyBush},
  cell{18}{5} = {BeautyBush},
  cell{18}{6} = {BeautyBush},
  cell{18}{7} = {BeautyBush},
  cell{18}{8} = {BeautyBush},
  cell{19}{9} = {r=2}{},
  cell{19}{10} = {r=2}{},
  cell{19}{11} = {r=2}{},
  cell{19}{12} = {r=2}{},
  cell{19}{13} = {r=2}{},
  cell{19}{14} = {r=2}{},
  cell{19}{15} = {r=2}{},
  cell{21}{3} = {BurntOrange,fg=white},
  cell{21}{4} = {Manhattan},
  cell{21}{5} = {Manhattan},
  cell{21}{6} = {Manhattan},
  cell{21}{7} = {Manhattan},
  cell{21}{8} = {Manhattan},
  cell{21}{9} = {r=3}{},
  cell{21}{10} = {r=3}{},
  cell{21}{11} = {r=3}{},
  cell{21}{12} = {r=3}{},
  cell{21}{13} = {r=3}{},
  cell{21}{14} = {r=3}{},
  cell{21}{15} = {r=3}{},
  cell{24}{3} = {BeautyBush},
  cell{24}{4} = {BeautyBush},
  cell{24}{5} = {BeautyBush},
  cell{24}{6} = {BeautyBush},
  cell{24}{7} = {BeautyBush},
  cell{24}{8} = {BeautyBush},
  cell{25}{2} = {r=2}{},
  cell{25}{3} = {BeautyBush,c},
  cell{25}{4} = {BeautyBush,c},
  cell{25}{5} = {BeautyBush,c},
  cell{25}{6} = {BeautyBush,c},
  cell{25}{7} = {BeautyBush,c},
  cell{25}{8} = {BeautyBush,c},
  cell{25}{9} = {c},
  cell{25}{10} = {c},
  cell{25}{11} = {c},
  cell{25}{12} = {c},
  cell{25}{13} = {c},
  cell{25}{14} = {c},
  cell{25}{15} = {c},
  cell{27}{1} = {r=9}{},
  cell{27}{2} = {r=3}{},
  cell{27}{9} = {r=3}{},
  cell{27}{10} = {r=3}{},
  cell{27}{11} = {r=3}{},
  cell{27}{12} = {r=3}{},
  cell{27}{13} = {r=3}{},
  cell{27}{14} = {r=3}{},
  cell{27}{15} = {r=3}{},
  cell{30}{2} = {r=4}{},
  cell{30}{3} = {BurntOrange,fg=white},
  cell{30}{4} = {BeautyBush},
  cell{30}{5} = {BeautyBush},
  cell{30}{6} = {BeautyBush},
  cell{30}{7} = {BeautyBush},
  cell{30}{8} = {BeautyBush},
  cell{31}{3} = {BurntOrange,fg=white},
  cell{31}{4} = {BeautyBush},
  cell{31}{5} = {BeautyBush},
  cell{31}{6} = {BeautyBush},
  cell{31}{7} = {BeautyBush},
  cell{31}{8} = {BeautyBush},
  cell{32}{3} = {BurntOrange,fg=white},
  cell{32}{4} = {BeautyBush},
  cell{32}{5} = {BeautyBush},
  cell{32}{6} = {BeautyBush},
  cell{32}{7} = {BeautyBush},
  cell{32}{8} = {BeautyBush},
  cell{32}{9} = {r=2}{},
  cell{32}{10} = {r=2}{},
  cell{32}{11} = {r=2}{},
  cell{32}{12} = {r=2}{},
  cell{32}{13} = {r=2}{},
  cell{32}{14} = {r=2}{},
  cell{32}{15} = {r=2}{},
  cell{33}{3} = {BurntOrange,fg=white},
  cell{34}{2} = {r=2}{},
  cell{34}{3} = {c},
  cell{34}{4} = {c},
  cell{34}{5} = {c},
  cell{34}{6} = {c},
  cell{34}{7} = {c},
  cell{34}{8} = {c},
  cell{34}{9} = {c},
  cell{34}{10} = {c},
  cell{34}{11} = {c},
  cell{34}{12} = {c},
  cell{34}{13} = {c},
  cell{34}{14} = {c},
  cell{34}{15} = {c},
  vlines,
  vline{4} = {4}{dotted},
  hline{1,3,14,27,36} = {-}{},
  hline{2,5-6,9-10,13,15,17,19,26,35} = {3-15}{},
  hline{4,7,16,20-24,28-29,31-33} = {3-8}{},
  hline{8,18,25,30} = {2-15}{},
  hline{11} = {2}{},
  hline{16,21,31-32} = {9-15}{dotted},
  hline{24,34} = {9-15}{dashed},
  hline{34} = {2-8}{},
}
\begin{sideways}\end{sideways}                & \begin{sideways}Layer\end{sideways}      & Attack                              &               &               &               &               &               & Defense                                                                                                                                                 &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Category                            & $\mathcal{B}$ & $\mathcal{Q}$ & $\mathcal{X}$ & $\mathcal{V}$ & $\mathcal{D}$ & Category                                                                                                                                                & $\mathcal{I}$                          & $\Lambda$                                                                                        & $\mathcal{E}$                                                                                    & $\beta$                                                                                              & $\mathcal{F}$                                                                                & $\vartheta$                                                                              \\
\begin{sideways}Confidentiality\end{sideways} & \begin{sideways}Higher\end{sideways}     & Communication Surveillance          & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\LEFTcircle$ & Message Obfuscation                                                                                                                                     & P                                      & $\LEFTcircle$                                                                                    & $\CIRCLE$                                                                                        & $\CIRCLE$                                                                                            & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Privacy Leakage                     & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Sensitive Information Sniffing      & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & {Better Implementation \&  Patching\\Message Obfuscation}                                                                                                  & {P\\P}                                 & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\Circle$\\$\Circle$}                                                                           & {$\Circle$\\$\Circle$}                                                                               & {$\Circle$\\$\Circle$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              &                                          & Memory Leakage                      & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & {Memory and Firmware Concealment\\Better Implementation Patching}                                                                                       & {P\\P}                                 & {$\CIRCLE$\\$\CIRCLE$}                                                                           & {$\LEFTcircle$\\$\Circle$}                                                                       & {$\Circle$\\$\Circle$}                                                                               & {$\LEFTcircle$\\$\Circle$}                                                                   & {$\LEFTcircle$\\$\CIRCLE$}                                                               \\
                                              &                                          & Information and Firmware Dump       & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error-Based Reconnaissance          & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & {One-Shot Mode\\lnterframe-Spacing Anonymization\\ID Anonymization}                                                                                     & {P\\P\\P}                              & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\Circle$\\$\LEFTcircle$\\$\Circle$}                                                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$}                                                            & {$\Circle$\\$\Circle$\\$\Circle$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & Clock-Skew Network Mapping          & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\LEFTcircle$ & Skew Cloaking                                                                                                                                           & P                                      & $\CIRCLE$                                                                                        & $\LEFTcircle$                                                                                    & $\Circle$                                                                                            & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Signal and Hardware Profiling       & $\CIRCLE$     & $\CIRCLE$     & $\LEFTcircle$ & $\CIRCLE$     & $\LEFTcircle$ & –                                                                                                                                                       & –                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        \\
                                              & \begin{sideways}Transwire\end{sideways}  &                                     &               &               &               &               &               &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Topology Intelligence               & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Electromagnetic Emissions           & $\CIRCLE$     & $\CIRCLE$     & $\LEFTcircle$ & $\CIRCLE$     & $\LEFTcircle$ & Shielding and Signal Slope Control                                                                                                                      & P                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & $\Circle$                                                                                \\
\begin{sideways}Integrity\end{sideways}       & \begin{sideways}Higher\end{sideways}     & Fake Data Fabrication               & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\LEFTcircle$ & Content Inspection                                                                                                                                      & D                                      & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Memory and Firmware Manipulation    & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & Firmware Attestation                                                                                                                                    & D,P                                    & $\CIRCLE$                                                                                        & $\Circle$                                                                                        & $\Circle$                                                                                            & $\CIRCLE$                                                                                    & $\LEFTcircle$                                                                            \\
                                              &                                          & Bypassing Diagnostic Authentication & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & {Diagnostic Session Authentication\\Control Flow Integrity}                                                                                             & {P\\P}                                 & {$\CIRCLE$\\$\LEFTcircle$}                                                                       & {$\Circle$\\$\LEFTcircle$}                                                                       & {$\Circle$\\$\Circle$}                                                                               & {$\Circle$\\$\CIRCLE$}                                                                       & {$\CIRCLE$\\$\LEFTcircle$}                                                               \\
                                              &                                          & Session-Based Buffer Overflow       & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & $\Circle$     & {Better Implementation Patching\\ECU Guardian\\Content Inspection}                                                                                      & {P\\P\\~D,P*}                          & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                    & {$\Circle$\\$\CIRCLE$\\$\Circle$}                                                            & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                                                    \\
                                              & \begin{sideways}Controller\end{sideways} & Impersonation and Replay            & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & {Content Inspection\\PIDS\\Per-ECU Authentication\\Centralized Authentication\\Time IFS Anonymization\\Bit-Banger IDS\\Victim Resistance\\ECU Guardian} & {D\\D,P*\\D,P\\D,P*\\D,P*\\D,P*\\P\\P} & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} & {$\Circle$\\$\Circle$\\$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$} & {$\Circle$\\$\Circle$\\$\LEFTcircle$\\$\LEFTcircle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$} & {$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\Circle$\\$\LEFTcircle$\\$\CIRCLE$} & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$} \\
                                              &                                          & Poly-semantic Frames                & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\LEFTcircle$ & Unifying Sampling Points                                                                                                                                & P                                      & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\LEFTcircle$                                                                                & $\LEFTcircle$                                                                            \\
                                              &                                          & Frame Tampering~                    & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Double Receive                      & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & {ECU Guardian\\Bit-Banger IDS\\Dynamic Fragmentation}                                                                                                   & {P\\D,P*\\P*}                          & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                        & {$\Circle$\\$\Circle$\\$\Circle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                    & {$\CIRCLE$\\$\Circle$\\$\CIRCLE$}                                                            & {$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$}                                                \\
                                              &                                          & Polyglot Frames                     & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\LEFTcircle$ &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Unorthodox Frames                   & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Frame Hijacking                     & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & {ID Anonymization\\Interframe-Spacing Anonymization}                                                                                                    & {P\\P}                                 & {$\LEFTcircle$\\$\LEFTcircle$}                                                                   & {$\Circle$\\$\LEFTcircle$}                                                                       & {$\Circle$\\$\LEFTcircle$}                                                                           & {$\Circle$\\$\Circle$}                                                                       & {$\CIRCLE$\\$\CIRCLE$}                                                                   \\
                                              & \begin{sideways}Transwire\end{sideways}  & Physical-Fingerprint Distortion     & $\Circle$     & ~$\Circle$    & ~$\Circle$    & $\CIRCLE$     & $\Circle$     & {Bit-Banger IDS \\ID Anonymization\\Interframe-Spacing Anonymization}                                                                                   & {D,P*\\P\\P}                           & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                            & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                            & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                        \\
                                              &                                          & Physical Architecture Manipulation  & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & $\CIRCLE$     & $\Circle$     & PIDS (Locator)                                                                                                                                          & D                                      & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\CIRCLE$                                                                                    & $\CIRCLE$                                                                                \\
\begin{sideways}Availability\end{sideways}    & \begin{sideways}Higher\end{sideways}     & ECU Functionality Disabling         & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\LEFTcircle$ & {Better Implementation  Patching\\Content Inspection \\ECU Guardian}                                                                                    & {P\\D\\P}                              & {$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                                    & {$\Circle$\\$\Circle$\\$\CIRCLE$}                                                            & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$}                                                \\
                                              &                                          & Higher-Layer Sybil Exhaustion       & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              &                                          & Request Overwhelming                & $\Circle$     & $\Circle$     & $\Circle$     & $\LEFTcircle$ & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Controller\end{sideways} & Error State Manipulation            & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & One-Shot Mode                                                                                                                                           & S                                      & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\LEFTcircle$                                                                                        & $\Circle$                                                                                    & $\CIRCLE$                                                                                \\
                                              &                                          & Error-Injection                     & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & {Error Handling IDS\\ID Anonymization\\Interframe-Spacing Anonymization}                                                                                & {D\\P\\D,P}                            & {$\CIRCLE$\\$\LEFTcircle$\\$\LEFTcircle$}                                                        & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                            & {$\Circle$\\$\Circle$\\$\LEFTcircle$}                                                                & {$\Circle$\\$\Circle$\\$\Circle$}                                                            & {$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$}                                                    \\
                                              &                                          & Bus Access Denial                   & $\Circle$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     & {Layer-II Node Suspension\\ID Priority Dissociation\\Dynamic Fragmentation \\ECU Guardian\\Bit-Banger IDS}                                              & {P\\P\\P*\\P\\D}                       & {$\LEFTcircle$\\$\LEFTcircle$\\$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$}                              & {$\Circle$\\$\LEFTcircle$\\$\Circle$\\$\Circle$\\$\Circle$}                                      & {$\Circle$\\$\CIRCLE$\\$\Circle$\\$\Circle$\\$\Circle$}                                              & {$\Circle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$\\$\Circle$}                                      & {$\CIRCLE$\\$\LEFTcircle$\\$\CIRCLE$\\$\CIRCLE$\\$\CIRCLE$}                              \\
                                              &                                          & Synchronization Disruption          & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\Circle$     &                                                                                                                                                         &                                        &                                                                                                  &                                                                                                  &                                                                                                      &                                                                                              &                                                                                          \\
                                              & \begin{sideways}Transwire\end{sideways}  & Signal Attenuation                  & $\LEFTcircle$ & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\CIRCLE$     & PIDS                                                                                                                                                    & D                                      & $\LEFTcircle$                                                                                    & $\Circle$                                                                                        & $\Circle$                                                                                            & $\Circle$                                                                                    & $\LEFTcircle$                                                                            \\
                                              &                                          & Physical Vandalism                  & $\CIRCLE$     & $\Circle$     & $\Circle$     & $\CIRCLE$     & $\CIRCLE$     & –                                                                                                                                                       & –                                      & –                                                                                                & –                                                                                                & –                                                                                                    & –                                                                                            & –                                                                                        
\end{tblr}
}
\end{table*}

==> Tables/IVB_RootCause.tex <==
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{1,0.9,0.86}
\definecolor{BurntOrange}{rgb}{0.5,0.5,0.5}
\definecolor{Manhattan}{rgb}{0.854,0.854,0.854}

\begin{table}[t]
\caption{Root causes for CAN attacks. \kha{Appearance + Error Inject and manip do not have R3}} 
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
      %& R1: Attacker Access      & R2: Shared Media        & R3: Exploitable Priority  & R4: Error Handling        & R5: Layer-II            & R6: Vulnerable Higher-Layer & R7: Physical Layer       & DR1: Cryptography        & DR2: Costly Attacker Signal & DR3: Difficult Environment \\
      %& to Network (I)           & Properties (I)          & System (I)                & Properties (IU)           & Rule Violation          & Protocols                   & Properties (IU)          & Challenges  (I)             & Filtering and Disabling (I)     & Understanding              \\
%& \begin{sideways}$\mathcal{R}$1 (I) \end{sideways}& \begin{sideways}$\mathcal{R}$2\end{sideways} & \begin{sideways}$\mathcal{R}3$\end{sideways} (I) & \begin{sideways}$\mathcal{R}$4\end{sideways} (I) & \begin{sideways}$\mathcal{R}$5\end{sideways} (IU) & \begin{sideways}$\mathcal{R}$6\end{sideways} & \begin{sideways}$\mathcal{R}$7\end{sideways} & \begin{sideways}$\mathcal{R}$8 (IU)\end{sideways} & \begin{sideways}$\mathcal{DR}$1 (I)\end{sideways} & \begin{sideways}$\mathcal{DR}$2 (I\end{sideways}) & \begin{sideways}$\mathcal{DR}$3\end{sideways}  \\
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R1\,(I)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R2\,(I)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R3\,(I)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R4\,(IU)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R5\,(I)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R6\,(IU)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R7$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R8$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal R9$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal{DR}1\,(I)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal{DR}2\,(I)$}}}
& {\rotatebox{90}{\parbox[b]{3.5em}{\raggedright$\mathcal{DR}3$}}}
\\
    \hline\hline
CAN FD &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE & \LEFTcircle &\CIRCLE &\CIRCLE \\
\hline
CAN XL (Err. On) &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE & \LEFTcircle &\CIRCLE &\CIRCLE \\
\hline
CAN XL (Err. Off) &\CIRCLE &\CIRCLE &\CIRCLE &\LEFTcircle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE & \LEFTcircle &\CIRCLE &\CIRCLE \\
\hline
10BASE-T1S &\CIRCLE &\CIRCLE &\CIRCLE &\Circle &\CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE & \LEFTcircle &\CIRCLE &\CIRCLE \\
\hline
  \end{tabular}}
\end{table}


==> Tables/MySun.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Mercury}{rgb}{0.901,0.901,0.901}
\definecolor{SilverChalice}{rgb}{0.678,0.678,0.678}
\begin{table}[]
\centering
\caption{What attacks each attacker model can launch \kha{fix X and Q}}
\label{tbl:mapping}

\resizebox*{\columnwidth}{!}{
%0.5\textheight
\begin{tblr}{
  cells = {c},
  row{9} = {Mercury},
  row{10} = {Mercury},
  row{11} = {Mercury},
  row{12} = {SilverChalice},
  row{13} = {SilverChalice},
  cell{1}{1} = {c=3}{},
  cell{2}{1} = {r=12}{},
  cell{2}{2} = {r=10}{},
  cell{2}{3} = {r=7}{},
  cell{2}{4} = {r=7}{},
  cell{2}{5} = {r=2}{},
  cell{4}{5} = {r=2}{},
  cell{6}{5} = {r=3}{},
  cell{9}{3} = {r=3}{},
  cell{9}{4} = {r=3}{},
  cell{9}{5} = {r=2}{},
  cell{12}{2} = {c=2,r=2}{},
  vlines,
  hline{1-2,14} = {-}{},
  hline{3,5,7-8,10} = {6-7}{},
  hline{4,6,11} = {5-7}{},
  hline{9} = {3-7}{},
  hline{12} = {2-7}{},
  hline{13} = {4-7}{},
}
Ability ($\mathcal{B}$)                     &                                                  &                                                               & $\mathcal{X}$                                    & $\mathcal{V}$                       & $\mathcal{D}$                               & Attack Category                                                                                                                                                                                    \\
\begin{sideways}Down to earth\end{sideways} & \begin{sideways}Bit banger\end{sideways}          & \begin{sideways}By the rules $(\mathcal{Q}: G)$\end{sideways}                    & \begin{sideways}Remote\end{sideways}                & $\CIRCLE$                           & $\Circle$                                   & {\small Error-Based Reconnaissance (C)\\Impersonation and Replay (I)\\Frame Hijacking (I)\\Physical-Fingerprint Distortion (I)\\Error State Manipulation (A)\\Error-Injection (A)\\Bus Access Denial (A)} \\
                                            &                                                  &                                                               &                                                  &                                     & $\LEFTcircle$                               & {\small Communication Surveillance (C)\\Fake Data Fabrication (I)}                                                                                                                                        \\
                                            &                                                  &                                                               &                                                  & $\LEFTcircle$                       & $\Circle$                                   & {\small Higher-Layer Sybil Exhaustion (A)\\Request Overwhelming (A)}                                                                                                                                      \\
                                            &                                                  &                                                               &                                                  &                                     & $\LEFTcircle$                               & {\small Privacy Leakage (C)\\Clock-Skew Network Mapping (C)\\ECU Functionality Disabling (A)}                                                                                                             \\
                                            &                                                  &                                                               &                                                  & $\Circle$                           & $\Circle$                                   & {\small Memory Leakage (C)\\Session-Based Buffer Overflow (I)}                                                                                                                                            \\
                                            &                                                  &                                                               &                                                  &                                     & $\LEFTcircle$                               & {\small Sensitive Information Sniffing (C)\\Bypassing Diagnostic Authentication (I)}                                                                                                                      \\
                                            &                                                  &                                                               &                                                  &                                     & $\CIRCLE$                                   & {\small Information and Firmware Dump (C)\\Memory and Firmware Manipulation (I)}                                                                                                                          \\
                                            &                                                  & \begin{sideways}$\mathcal{Q}:$ $G\rightarrow S$\end{sideways} & \begin{sideways}Remote $\rightarrow$ Limited\end{sideways} & $\CIRCLE$                           & $\Circle$                                   & {\small Double Receive (I)\\Unorthodox Frames (I)\\Synchronization Disruption (A)}                                                                                                                        \\
                                            &                                                  &                                                               &                                                  &                                     & $\CIRCLE$                                   & {\small Signal Attenuation} (A)                                                                                                                                                                             \\
                                            &                                                  &                                                               &                                                  & {\\$\LEFTcircle$}                       & {\\$\LEFTcircle$}                               & {\small Poly-semantic Frames (I)\\Frame Tampering (I)\\Polyglot Frames (I)}                                                                                                                               \\
                                            & \begin{sideways}$\mathcal{Q}$: $S$\end{sideways} &                                                               & {\\\begin{sideways}Limited\end{sideways}}                                         & {\\$\CIRCLE$} & {\\$\LEFTcircle$} & {\small Clock-Skew Network Mapping (C)\\Topology Intelligence (C)\\Electromagnetic Emissions (C)}                                                                                                         \\
                                            &                                                  &                                                               & \begin{sideways}Full   \end{sideways}                  & $\CIRCLE$                           & $\Circle$                                   & {\small Physical Architecture Manipulation (I)\\Physical Vandalism (A)}                                                                                                                                   
\end{tblr}
}
\end{table}

==> Tables/Papers.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Paper contribution to CIA elements and CAN stack layers.}
\label{tbl:papers}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccccc@{}}
& \multicolumn{3}{c}{\textbf{Security Element}}
& \multicolumn{3}{c}{\textbf{Layer}} \\
\cmidrule(lr){2-4}\cmidrule(l){5-7}
& \textbf{Conf.}
& \textbf{Integ.}
& \textbf{Avail.}
& \textbf{High.}
& \textbf{Ctrl.}
& \textbf{Trans.} \\
\midrule
\textbf{All Attack (67)}
& 33 & 28 & 23 & 29 & 34 & 21 \\
$\hookrightarrow$ \textbf{Excl. Dual-Use (50)}
& 17 & 28 & 22 & 29 & 32 & 6 \\
\textbf{All Defense (107)}
& 19 & 88 & 5 & 39 & 70 & 17 \\
\bottomrule
\end{tabular*}

\end{table}

==> Tables/RC.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
\footnotesize
\label{tbl:altsec}

\begin{tblr}{
  cells = {c},
  cell{1}{2} = {c=6}{},
  cell{3}{7} = {fg=black},
  hlines,
  vlines,
}
                           & Insecurity Root-Cause             &                                   &                                   &                                   &                                   &                                   \\
                           & \begin{sideways}RC!\end{sideways} & \begin{sideways}RC2\end{sideways} & \begin{sideways}RC3\end{sideways} & \begin{sideways}RC4\end{sideways} & \begin{sideways}RC5\end{sideways} & \begin{sideways}RC6\end{sideways} \\
Communication Surveillance & $\Circle$                         & $\Circle$                         & $\CIRCLE$                         & $\CIRCLE$                         & $\CIRCLE$                         & $\checkmark$                      \\
Error Injection            &                                   &                                   &                                   &                                   &                                   &                                   \\
Error State Manipulation   &                                   &                                   &                                   &                                   &                                   &                                   \\
Error Based Reconnaissance &                                   &                                   &                                   &                                   &                                   &                                   \\
Impersonation and Replay   &                                   &                                   &                                   &                                   &                                   &                                   \\
Double Receive             &                                   &                                   &                                   &                                   &                                   &                                   \\
Unorthodox Frames          &                                   &                                   &                                   &                                   &                                   &                                   \\
Frame Hijacking            &                                   &                                   &                                   &                                   &                                   &                                   \\
Fingerprint Distortion     &                                   &                                   &                                   &                                   &                                   &                                   \\
Bus Access Denial          &                                   &                                   &                                   &                                   &                                   &                                   \\
Synchronization Disruption &                                   &                                   &                                   &                                   &                                   &                                   \\
CANFD                      & $\Circle$                         & $\Circle$                         & $\CIRCLE$                         & $\CIRCLE$                         & $\CIRCLE$                         & $\uparrow$                        \\
CANXL                      & $\LEFTcircle$                     & $\LEFTcircle$                     & $\CIRCLE$                         & $\CIRCLE$                         &                                   &                                   \\
10Base-T1S                 & $\LEFTcircle$                     & $\LEFTcircle$                     & $\CIRCLE$                         & $\LEFTcircle$                     & –                                 &                                   
\end{tblr}
}
\end{table}

==> Tables/RC2.tex <==
% \usepackage{rotating}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}
\centering
\refstepcounter{table}
\resizebox{\columnwidth}{!}{
\label{tbl:altsec}
\arrayrulecolor{black}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c||c|c|c|} 
\hhline{~-----------|t|---|}
\multicolumn{1}{c|}{}      & {\cellcolor[rgb]{0.741,0.49,0.49}}\begin{sideways}\textcolor{white}{Com. Surveillance \Circle}\end{sideways} & \begin{sideways}Error Injection \Circle\end{sideways} & \begin{sideways}E. State Manip. \Circle\end{sideways} & \begin{sideways}E. Net Recon.\end{sideways} & {\cellcolor[rgb]{1,0.792,0.792}}\begin{sideways}Impersion  \& Rep \LEFTcircle.\end{sideways} & {\cellcolor[rgb]{0.741,0.867,0.741}}\begin{sideways}Double Receive \Circle \end{sideways} & {\cellcolor[rgb]{0.741,0.867,0.741}}\begin{sideways}Unorth. Frames \end{sideways} & \begin{sideways}~Frame Hijacking\end{sideways} & \begin{sideways}Fingerprint Distort.\end{sideways} & {\cellcolor[rgb]{1,0.792,0.792}}\begin{sideways}Bus Access Denial \Circle \end{sideways} & {\cellcolor[rgb]{0.741,0.867,0.741}}\begin{sideways}Synch. Disrupt. \Circle\end{sideways} & \begin{sideways}CANFD\end{sideways} & \begin{sideways}CANXL\end{sideways} & \begin{sideways}10-Base-T1S\end{sideways}  \\ 
\hhline{|------------||-=-|}
RC1                        & {\cellcolor[rgb]{0.741,0.49,0.49}}$\checkmark$                                                       & $\uparrow$                                    & $\uparrow$                                    & $\checkmark$                                & {\cellcolor[rgb]{1,0.792,0.792}}$\checkmark$                                   & {\cellcolor[rgb]{0.741,0.867,0.741}}$\uparrow$                                   & {\cellcolor[rgb]{0.741,0.867,0.741}}                                             & $\checkmark$                                   & $\uparrow$                                         & {\cellcolor[rgb]{1,0.792,0.792}}$\checkmark$                                    & {\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$                                  & $\checkmark$                        & $\checkmark$                        & $\checkmark$                               \\ 
\hline
RC2                        & {\cellcolor[rgb]{0.741,0.49,0.49}}                                                                   & $\checkmark$                                  & $\checkmark$                                  & $\checkmark$                                & {\cellcolor[rgb]{1,0.792,0.792}}$\checkmark$                                   & {\cellcolor[rgb]{0.741,0.867,0.741}}                                             & {\cellcolor[rgb]{0.741,0.867,0.741}}                                             & $\checkmark$                                   & $\checkmark$                                       & {\cellcolor[rgb]{1,0.792,0.792}}$\checkmark$                                    & {\cellcolor[rgb]{0.741,0.867,0.741}}                                              & $\checkmark$                        & $\checkmark$                        & $\checkmark$                               \\ 
\hhline{|----------->{\arrayrulecolor{blue}}=>{\arrayrulecolor{black}}:|---|}
RC3                        & {\cellcolor[rgb]{0.741,0.49,0.49}}                                                                   & $\checkmark$                                  & $\checkmark$                                  & $\checkmark$                                & {\cellcolor[rgb]{1,0.792,0.792}}                                               & {\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$                                 & {\cellcolor[rgb]{0.741,0.867,0.741}}                                             & $\checkmark$                                   & $\checkmark$                                       & {\cellcolor[rgb]{1,0.792,0.792}}                                                & {\cellcolor[rgb]{0.741,0.867,0.741}}                                              & $\checkmark$                        & R                                   & R                                          \\ 
\hline
RC4                        & {\cellcolor[rgb]{0.741,0.49,0.49}}                                                                   &                                               &                                               &                                             & {\cellcolor[rgb]{1,0.792,0.792}}                                               & {\cellcolor[rgb]{0.741,0.867,0.741}}                                             & {\cellcolor[rgb]{0.741,0.867,0.741}}                                             &                                                &                                                    & {\cellcolor[rgb]{1,0.792,0.792}}                                                & {\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$                                  & $\checkmark$                        & R                                   & R                                          \\ 
\hline
RC5                        & {\cellcolor[rgb]{0.741,0.49,0.49}}$\uparrow$                                                         & $\uparrow$                                    & $\uparrow$                                    & $\uparrow$                                  & {\cellcolor[rgb]{1,0.792,0.792}}$\uparrow$                                     & {\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$                                 & {\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$                                 & $\uparrow$                                     & $\uparrow$                                         & {\cellcolor[rgb]{1,0.792,0.792}}$\uparrow$                                      & {\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$                                  & ?                                   & R                                   & R                                          \\ 
\hhline{|============::===|}
\multicolumn{1}{|l|}{GRC1} & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.741,0.49,0.49}}$\checkmark$}                                  & \multicolumn{1}{l|}{}                         & \multicolumn{1}{l|}{}                         & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.792,0.792}}$\checkmark$}              & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.741,0.867,0.741}}}                        & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.741,0.867,0.741}}}                        & \multicolumn{1}{l|}{$\checkmark$}              & \multicolumn{1}{l|}{}                              & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.792,0.792}}}                           & \multicolumn{1}{l||}{{\cellcolor[rgb]{0.741,0.867,0.741}}}                        & \multicolumn{1}{l|}{$\checkmark$}   & \multicolumn{1}{l|}{$\checkmark$}   & \multicolumn{1}{l|}{$\checkmark$}          \\ 
\hline
\multicolumn{1}{|l|}{GRC2} & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.741,0.49,0.49}}$\uparrow$}                                    & \multicolumn{1}{l|}{$\checkmark$}             & \multicolumn{1}{l|}{$\checkmark$}             & \multicolumn{1}{l|}{$\uparrow$}             & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.792,0.792}}$\uparrow$}                & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.741,0.867,0.741}}$\uparrow$}              & \multicolumn{1}{l|}{{\cellcolor[rgb]{0.741,0.867,0.741}}$\uparrow$}              & \multicolumn{1}{l|}{$\uparrow$}                & \multicolumn{1}{l|}{$\uparrow$}                    & \multicolumn{1}{l|}{{\cellcolor[rgb]{1,0.792,0.792}}$\checkmark$}               & \multicolumn{1}{l||}{{\cellcolor[rgb]{0.741,0.867,0.741}}$\checkmark$}            & \multicolumn{1}{l|}{$\checkmark$}   & \multicolumn{1}{l|}{$\checkmark$}   & \multicolumn{1}{l|}{$\checkmark$}          \\
\hline
\end{tabular}
}
\end{table}

==> Tables/RC3.tex <==
% \usepackage{rotating}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}
\centering
\refstepcounter{table}
\resizebox{\columnwidth}{!}{
\label{tbl:CANRC}
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hhline{~------------|}
\multicolumn{1}{c|}{}                 & {\cellcolor[rgb]{1,0.804,0.804}}\begin{sideways}Fake Data F. \Circle\end{sideways} & {\cellcolor[rgb]{1,0.804,0.804}}\begin{sideways}Com. Surveil. \Circle\end{sideways} & \begin{sideways}Imperson.  Rep remove rc3. RC5?\end{sideways} & \begin{sideways}B. Ax Denial \textcolor[rgb]{0.867,0.867,0.867}{\Circle}\end{sideways} & \begin{sideways}Error Injection \textcolor[rgb]{0.867,0.867,0.867}{\Circle}\end{sideways} & \begin{sideways}E. State Manip. \textcolor[rgb]{0.867,0.867,0.867}{\Circle}\end{sideways} & \begin{sideways}E. Net. Recon.\end{sideways} & \begin{sideways}Frame Hijack\end{sideways} & \begin{sideways}Fngrprnt Distort.~\end{sideways} & {\cellcolor[rgb]{0.867,0.867,0.867}}\begin{sideways}Unorth. Frames\end{sideways} & {\cellcolor[rgb]{0.867,0.867,0.867}}\begin{sideways}Double Receive (Add DRC2)\Circle\end{sideways} & {\cellcolor[rgb]{0.867,0.867,0.867}}\begin{sideways}Synch. Disrupt. \Circle\end{sideways}  \\ 
\hline
RC1                                   & {\cellcolor[rgb]{1,0.804,0.804}}$\checkmark$                                                      & {\cellcolor[rgb]{1,0.804,0.804}}$\checkmark$                                                       & $\checkmark$                                  & $\checkmark$                                                                                          & $\checkmark$                                                                                             & $\checkmark$                                                                                             & $\checkmark$                                 & $\checkmark$                               & $\checkmark$                                     & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                 & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                                        & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                                          \\ 
\hline
RC2                                   & {\cellcolor[rgb]{1,0.804,0.804}}                                                                  & {\cellcolor[rgb]{1,0.804,0.804}}$\checkmark$                                                       & $\checkmark$                                  & $\checkmark$                                                                                          & $\uparrow$                                                                                               & $\uparrow$                                                                                               & $\checkmark$                                 & $\checkmark$                               & $\uparrow$                                       & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                                          & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                                          \\ 
\hline
RC3                                   & {\cellcolor[rgb]{1,0.804,0.804}}                                                                  & {\cellcolor[rgb]{1,0.804,0.804}}                                                                   & $\checkmark$                     & $\checkmark$                                                                             & $\checkmark$                                                                                             & $\checkmark$                                                                                             & $\checkmark$                                 & $\checkmark$                               & $\checkmark$                                     & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                                                    & {\cellcolor[rgb]{0.867,0.867,0.867}}                                                                      \\ 
\hline
RC4                                   & {\cellcolor[rgb]{1,0.804,0.804}}                                                                  & {\cellcolor[rgb]{1,0.804,0.804}}                                                                   &                                               &                                                                                                       & $\checkmark$                                                                                             & $\checkmark$                                                                                             & $\checkmark$                                 & $\checkmark$                               & $\checkmark$                                     & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                                        & {\cellcolor[rgb]{0.867,0.867,0.867}}                                                                      \\ 
\hline
\rowcolor[rgb]{0.867,0.867,0.867} RC5 &                                                                                                   & $\uparrow$                                                                                         & $\uparrow$                                    & $\uparrow$                                                                                            & $\uparrow$                                                                                               & $\uparrow$                                                                                               & $\uparrow$                                   & $\uparrow$                                 & $\uparrow$                                       & $\checkmark$                                                                     & $\checkmark$                                                                                            & $\checkmark$                                                                                              \\ 
\hhline{|=============|}
DRC1                                  & {\cellcolor[rgb]{1,0.804,0.804}}                                                                  & {\cellcolor[rgb]{1,0.804,0.804}}$\checkmark$                                                       & $\checkmark$                                  &                                                                                                       &                                                                                                          &                                                                                                          &                                              & $\checkmark$                               &                                                  & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                                                    & {\cellcolor[rgb]{0.867,0.867,0.867}}                                                                      \\ 
\hline
DRC2                                  & {\cellcolor[rgb]{1,0.804,0.804}}                                                                  & {\cellcolor[rgb]{1,0.804,0.804}}$\uparrow$                                                         & $\uparrow$                                    & $\checkmark$                                                                                          & $\checkmark$                                                                                             & $\checkmark$                                                                                             & $\uparrow$                                   & $\uparrow$                                 & $\uparrow$                                       & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                   & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                                          & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                                          \\ 
\hline
DRC3                                  & {\cellcolor[rgb]{1,0.804,0.804}}$\checkmark$                                                      & {\cellcolor[rgb]{1,0.804,0.804}}                                                                   &                                               &                                                                                                       &                                                                                                          &                                                                                                          &                                              & $\uparrow$                                 &                                                  & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                   & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                                          & {\cellcolor[rgb]{0.867,0.867,0.867}}                                                                      \\
\hline
\end{tabular}
}
\end{table}

==> Tables/RC4.tex <==
% \usepackage{rotating}
% \usepackage{colortbl}
% \usepackage{hhline}
% \definecolor{BurntOrange}{rgb}{0.5,0.5,0.5}
% \definecolor{Manhattan}{rgb}{0.854,0.854,0.854}
% to make back orange replace:{0.678,0.678,0.678} with {0.945,0.733,0.612}
\begin{table}
\centering
\caption{Attack and defense-gap root-cause vetting}
\label{tbl:CANRC}
\resizebox{\columnwidth}{!}{
\begin{tabular}{||c||c|c|c|c|c|c|c|c|c||c|c|c||c|c|c||} 
\hhline{~|t:=========:t:===:t:===:t|}
\multicolumn{1}{c||}{}                           & {\cellcolor[rgb]{1,0.9,0.86}}\begin{sideways}Fake Data F.\end{sideways} & {\cellcolor[rgb]{1,0.9,0.86}}\begin{sideways}Com. Surveil.\end{sideways} & \begin{sideways}Imperson.   Rep\end{sideways} & {\cellcolor[rgb]{0.678,0.678,0.678}}\begin{sideways}B. Ax Denial \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & {\cellcolor[rgb]{0.678,0.678,0.678}}\begin{sideways}Error Injection \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & {\cellcolor[rgb]{0.678,0.678,0.678}}\begin{sideways}E. State Manip. \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Net. Recon.\end{sideways} & \begin{sideways}Frame Hijack\end{sideways} & \begin{sideways}Fngrprnt Distort.~\end{sideways} & \begin{sideways}CANFD\end{sideways} & \begin{sideways}CANXL\end{sideways} & \begin{sideways}10B-T1S\end{sideways} & {\cellcolor[rgb]{0.867,0.867,0.867}}\begin{sideways}Unorth. Frames\end{sideways} & {\cellcolor[rgb]{0.678,0.678,0.678}}\begin{sideways}Double Receive\end{sideways} & {\cellcolor[rgb]{0.678,0.678,0.678}}\begin{sideways}Synch. Disrupt.\end{sideways}  \\ 
\hhline{|t:=::=========::===::===:|}
$\mathcal{R}$1                                   & $\checkmark$                                                               & $\checkmark$                                                                & $\checkmark$                                  & $\checkmark$                                                                                                        & $\checkmark$                                                                                                           & $\checkmark$                                                                                                           & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                             & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                 & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                 & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                   \\ 
\hline
$\mathcal{R}$2                                   &                                                                            & $\checkmark$                                                                & $\checkmark$                                  & $\checkmark$                                                                                                        & $\uparrow$                                                                                                             & $\uparrow$                                                                                                             & $\checkmark$                              & $\checkmark$                               & $\uparrow$                                       & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                   & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                   \\ 
\hline
$\mathcal{R}$3                                   &                                                                            &                                                                             &                                               & $\checkmark$                                                                                                        & $\checkmark$                                                                                                           & $\checkmark$                                                                                                           & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                               \\ 
\hline
$\mathcal{R}$4                                   &                                                                            &                                                                             &                                               &                                                                                                                     & $\checkmark$                                                                                                           & $\checkmark$                                                                                                           & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\LEFTcircle$                       & $\Circle$                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                 & {\cellcolor[rgb]{0.867,0.867,0.867}}                                               \\ 
\hline
\rowcolor[rgb]{0.867,0.867,0.867} $\mathcal{R}$5 &                                                                            & $\halfcheckmark$                                                            &                                               & $\halfcheckmark$                                                                                                    & $\halfcheckmark$                                                                                                       & $\halfcheckmark$                                                                                                       & $\halfcheckmark$                          & $\halfcheckmark$                           & $\halfcheckmark$                                 &                                     &                                     &                                       & $\checkmark$                                                                     & $\checkmark$                                                                     & $\checkmark$                                                                       \\ 
\hhline{|:=::=========::===::===:|}
$\mathcal{DR}$1                                  &                                                                            & $\checkmark$                                                                & $\checkmark$                                  &                                                                                                                     &                                                                                                                        &                                                                                                                        &                                           & $\checkmark$                               &                                                  & $\LEFTcircle$                       & $\LEFTcircle$                       & $\LEFTcircle$                         & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                               \\ 
\hline
$\mathcal{DR}$2                                  &                                                                            &                                                                             & $\uparrow$                                    & $\checkmark$                                                                                                        & $\checkmark$                                                                                                           & $\checkmark$                                                                                                           & $\uparrow$                                & $\halfcheckmark$                           & $\halfcheckmark$                                 & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                             & {\cellcolor[rgb]{0.867,0.867,0.867}}$\uparrow$                                   & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                 & {\cellcolor[rgb]{0.867,0.867,0.867}}$\checkmark$                                   \\ 
\hline
$\mathcal{DR}$3                                  & $\checkmark$                                                               &                                                                             & $\uparrow$                                    &                                                                                                                     &                                                                                                                        &                                                                                                                        &                                           & $\uparrow$                                 &                                                  & $\CIRCLE $                          & $\CIRCLE $                          & $\CIRCLE $                            & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                             & {\cellcolor[rgb]{0.867,0.867,0.867}}                                               \\ 
\hhline{|:=::=========::===:b:===:b|}
FD                                               & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                   & $\CIRCLE$                                     & $\CIRCLE$                                                                                                           & $\CIRCLE$                                                                                                              & $\CIRCLE$                                                                                                              & $\CIRCLE$                                 & $\CIRCLE$                                  & $\CIRCLE$                                        & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                                                             & \multicolumn{1}{c}{}                                                             & \multicolumn{1}{c}{}                                                               \\ 
\hhline{||-||---------||~~~~~~}
XL                                               & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                   & $\CIRCLE$                                     & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                                                           & $-$                                                                                                                    & $-$                                                                                                                    & $-$                                       & $-$                                        & $-$                                              & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                                                             & \multicolumn{1}{c}{}                                                             & \multicolumn{1}{c}{}                                                               \\ 
\hhline{||-||---------||~~~~~~}
T1S                                              & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                   & $\CIRCLE$                                     & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$                                                                           & $-$                                                                                                                    & $\Circle$                                                                                                              & {\cellcolor[rgb]{1,0.9,0.86}}$\CIRCLE$ & $-$                                        & $-$                                              & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                                                             & \multicolumn{1}{c}{}                                                             & \multicolumn{1}{c}{}                                                               \\
\hhline{|b:=:b:=========:b|~~~~~~}
\end{tabular}
}
\end{table}

==> Tables/RCAlt.tex <==
% \usepackage{rotating}
% \usepackage{tabularray}
\begin{table}
\centering

\resizebox{\columnwidth}{!}{
\footnotesize
\refstepcounter{table}
\label{tbl:altsec}
\begin{tblr}{
  cells = {c},
  vline{2-10} = {1}{},
  vline{-} = {2-4}{},
  hline{1} = {2-9}{},
  hline{2-5} = {-}{},
}
            & RC1                       & RC2                       & RC3                       & RC4                       & RC5 & DRC1                      & DRC2                      & DRC3                      \\
CANFD       & $\checkmark$& $\checkmark$& $\checkmark$& $\checkmark$& ?    & $\checkmark$& $\checkmark$& $\checkmark$\\
CANXL       & $\checkmark$& $\checkmark$& $\checkmark$& R                         & R    & $\checkmark$& $\checkmark$& $\checkmark$\\
10-BASE T1S & $\checkmark$& $\checkmark$& $\checkmark$& R                         & R    & $\checkmark$& $\checkmark$& $\checkmark$
\end{tblr}
}
\end{table}

==> Tables/RCEliminate.tex <==
% \usepackage{rotating}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}
\centering
\caption{Attack and defense-gap root-cause vetting. \kha{Edit}}
\label{tbl:CANRC}
\resizebox{\columnwidth}{0.1\textheight}{
\begin{tabular}{||c||c|c|c|c|c|c|c|c|c||c|c|c||} 
\hhline{~|t:=========:t:===:t|}
\multicolumn{1}{c||}{} & {\cellcolor[rgb]{1,0.902,0.859}}\begin{sideways}Fake Data F.\end{sideways} & {\cellcolor[rgb]{1,0.902,0.859}}\begin{sideways}Com. Surveil.\end{sideways} & \begin{sideways}Imperson.   Rep\end{sideways} & \begin{sideways}B. Ax Denial \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Error Injection \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}E. State Man. \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Net. Recon.\end{sideways} & \begin{sideways}Frame Hijack\end{sideways} & \begin{sideways}Fngrprnt Dist.~\end{sideways} & \begin{sideways}CANFD\end{sideways} & \begin{sideways}CANXL\end{sideways} & \begin{sideways}10B-T1S\end{sideways}  \\ 
\hhline{|t:=::=========::===:|}
$\mathcal{R}$1         & $\checkmark$                                                               & $\checkmark$                                                                & $\checkmark$                                  & $\checkmark$                                                                    & $\checkmark$                                                                       & $\checkmark$                                                                       & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{R}$2         &                                                                            & $\checkmark$                                                                & $\checkmark$                                  & $\checkmark$                                                                    & $\uparrow$                                                                         & $\uparrow$                                                                         & $\checkmark$                              & $\checkmark$                               & $\uparrow$                                       & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{R}$3         &                                                                            &                                                                             &                                               & $\checkmark$                                                                    & $\checkmark$                                                                       & $\checkmark$                                                                       & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{R}$4         &                                                                            &                                                                             &                                               &                                                                                 & $\checkmark$                                                                       & $\checkmark$                                                                       & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\LEFTcircle$                       & $\Circle$                              \\ 
\hline
$\mathcal{DR}$1        &                                                                            & $\checkmark$                                                                & $\checkmark$                                  &                                                                                 &                                                                                    &                                                                                    &                                           & $\checkmark$                               &                                                  & $\LEFTcircle$                       & $\LEFTcircle$                       & $\LEFTcircle$                          \\ 
\hline
$\mathcal{DR}$2        &                                                                            &                                                                             & $\uparrow$                                    & $\checkmark$                                                                    & $\checkmark$                                                                       & $\checkmark$                                                                       & $\uparrow$                                & $\halfcheckmark$                           & $\halfcheckmark$                                 & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{DR}$3        & $\checkmark$                                                               &                                                                             & $\uparrow$                                    &                                                                                 &                                                                                    &                                                                                    &                                           & $\uparrow$                                 &                                                  & $\CIRCLE $                          & $\CIRCLE $                          & $\CIRCLE $                             \\ 
\hhline{|:=::=========::===:b|}
CANFD                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                   & $\CIRCLE$                                     & $\CIRCLE$                                                                       & $\CIRCLE$                                                                          & $\CIRCLE$                                                                          & $\CIRCLE$                                 & $\CIRCLE$                                  & $\CIRCLE$                                        & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                   \\ 
\hhline{||-||---------||~~~}
CANXL                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                   & $\CIRCLE$                                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                       & $-$                                                                                & $-$                                                                                & $-$                                       & $-$                                        & $-$                                              & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                   \\ 
\hhline{||-||---------||~~~}
10BASE-T1S                    & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                   & $\CIRCLE$                                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                       & $-$                                                                                & $\Circle$                                                                          & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $-$                                        & $-$                                              & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                   \\
\hhline{|b:=:b:=========:b|~~~}
\end{tabular}
}
\end{table}

==> Tables/RCEliminateNew.tex <==
% \usepackage{rotating}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}
\centering
\caption{Attack and defense-gap root-cause vetting. \kha{Edit}}
\label{tbl:CANRC}
\resizebox{\columnwidth}{0.1\textheight}{
\begin{tabular}{||c||c|c|c|c|c|c|c|c|c|c|c||c|c|c|c||} 
\hhline{~|t:===========:t:====:t|}
\multicolumn{1}{c||}{} & {\cellcolor[rgb]{1,0.902,0.859}}\begin{sideways}Com. Surveil.\end{sideways} & \begin{sideways}Priv. Leak.\end{sideways} & \begin{sideways}Fake Data F.\end{sideways}  & \begin{sideways}Imperson.   Rep\end{sideways} & \begin{sideways}B. Ax Denial \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Error Injection \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}E. State Man. \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Net. Recon.\end{sideways} & \begin{sideways}Frame Hijack\end{sideways} & \begin{sideways}Fngrprnt Dist.~\end{sideways} & \begin{sideways}Skew Map.\end{sideways} &  \begin{sideways}CANFD\end{sideways} & \begin{sideways}CANXL (Err. On)\end{sideways} & \begin{sideways}CANXL (Err. Off)\end{sideways} & \begin{sideways}10BASE-T1S\end{sideways}  \\ 
\hhline{|t:=::===========::====:|}
$\mathcal{R}$1         &    $\checkmark$                                                                        &   $\checkmark$                                                                          & $\checkmark$                                        & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$\\ 
\hline
$\mathcal{R}$3 &  $\checkmark$ & $\checkmark$ & & $\checkmark$ & $\checkmark$ & & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$\\ 
\hline
$\mathcal{R}$4 & & & & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $\CIRCLE$  & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$\\ 
\hline
$\mathcal{R}$5 & & & & & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $\CIRCLE$  & $\CIRCLE$ & $\LEFTcircle$ & $\Circle$\\ 
\hline
$\mathcal{DR}$1 & $\checkmark$ & $\checkmark$ & & $\checkmark$ & & & & & $\checkmark$ & & & $\LEFTcircle$  & $\LEFTcircle$ & $\LEFTcircle$ & $\LEFTcircle$\\ 
\hline
$\mathcal{DR}$2 & & & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & & $\CIRCLE$ & $\CIRCLE$  & $\CIRCLE$ & $\CIRCLE$\\ 
\hhline{|:=::===========::====:b|}
CANFD & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}\\ 
\hhline{||-||-----------||~~~~}
CANXL (Err. On) & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}\\
\hhline{||-||-----------||~~~~}
CANXL (Err. Off) & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $\CIRCLE$ & $\Circle$ & - & - & $\CIRCLE$ & $\CIRCLE$ & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}\\
\hhline{||-||-----------||~~~~}
10BASE-T1S & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & - & $\Circle$ & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & - & - & $\CIRCLE$ & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}\\
\hhline{|b:=:b:===========:b|~~~~}
\end{tabular}
}
\end{table}

==> Tables/RCEliminateRevised.tex <==
% \usepackage{rotating}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}
\centering
\caption{Attack and defense-gap root-cause vetting. \kha{Edit}}
\label{tbl:CANRC}
\resizebox{\columnwidth}{0.1\textheight}{
\begin{tabular}{||c||c|c|c|c|c|c|c|c|c||c|c|c||} 
\hhline{~|t:=========:t:===:t|}
\multicolumn{1}{c||}{} & {\cellcolor[rgb]{1,0.902,0.859}}\begin{sideways}Fake Data F.\end{sideways} & {\cellcolor[rgb]{1,0.902,0.859}}\begin{sideways}Com. Surveil.\end{sideways} & \begin{sideways}Imperson.   Rep\end{sideways} & \begin{sideways}B. Ax Denial \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Error Injection \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}E. State Man. \textcolor[rgb]{0.867,0.867,0.867}{}\end{sideways} & \begin{sideways}Net. Recon.\end{sideways} & \begin{sideways}Frame Hijack\end{sideways} & \begin{sideways}Fngrprnt Dist.~\end{sideways} & \begin{sideways}CANFD\end{sideways} & \begin{sideways}CANXL\end{sideways} & \begin{sideways}10B-T1S\end{sideways}  \\ 
\hhline{|t:=::=========::===:|}
$\mathcal{R}$3         &                                                                            &                                                                             &                                               &                                                                                 & $\checkmark$                                                                       & $\checkmark$                                                                       & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\LEFTcircle$                       & $\Circle$                              \\ 
\hline
$\mathcal{R}$6         & $\checkmark$                                                                            & $\checkmark$                                                                & $\checkmark$                                  & $\checkmark$                                                                    &                                                                          &                                                                          & $\checkmark$                              &                               &                                        & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{R}$7         &                                                                            &                                                                             &      $\checkmark$                                         & $\checkmark$                                                                    & $\checkmark$                                                                       & $\checkmark$                                                                       & $\checkmark$                              & $\checkmark$                               & $\checkmark$                                     & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{DR}$1        &                                                                            & $\checkmark$                                                                & $\checkmark$                                  &                                                                                 &                                                                                    &                                                                                    &                                           & $\checkmark$                               &                                                  & $\LEFTcircle$                       & $\LEFTcircle$                       & $\LEFTcircle$                          \\ 
\hline
$\mathcal{DR}$2        &                                                                            &                                                                             &                                     & $\checkmark$                                                                    & $\checkmark$                                                                       & $\checkmark$                                                                       &                                 &                            &                                  & $\CIRCLE$                           & $\CIRCLE$                           & $\CIRCLE$                              \\ 
\hline
$\mathcal{DR}$3        & $\checkmark$                                                               &                                                                             &   $\checkmark$  &                                                                                 &                                                                                    &                                                                                    &                                           &  $\checkmark$                                &                                                  & $\CIRCLE $                          & $\CIRCLE $                          & $\CIRCLE $                             \\ 
\hhline{|:=::=========::===:b|}
CANFD                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                   & $\CIRCLE$                                     & $\CIRCLE$                                                                       & $\CIRCLE$                                                                          & $\CIRCLE$                                                                          & $\CIRCLE$                                 & $\CIRCLE$                                  & $\CIRCLE$                                        & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                   \\ 
\hhline{||-||---------||~~~}
CANXL                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                   & $\CIRCLE$                                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                       & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                                                                & $\Circle$                                                                               & $-$                                       & $-$                                        & $-$                                              & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                   \\ 
\hhline{||-||---------||~~~}
10BASE-T1S                    & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                  & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                   & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                     & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$                                       & $-$                                                                                & $\Circle$                                                                          & {\cellcolor[rgb]{1,0.902,0.859}}$\CIRCLE$ & $-$                                        & $-$                                              & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                & \multicolumn{1}{c}{}                   \\
\hhline{|b:=:b:=========:b|~~~}
\end{tabular}
}
\end{table}

==> Tables/backuptable.tex <==
% \usepackage{color}
% \usepackage{rotating}
% \usepackage{tabularray}
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.945,0.752,0.752}
\begin{table*}
\caption{Broad CAN attack categories severity assessment juxtaposed with assessed effectiveness of the main defense categories. Dashed lines mean that whatever is above the line holds below it while whatever is below the line does not hold above it. Dotted lines mean the opposite.}
\centering
\label{tbl:bigtable}
\resizebox{\textwidth}{!}{
\begin{tblr}{
  row{odd} = {c},
  row{2} = {c},
  row{4} = {c},
  row{6} = {c},
  row{8} = {c},
  row{12} = {c},
  row{14} = {c},
  row{16} = {c},
  row{18} = {c},
  row{20} = {c},
  row{22} = {c},
  row{24} = {BeautyBush,c},
  row{26} = {c},
  row{28} = {c},
  row{30} = {c},
  row{32} = {c},
  row{34} = {c},
  row{36} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=6}{},
  cell{1}{9} = {c=7}{},
  cell{3}{1} = {r=11}{},
  cell{3}{2} = {r=5}{},
  cell{3}{3} = {Matrix,fg=white},
  cell{3}{4} = {BeautyBush},
  cell{3}{5} = {BeautyBush},
  cell{3}{6} = {BeautyBush},
  cell{3}{7} = {BeautyBush},
  cell{3}{8} = {BeautyBush},
  cell{4}{3} = {fg=white},
  cell{6}{9} = {r=2}{},
  cell{6}{10} = {r=2}{},
  cell{6}{11} = {r=2}{},
  cell{6}{12} = {r=2}{},
  cell{6}{13} = {r=2}{},
  cell{6}{14} = {r=2}{},
  cell{6}{15} = {r=2}{},
  cell{8}{2} = {r=3}{},
  cell{8}{3} = {BeautyBush},
  cell{8}{4} = {BeautyBush},
  cell{8}{5} = {BeautyBush},
  cell{8}{6} = {BeautyBush},
  cell{8}{7} = {BeautyBush},
  cell{8}{8} = {BeautyBush},
  cell{10}{3} = {r=2}{c},
  cell{10}{4} = {r=2}{c},
  cell{10}{5} = {r=2}{c},
  cell{10}{6} = {r=2}{c},
  cell{10}{7} = {r=2}{c},
  cell{10}{8} = {r=2}{},
  cell{10}{9} = {r=3}{c},
  cell{10}{10} = {r=3}{c},
  cell{10}{11} = {r=3}{c},
  cell{10}{12} = {r=3}{c},
  cell{10}{13} = {r=3}{c},
  cell{10}{14} = {r=3}{c},
  cell{10}{15} = {r=3}{c},
  cell{11}{2} = {r=3}{},
  cell{14}{1} = {r=15}{},
  cell{14}{2} = {r=4}{},
  cell{18}{2} = {r=9}{},
  cell{18}{3} = {BeautyBush},
  cell{18}{4} = {BeautyBush},
  cell{18}{5} = {BeautyBush},
  cell{18}{6} = {BeautyBush},
  cell{18}{7} = {BeautyBush},
  cell{18}{8} = {BeautyBush},
  cell{19}{9} = {r=2}{},
  cell{19}{10} = {r=2}{},
  cell{19}{11} = {r=2}{},
  cell{19}{12} = {r=2}{},
  cell{19}{13} = {r=2}{},
  cell{19}{14} = {r=2}{},
  cell{19}{15} = {r=2}{},
  cell{21}{3} = {Matrix,fg=white},
  cell{21}{4} = {BeautyBush},
  cell{21}{5} = {BeautyBush},
  cell{21}{6} = {BeautyBush},
  cell{21}{7} = {BeautyBush},
  cell{21}{8} = {BeautyBush},
  cell{21}{9} = {r=4}{},
  cell{21}{10} = {r=4}{},
  cell{21}{11} = {r=4}{},
  cell{21}{12} = {r=4}{},
  cell{21}{13} = {r=4}{},
  cell{21}{14} = {r=4}{},
  cell{21}{15} = {r=4}{},
  cell{25}{3} = {BeautyBush},
  cell{25}{4} = {BeautyBush},
  cell{25}{5} = {BeautyBush},
  cell{25}{6} = {BeautyBush},
  cell{25}{7} = {BeautyBush},
  cell{25}{8} = {BeautyBush},
  cell{27}{2} = {r=2}{},
  cell{29}{1} = {r=8}{},
  cell{29}{2} = {r=3}{},
  cell{29}{9} = {r=3}{},
  cell{29}{10} = {r=3}{},
  cell{29}{11} = {r=3}{},
  cell{29}{12} = {r=3}{},
  cell{29}{13} = {r=3}{},
  cell{29}{14} = {r=3}{},
  cell{29}{15} = {r=3}{},
  cell{32}{2} = {r=3}{},
  cell{32}{3} = {Matrix,fg=white},
  cell{32}{4} = {BeautyBush},
  cell{32}{5} = {BeautyBush},
  cell{32}{6} = {BeautyBush},
  cell{32}{7} = {BeautyBush},
  cell{32}{8} = {BeautyBush},
  cell{33}{3} = {Matrix,fg=white},
  cell{33}{4} = {BeautyBush},
  cell{33}{5} = {BeautyBush},
  cell{33}{6} = {BeautyBush},
  cell{33}{7} = {BeautyBush},
  cell{33}{8} = {BeautyBush},
  cell{34}{3} = {Matrix,fg=white},
  cell{34}{4} = {BeautyBush},
  cell{34}{5} = {BeautyBush},
  cell{34}{6} = {BeautyBush},
  cell{34}{7} = {BeautyBush},
  cell{34}{8} = {BeautyBush},
  cell{34}{9} = {r=2}{},
  cell{34}{10} = {r=2}{},
  cell{34}{11} = {r=2}{},
  cell{34}{12} = {r=2}{},
  cell{34}{13} = {r=2}{},
  cell{34}{14} = {r=2}{},
  cell{34}{15} = {r=2}{},
  cell{35}{2} = {r=2}{},
  cell{35}{3} = {Matrix,fg=white},
  cell{35}{4} = {BeautyBush},
  cell{35}{5} = {BeautyBush},
  cell{35}{6} = {BeautyBush},
  cell{35}{7} = {BeautyBush},
  cell{35}{8} = {BeautyBush},
  vlines,
  hline{1,3,14,29,37} = {-}{},
  hline{2,5-6,9-10,13,15,17,19,26,28} = {3-15}{},
  hline{4,7,12,16,20-25,30-31,33-34,36} = {3-8}{},
  hline{4,25,27,36} = {9-15}{dashed},
  hline{8,18,32} = {2-15}{},
  hline{11} = {2}{},
  hline{16} = {9-10,12-15}{dotted},
  hline{21,33-34} = {9-15}{dotted},
  hline{27,35} = {2-8}{},
}
\begin{sideways}Component\end{sideways}       & \begin{sideways}Layer\end{sideways}      & Attack                              &                                       &                                        &                                      &                                          &                                          & Defense                                                                                                                              &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Category                            & \begin{sideways}Ability\end{sideways} & \begin{sideways}Hardware\end{sideways} & \begin{sideways}Access\end{sideways} & \begin{sideways}Prevalence\end{sideways} & \begin{sideways}Complexity\end{sideways} & Category                                                                                                                             & \begin{sideways}Protection\end{sideways} & \begin{sideways}Coverage\end{sideways}                                            & \begin{sideways}ECU Impact\end{sideways}                                              & \begin{sideways}Bus Impact\end{sideways}                                                  & \begin{sideways}Infrastructure\end{sideways}                                      & \begin{sideways}Validity\end{sideways}                                        \\
\begin{sideways}Confidentiality\end{sideways} & \begin{sideways}Higher\end{sideways}     & Communication Surveillance          & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \LEFTcircle                            & Message Obfuscation                                                                                                                  & P                                        & \LEFTcircle                                                                     & \CIRCLE                                                                             & \CIRCLE                                                                                 & \Circle                                                                         & \CIRCLE                                                                     \\
                                              &                                          & Privacy Leakage                     & \Circle                             & \Circle                              & \Circle                            & \LEFTcircle                            & \LEFTcircle                            & Privacy-preserving Transformations                                                                                                   & P                                        & \LEFTcircle                                                                     & --                                                                                  & --                                                                                      & \Circle                                                                         & \Circle                                                                     \\
                                              &                                          & Sensitive Information Sniffing      & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \LEFTcircle                            & {Better Protocol Implementation\\Message Obfuscation}                                                                                & {P\\P}                                   & {\CIRCLE\\\CIRCLE}                                                            & {\Circle\\\Circle}                                                                & {\Circle\\\Circle}                                                                    & {\Circle\\\Circle}                                                            & {\CIRCLE\\\CIRCLE}                                                        \\
                                              &                                          & Memory Leakage                      & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \Circle                                & {Memory and Firmware Concealment\\Better Protocol Implementation\\Diagnostic Session Authentication}                                 & {P\\P\\P}                                & {\CIRCLE\\\CIRCLE\\\LEFTcircle}                                             & {\LEFTcircle\\\Circle\\\Circle}                                                 & {\Circle\\\Circle\\\Circle}                                                         & {\LEFTcircle\\\Circle\\\Circle}                                             & {\LEFTcircle\\\CIRCLE\\\CIRCLE}                                         \\
                                              &                                          & Information and Firmware Dump       & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \CIRCLE                                &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              & \begin{sideways}Controller\end{sideways} & Error-Based Reconnaissance          & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {Disabling Automatic Retransmissions\\lnterframe-Spacing Anonymization\\ID Anonymization}                                            & {P\\P\\P}                                & {\CIRCLE\\\LEFTcircle\\\LEFTcircle}                                         & {\Circle\\\LEFTcircle\\\Circle}                                                 & {\LEFTcircle\\\LEFTcircle\\\Circle}                                                 & {\Circle\\\Circle\\\Circle}                                                 & {\CIRCLE\\\CIRCLE\\\CIRCLE}                                             \\
                                              &                                          & Clock-Skew Network Mapping          & \Circle                             & \Circle                              & \Circle                            & \LEFTcircle                            & \LEFTcircle                            & Skew Cloaking                                                                                                                        & P                                        & \CIRCLE                                                                         & \LEFTcircle                                                                         & \Circle                                                                                 & \Circle                                                                         & \CIRCLE                                                                     \\
                                              &                                          & Signal and Hardware Profiling       & \CIRCLE                             & \CIRCLE                              & \LEFTcircle                        & \CIRCLE                                & \LEFTcircle                            & –                                                                                                                                    & –                                        & –                                                                                 & –                                                                                     & –                                                                                         & –                                                                                 & –                                                                             \\
                                              & \begin{sideways}Transwire\end{sideways}  &                                     &                                       &                                        &                                      &                                          &                                          &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Location Identification             & \CIRCLE                             & \CIRCLE                              & \CIRCLE                            & \CIRCLE                                & \LEFTcircle                            &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Electromagnetic Emissions           & \CIRCLE                             & \CIRCLE                              & \LEFTcircle                        & \CIRCLE                                & \LEFTcircle                            & Shielding and Signal Slope Control                                                                                                   & P                                        & --                                                                              & --                                                                                  & --                                                                                      & --                                                                              & \Circle                                                                     \\
\begin{sideways}Integrity\end{sideways}       & \begin{sideways}Higher\end{sideways}     & Fake Data Fabrication (Highly replicable)              & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \LEFTcircle                            & Content Inspection                                                                                                                   & D,P*                                     & \CIRCLE                                                                         & \Circle                                                                             & \Circle                                                                                 & \Circle                                                                         & \CIRCLE                                                                     \\
                                              &                                          & Memory and Firmware Manipulation    & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \CIRCLE                                & Firmware Attestation                                                                                                                 & D,P                                      & \CIRCLE                                                                         & \Circle                                                                             & \Circle                                                                                 & \CIRCLE                                                                         & \LEFTcircle                                                                 \\
                                              &                                          & Bypassing Diagnostic Authentication & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \LEFTcircle                            & {Diagnostic Session Authentication\\ECU Hardening}                                                                                   & {P\\P}                                   & {\CIRCLE\\\LEFTcircle}                                                        & {\Circle\\\LEFTcircle}                                                            & {\Circle\\\Circle}                                                                    & {\Circle\\\CIRCLE}                                                            & {\CIRCLE\\\LEFTcircle}                                                    \\
                                              &                                          & Session-Based Buffer Overflow       & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \Circle                                & {Content Inspection\\ECU Guardian\\Better Protocol Implementation}                                                                   & {D\\P\\P}                                & {\CIRCLE\\\LEFTcircle\\\CIRCLE}                                             & {\Circle\\\Circle\\\Circle}                                                     & {\Circle\\\Circle\\\Circle}                                                         & {\Circle\\\CIRCLE\\\Circle}                                                 & {\CIRCLE\\\LEFTcircle\\\Circle}                                         \\
                                              & \begin{sideways}Controller\end{sideways} & Impersonation and Replay            & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {PIDS\\Per-ECU Authentication\\Centralized Authentication\\Time  IFS Anonymization\\Bit-Banger IDS\\Victim Resistance\\ECU Guardian} & {D,P*\\D,P\\D,P\\D,P*\\D,P*\\P\\P}       & {\CIRCLE\\\LEFTcircle\\\CIRCLE\\\CIRCLE\\\CIRCLE\\\CIRCLE\\\CIRCLE} & {\Circle\\\CIRCLE\\\LEFTcircle\\\LEFTcircle\\\Circle\\\Circle\\\Circle} & {\Circle\\\LEFTcircle\\\LEFTcircle\\\LEFTcircle\\\Circle\\\Circle\\\Circle} & {\Circle\\\Circle\\\Circle\\\Circle\\\Circle\\\LEFTcircle\\\CIRCLE} & {\CIRCLE\\\CIRCLE\\\CIRCLE\\\CIRCLE\\\CIRCLE\\\CIRCLE\\\CIRCLE} \\
                                              &                                          & Poly-semantic Frames                & \LEFTcircle                         & \Circle                              & \Circle                            & \LEFTcircle                            & \LEFTcircle                            & {Unifying Sampling Points\\PIDS }                                                                                                    & {P\\D,P* }                               & {\LEFTcircle\\--}                                                             & {\Circle\\\Circle}                                                                & {\Circle\\\Circle}                                                                    & {\LEFTcircle\\\Circle}                                                        & {\LEFTcircle\\\Circle}                                                    \\
                                              &                                          & Frame Tampering                     & \LEFTcircle            & \Circle                 & \Circle               & \LEFTcircle               & \LEFTcircle               &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Double Receive                      & \LEFTcircle                         & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {ECU Guardian\\~Bit-Banger IDS\\Dynamic Fragmentation}                                                                               & {P\\D,P*\\P*}                            & {\LEFTcircle\\\LEFTcircle\\\CIRCLE}                                         & {\Circle\\\Circle\\\Circle}                                                     & {\Circle\\\Circle\\\Circle}                                                         & {\CIRCLE\\\Circle\\\CIRCLE}                                                 & {\LEFTcircle\\\CIRCLE\\\LEFTcircle}                                     \\
                                              &                                          & Polyglot Frames                     & \LEFTcircle                         & \Circle                              & \Circle                            & \LEFTcircle                            & \LEFTcircle                            &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Frame Tampering                     & \LEFTcircle                         & \Circle                              & \Circle                            & \LEFTcircle                            & \LEFTcircle                            &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Unorthodox Frames                   & \LEFTcircle                         & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Frame Hijacking                     & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {ID Anonymization\\Interframe-Spacing Anonymization}                                                                                 & {P\\P}                                   & {\LEFTcircle\\\LEFTcircle}                                                    & {\Circle\\\LEFTcircle}                                                            & {\Circle\\\LEFTcircle}                                                                & {\Circle\\\Circle}                                                            & {\CIRCLE\\\CIRCLE}                                                        \\
                                              &                                          & Clock-Skew Spoofing                 & \Circle                             & \Circle                              & \Circle                            & \Circle                                & \LEFTcircle                            & {Other PIDS\\Bit-Banger IDS}                                                                                                         & {D,P*\\D,P*}                             & {\CIRCLE\\\CIRCLE}                                                            & {\Circle\\\Circle}                                                                & {\Circle\\\Circle}                                                                    & {\Circle\\\Circle}                                                            & {\CIRCLE\\\CIRCLE}                                                        \\
                                              & \begin{sideways}Transwire\end{sideways}  & Physical-Fingerprint Distortion (higly)y    & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {ID Anonymization\\Interframe-Spacing Anonymization}                                                                                 & {P\\P}                                   & {\LEFTcircle\\\LEFTcircle}                                                    & {\Circle\\\LEFTcircle}                                                            & {\Circle\\\LEFTcircle}                                                                & {\Circle\\\Circle}                                                            & {\CIRCLE\\\CIRCLE}                                                        \\
                                              &                                          & Physical Architecture Manipulation  & \CIRCLE                             & \CIRCLE                              & \CIRCLE                            & \CIRCLE                                & \Circle                                & PIDS (Locator)                                                                                                                       & D                                        & \LEFTcircle                                                                     & \Circle                                                                             & \Circle                                                                                 & \CIRCLE                                                                         & \CIRCLE                                                                     \\
\begin{sideways}Availability\end{sideways}    & \begin{sideways}Higher\end{sideways}     & ECU Functionality Disabling         & \Circle                             & \Circle                              & \Circle                            & \LEFTcircle                            & \LEFTcircle                            & {Better Protocol Implementation\\Content Inspection \\ECU Guardian}                                                                  & {P\\D\\P}                                & {\CIRCLE\\\CIRCLE\\\CIRCLE}                                                 & {\Circle\\\Circle\\\Circle}                                                     & {\Circle\\\Circle\\\Circle}                                                         & {\Circle\\\Circle\\\CIRCLE}                                                 & {\LEFTcircle\\\LEFTcircle\\\CIRCLE}                                     \\
                                              &                                          & Higher-Layer Sybil Exhaustion       & \Circle                             & \Circle                              & \Circle                            & \LEFTcircle                            & \Circle                                &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Request Overwhelming                & \Circle                             & \Circle                              & \Circle                            & \LEFTcircle                            & \Circle                                &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              & \begin{sideways}Controller\end{sideways} & Error State Manipulation            & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & Disabling Automatic Retransmissions                                                                                                  & S                                        & \LEFTcircle                                                                     & \Circle                                                                             & \LEFTcircle                                                                             & \Circle                                                                         & \CIRCLE                                                                     \\
                                              &                                          & Error-Injection                     & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {Error Handling IDS\\ID Anonymization\\Interframe-Spacing Anonymization}                                                             & {D\\P\\D,P}                              & {\CIRCLE\\\LEFTcircle\\\LEFTcircle}                 & {\Circle\\\Circle\\\LEFTcircle}                             & {\Circle\\\Circle\\\LEFTcircle}                                 & {\Circle\\\Circle\\\Circle}                             & {\LEFTcircle\\\CIRCLE\\\CIRCLE}                     \\
                                              &                                          & Bus Access Denial                   & \Circle                             & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                & {Layer-II Node Suspension\\ID Priority Dissociation\\Dynamic Fragmentation \\ECU Guardian\\Bit-Banger IDS}                         & {P\\P\\P*\\P\\D}                         & {\LEFTcircle\\\LEFTcircle\\\CIRCLE\\\LEFTcircle~\\\CIRCLE}          & {\Circle\\\LEFTcircle\\\Circle\\\Circle\\\Circle}                           & {\Circle\\\CIRCLE\\\Circle\\\Circle~\\\Circle}                                  & {\Circle\\\CIRCLE\\\CIRCLE\\\CIRCLE\\\Circle}                           & {\CIRCLE\\\LEFTcircle\\\CIRCLE\\\CIRCLE\\\CIRCLE}                   \\
                                              & \begin{sideways}Transwire\end{sideways}  & Synchronization Disruption          & \LEFTcircle                         & \Circle                              & \Circle                            & \CIRCLE                                & \Circle                                &                                                                                                                                      &                                          &                                                                                   &                                                                                       &                                                                                           &                                                                                   &                                                                               \\
                                              &                                          & Signal Attenuation                  & \LEFTcircle                         & \Circle                              & \Circle                            & \CIRCLE                                & \CIRCLE                                & PIDS                                                                                                                                 & D                                        & \LEFTcircle                                                                     & \Circle                                                                             & \Circle                                                                                 & \Circle                                                                         & \LEFTcircle                                                                 
\end{tblr}
}
\end{table*}

==> Tables/defense_table.tex <==
% ================================================================
% PREAMBLE — add all of the following before \begin{document}
% Packages: \usepackage{array, multirow, graphicx, makecell, hhline}
%           \usepackage[table]{xcolor}
% ================================================================
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.90,0.70,0.60}
\definecolor{Manhattan}{rgb}{0.7600,0.7955,0.8992}
\definecolor{BurntOrange}{rgb}{0.3373, 0.4353, 0.7216}
\definecolor{Bobo}{RGB}{176,145,122}

\definecolor{SecureEfficient}{RGB}{34,139,34}
\definecolor{SecureOnly}{RGB}{140,150,60}
\definecolor{EfficientOnly}{RGB}{255,200,0}
\definecolor{Limited}{RGB}{195,100,210}

\newcolumntype{D}{>{\centering\arraybackslash}m{1.1cm}}

\newcommand{\datk}[1]{%
  \rotatebox[origin=c]{90}{\parbox{2.6cm}{\centering\small #1}}}

\newcommand{\tcell}[7]{%
  \cellcolor{#1}%
  \parbox[c]{\linewidth}{\centering
    \makebox[0.33\linewidth][c]{\footnotesize #2}%
    \makebox[0.33\linewidth][c]{\footnotesize #3}%
    \makebox[0.33\linewidth][c]{\footnotesize #4}\\[1pt]%
    \makebox[0.33\linewidth][c]{\footnotesize #5}%
    \makebox[0.33\linewidth][c]{\footnotesize #6}%
    \makebox[0.33\linewidth][c]{\footnotesize #7}}}

% ================================================================
\begin{table*}[!t]
\centering
\caption{CAN Defense Taxonomy and Effectiveness Assessment per Attack Category\\%
  \textbf{HL}: Higher Layer,\quad \textbf{CT}: Controller Layer,\quad \textbf{TW}: Transwire Layer}
\label{tbl:defense_taxonomy}
\label{tbl:bigtable}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{%
  |>{\centering\arraybackslash}m{0.42cm}%  col 1
  |>{\centering\arraybackslash}m{0.42cm}%  col 2
  |>{\centering\arraybackslash}m{2.5cm}%col 3
  |D|D|D|D|D%                              C1-C5
  |D|D|D|D|D|D|D|D|D|D%                   I1-I10
  |D|D|D|D|D|D|D|}%                        A1,A2,A3-A6,A8
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 1 : CIA grouping ====
\multicolumn{3}{|c|}{\multirow{3}{*}{\diagbox[width=3.6cm,height=3.48cm]{\raisebox{8ex}{\small\hspace{0.5cm}\textbf{Defenses}}}{\raisebox{-8ex}{\makebox[1.5cm][l]{\small\textbf{Attacks}}}}}} &
  \multicolumn{5}{c|}{\textbf{Confidentiality}} &
  \multicolumn{10}{c|}{\textbf{Integrity}} &
  \multicolumn{7}{c|}{\textbf{Availability}} \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 2 : Layer grouping ====
\multicolumn{3}{|c|}{} &
  \multicolumn{2}{c|}{\textbf{HL}}     &
  \multicolumn{1}{c|}{\textbf{CT}}     &
  \multicolumn{2}{c|}{\textbf{TW}}     &
  \multicolumn{3}{c|}{\textbf{HL}}     &
  \multicolumn{6}{c|}{\textbf{CT}}     &
  \multicolumn{1}{c|}{\textbf{TW}}     &
  \multicolumn{2}{c|}{\textbf{HL}}     &
  \multicolumn{4}{c|}{\textbf{CT}}     &
  \multicolumn{1}{c|}{\textbf{TW}}     \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 3 : Attack names ====
\multicolumn{3}{|c|}{} &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ca.\ Comm.\ Surveillance}}     &
  \datk{\Cb. Memory Leakage}          &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Cc. Network Reconnaissance}}    &
  \datk{\Cd. HW/Topology Profiling}    &
  \datk{\Ce. EM Emissions}            &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ia. Fake Data Fabrication}}   &
  \datk{\Ib. Mem./FW Manipulation}    &
  \datk{\Ic. Bypass Diag.\ Authentication}     &
  \datk{\cellcolor{Bobo}\Id. Impersonation \& Replay} &
  \datk{\cellcolor{Bobo}\Ie. Frame Hijacking}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\IF. Double Receive}}          &
  \datk{\cellcolor{Manhattan}\Ig. Unorthodox Frames}       &
  \datk{\Ih. Poly-Semantic Frames}    &
  \datk{\Ii. Frame Tampering}         &
  \datk{\cellcolor{Manhattan}\Ij. Physical FP Distortion}   &
  \datk{\Aa. ECU Func.\ Disabling}   &
  \datk{\Ab. Sybil Exhaustion}        &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ac. Error Injection}}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ad. Error State Manipulation}}      &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ae. Bus Access Denial}}       &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Af. Synchronization Disruption}}      &
  \datk{\Ag. Signal Attenuation}      \\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% CONFIDENTIALITY DEFENSES
%%------------------------------------------------------------------------------
\multirow{3}{*}{\rotatebox[origin=c]{90}{\small\textbf{Confidentiality}}}
& \rotatebox[origin=c]{90}{\small\textbf{HL}}
& \makecell[c]{\small\DCa.\ Encryption\\ \small \& Obfuscation}
%{\small\DCa.\ Encryption \& Obfuscation}
& \tcell{Limited}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\Circle$}{$\Circle$}{$\CIRCLE$}
& ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rotatebox[origin=c]{90}{\small\textbf{CT}}
& {\small\DCb.\ ID Anonymization}
& ~
& ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~
& ~ & ~ & ~
& ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rotatebox[origin=c]{90}{\small\textbf{TW}}
& {\small\DCc.\ Shielding \& Slope Control}
& ~  & ~  & ~  & ~
& \tcell{Limited}{- }{- }{$\Circle$}{- }{- }{-}
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% INTEGRITY DEFENSES
%%------------------------------------------------------------------------------
& \multirow{3}{*}{\rotatebox[origin=c]{90}{\small\textbf{HL~~~~~}}}
& {\small\DIb.\ Content Inspection}
& ~  & ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{D}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~
& ~
& ~  & ~  & ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  {\small\DIc.\ Patching \& Implementation}
& ~
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~
& ~
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~  & ~  & ~  & ~  & ~
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\multirow{10}{*}{\rotatebox[origin=c]{90}{\small\textbf{Integrity}}} & &
  {\small\DId.\ ECU FW Hardening}
& ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}
& ~  & ~  & ~
& ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}
& ~  & ~  & ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{4}{*}{\rotatebox[origin=c]{90}{\small\textbf{CT~~~~~~~~~~}}}
& {\small\DIa.\ Message Authentication}
& ~ & ~ & ~ & ~ & ~
& ~ & ~
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  {\small\DIF.\ Victim Resistance}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \tcell{SecureEfficient}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \makecell[c]{\small\DIi.\ Physical\\\small IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{D}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~
& ~  & ~
& \tcell{EfficientOnly}{D}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~
& \tcell{EfficientOnly}{D}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\makecell[c]{\small\DIg.\ Unify\\ \small Sample Points}
  %{\small\DIg.\ Unify Sample Points}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}
& ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{3}{*}{\rotatebox[origin=c]{90}{\small\textbf{TW~~~~~}}}
& {\small\DIh.\ Time \& IFS Anonymization}
& ~  & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~
& ~ & ~ & ~
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\LEFTcircle$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  {\small\DIj.\ Bit-Banger IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D,*}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{SecureEfficient}{D,*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  {\small\DIk.\ ECU Guardian}
& ~ & ~ & ~ & ~ & ~
& ~
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& ~
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{P}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& & &
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% AVAILABILITY DEFENSES
%%------------------------------------------------------------------------------
& \multirow{4}{*}{\rotatebox[origin=c]{90}{\small\textbf{CT~~~~~~~~~~}}} &
  {\small\DAc. Error Handling IDS}
& ~  & ~
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~
& ~ & ~ & ~
& ~
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{D}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~
& \tcell{EfficientOnly}{D}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\multirow{5}{*}{\rotatebox[origin=c]{90}{\small\textbf{Availability}}}
 & &
  {\small\DAd.\ L2 Node Suspension}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& \tcell{EfficientOnly}{P}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
{\small\DAa.\ ID-Priority Dissociation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \tcell{Limited}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\LEFTcircle$}{$\Circle$}{$\Circle$}
& \tcell{Limited}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\LEFTcircle$}{$\Circle$}{$\Circle$}
& \tcell{Limited}{P}{$\LEFTcircle$}{$\LEFTcircle$}{$\LEFTcircle$}{$\Circle$}{$\Circle$}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  {\small\DAb.\ One-Shot Mode}
& ~  & ~
& \tcell{EfficientOnly}{S}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~
& ~ & ~ & ~
& ~
& \tcell{EfficientOnly}{S}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~  & ~  & ~
& \tcell{EfficientOnly}{S}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~  & ~
& \tcell{EfficientOnly}{S}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rotatebox[origin=c]{90}{\small\textbf{TW}}
& {\small\DAe.\ Dynamic Fragmentation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& ~
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& ~  & ~
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
& \tcell{SecureOnly}{*}{$\CIRCLE$}{$\LEFTcircle$}{$\CIRCLE$}{$\CIRCLE$}{$\Circle$}
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\multicolumn{3}{|c|}{\multirow{2}{*}{\textbf{Cell Color}}} & \cellcolor{SecureEfficient}{} & \multicolumn{3}{c|}{Secure \& Lightweight} & \cellcolor{SecureOnly}{} & \multicolumn{2}{c|}{Secure} & {} & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Cell Content}}} & \multicolumn{4}{c|}{Insurance (\ins)} & \multicolumn{4}{c|}{Coverage (\cov)} & \multicolumn{4}{c|}{Validity (\val)} \\
\hhline{|~~~|-|-|-|-|-|-|-|~|~~|-|-|-|-|-|-|-|-|-|-|-|-|}
\multicolumn{3}{|c|}{} & \cellcolor{EfficientOnly}{} & \multicolumn{3}{c|}{Lightweight} & \cellcolor{Limited}{} & \multicolumn{2}{c|}{Limited}  & {} & \multicolumn{2}{c|}{} & \multicolumn{4}{c|}{ECU Operation Efficiency (\ecu)} & \multicolumn{4}{c|}{Bus Performance (\bus)} & \multicolumn{4}{c|}{Infra. Compatibility (\infra)}  \\
\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\end{tabular}%
}% end \resizebox
\end{table*}

==> Tables/defense_table2.tex <==
% ================================================================
% PREAMBLE — add all of the following before \begin{document}
% Packages: \usepackage{array, multirow, graphicx, makecell, hhline, amssymb, tikz}
%           \usepackage{diagbox}
%           \usepackage[table]{xcolor}
% ================================================================
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.90,0.70,0.60}
\definecolor{Manhattan}{rgb}{0.7600,0.7955,0.8992}
\definecolor{BurntOrange}{rgb}{0.3373, 0.4353, 0.7216}
\definecolor{Bobo}{RGB}{176,145,122}

% Verdict colors (kept consistent with defense_table.tex).
\definecolor{SecureEfficient}{RGB}{34,139,34}
\definecolor{SecureOnly}{RGB}{140,150,60}
\definecolor{EfficientOnly}{RGB}{255,200,0}
\definecolor{Limited}{RGB}{195,100,210}

% All 22 attack columns use the same wider fixed width.  The slightly
% narrower defense columns leave more horizontal room for the attack grid.
\newcolumntype{D}{>{\centering\arraybackslash}m{0.78cm}}

\newcommand{\datk}[1]{%
  \rotatebox[origin=c]{90}{\parbox{2.2cm}{\centering\footnotesize #1}}}

\newcommand{\tblhead}[1]{{\footnotesize\bfseries #1}}

% A fixed-height label makes every defense row equal, while the tighter
% baseline removes excess white space between two-line defense names.
\newlength{\DefenseRowHeight}
\setlength{\DefenseRowHeight}{0.64cm}
\newcommand{\dname}[1]{%
  \parbox[c][\DefenseRowHeight][c]{2.08cm}{%
    \centering\footnotesize\setlength{\baselineskip}{7.5pt}#1}}

% Explicit centered boxes keep every bold column and row heading centered in
% both directions.  Fixed-width multirow boxes also prevent long rotated
% category labels from shifting within the two narrow label columns.
\newlength{\DefenseColumnHeaderHeight}
\setlength{\DefenseColumnHeaderHeight}{0.36cm}
\newcommand{\columncategory}[1]{%
  \parbox[c][\DefenseColumnHeaderHeight][c]{2.3cm}{\centering\tblhead{#1}}}
\newcommand{\columnlayer}[1]{%
  \parbox[c][\DefenseColumnHeaderHeight][c]{0.55cm}{\centering\tblhead{#1}}}
% #2 compensates for the difference between multirow's array-strut height
% and the actual fixed defense-row height.  multirow treats a positive
% adjustment as upward, so these positive measurements are applied negatively.
\newcommand{\rowcategory}[3]{%
  \multirow[c]{#1}{0.36cm}[-#2]{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#3}}}}
\newcommand{\rowlayergroup}[3]{%
  \multirow[c]{#1}{0.36cm}[-#2]{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#3}}}}
\newcommand{\rowlayer}[1]{%
  \parbox[c][\DefenseRowHeight][c]{0.36cm}{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#1}}}}

\newlength{\DefenseHeaderWidth}
\newlength{\DefenseHeaderHeight}
\newcommand{\defensecorner}{%
  \begin{tikzpicture}[baseline=(current bounding box.center)]
    \path[use as bounding box] (0,0) rectangle
      (\DefenseHeaderWidth,\DefenseHeaderHeight);
    \draw[line width=\arrayrulewidth]
      (0,\DefenseHeaderHeight) -- (\DefenseHeaderWidth,0);
    \node[anchor=west,font=\footnotesize\bfseries]
      at (0.22cm,0.72cm) {Defenses};
    \node[anchor=east,font=\footnotesize\bfseries]
      at (\dimexpr\DefenseHeaderWidth-0.22cm\relax,2.28cm) {Attacks};
  \end{tikzpicture}}

% Each populated cell contains exactly two symbols, in this order:
%   (1) security assessment, (2) efficiency assessment.
% Security:  check = secure/effective; cross = security/effectiveness threshold not met.
% Efficiency: filled diamond = efficient; open diamond = efficiency threshold not met.
\newcommand{\SecureSymbol}{\ensuremath{\checkmark}}
\newcommand{\InsecureSymbol}{\ensuremath{\times}}
\newcommand{\EfficientSymbol}{\ensuremath{\blacklozenge}}
\newcommand{\InefficientSymbol}{\ensuremath{\lozenge}}

% Preserve the former four cell-verdict classes as a 2-by-2 symbol mapping.
\expandafter\def\csname overview@SecureEfficient\endcsname{%
  \SecureSymbol\hspace{0.22em}\EfficientSymbol}
\expandafter\def\csname overview@SecureOnly\endcsname{%
  \SecureSymbol\hspace{0.22em}\InefficientSymbol}
\expandafter\def\csname overview@EfficientOnly\endcsname{%
  \InsecureSymbol\hspace{0.22em}\EfficientSymbol}
\expandafter\def\csname overview@Limited\endcsname{%
  \InsecureSymbol\hspace{0.22em}\InefficientSymbol}

\newcommand{\ocell}[1]{%
  \cellcolor{#1}%
  \parbox[c][\DefenseRowHeight][c]{\linewidth}{%
    \centering\footnotesize\strut
    \raisebox{-0.20ex}{\csname overview@#1\endcsname}}}

% ================================================================
\begin{table*}[!t]
\centering
\caption{Overview of CAN Defense Security and Efficiency per Attack Category\\%
  \textbf{HL}: Higher Layer,\quad \textbf{CT}: Controller Layer,\quad \textbf{TW}: Transwire Layer}
\label{tbl:defense_taxonomy}
\label{tbl:bigtable}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{0.60}
\setlength{\DefenseHeaderWidth}{%
  \dimexpr2.92cm+6\tabcolsep+2\arrayrulewidth\relax}
\setlength{\DefenseHeaderHeight}{2.75cm}
\begin{tabular}{%
  |>{\centering\arraybackslash}m{0.36cm}%  col 1
  |>{\centering\arraybackslash}m{0.36cm}%  col 2
  |>{\centering\arraybackslash}m{2.2cm}%col 3
  |D|D|D|D|D%                              C1-C5
  |D|D|D|D|D|D|D|D|D|D%                   I1-I10
  |D|D|D|D|D|D|D|}%                        A1,A2,A3-A6,A8
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 1 : CIA grouping ====
\multicolumn{3}{|@{}c@{}|}{\multirow{3}{*}{\defensecorner}} &
  \multicolumn{5}{c|}{\columncategory{Confidentiality}} &
  \multicolumn{10}{c|}{\columncategory{Integrity}} &
  \multicolumn{7}{c|}{\columncategory{Availability}} \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 2 : Layer grouping ====
\multicolumn{3}{|c|}{} &
  \multicolumn{2}{c|}{\columnlayer{HL}}     &
  \multicolumn{1}{c|}{\columnlayer{CT}}     &
  \multicolumn{2}{c|}{\columnlayer{TW}}     &
  \multicolumn{3}{c|}{\columnlayer{HL}}     &
  \multicolumn{6}{c|}{\columnlayer{CT}}     &
  \multicolumn{1}{c|}{\columnlayer{TW}}     &
  \multicolumn{2}{c|}{\columnlayer{HL}}     &
  \multicolumn{4}{c|}{\columnlayer{CT}}     &
  \multicolumn{1}{c|}{\columnlayer{TW}}     \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 3 : Attack names ====
\multicolumn{3}{|c|}{} &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ca.\ Comm.\ Surveillance}}     &
  \datk{\Cb. Memory Leakage}          &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Cc. Network Reconnaissance}}    &
  \datk{\Cd. HW/Topology Profiling}    &
  \datk{\Ce. EM Emissions}            &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ia. Fake Data Fabrication}}   &
  \datk{\Ib. Mem./FW Manipulation}    &
  \datk{\Ic. Bypass Diag.\ Authentication}     &
  \datk{\cellcolor{Bobo}\Id. Impersonation \& Replay} &
  \datk{\cellcolor{Bobo}\Ie. Frame Hijacking}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\IF. Double Receive}}          &
  \datk{\cellcolor{Manhattan}\Ig. Unorthodox Frames}       &
  \datk{\Ih. Poly-Semantic Frames}    &
  \datk{\Ii. Frame Tampering}         &
  \datk{\cellcolor{Manhattan}\Ij. Physical FP Distortion}   &
  \datk{\Aa. ECU Func.\ Disabling}   &
  \datk{\Ab. Sybil Exhaustion}        &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ac. Error Injection}}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ad. Error State Manipulation}}      &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ae. Bus Access Denial}}       &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Af. Synchronization Disruption}}      &
  \datk{\Ag. Signal Attenuation}      \\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% CONFIDENTIALITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{3}{-0.04cm}{Confidentiality}
& \rowlayer{HL}
& \dname{\DCa.\ Encryption\\\& Obfuscation}
& \ocell{Limited}
& ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{CT}
& \dname{\DCb.\ ID Anonymization}
& ~
& ~
& \ocell{EfficientOnly}
& ~  & ~
& ~ & ~ & ~
& ~
& \ocell{EfficientOnly}
& ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{TW}
& \dname{\DCc.\ Shielding \&\\Slope Control}
& ~  & ~  & ~  & ~
& \ocell{Limited}
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% INTEGRITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{10}{1.79cm}{Integrity} & \rowlayergroup{3}{0.44cm}{HL}
& \dname{\DIb.\ Content Inspection}
& ~  & ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~
& ~
& ~  & ~  & ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIc.\ Patching \&\\Implementation}
& ~
& \ocell{SecureEfficient}
& ~  & ~  & ~
& ~
& \ocell{SecureEfficient}
& \ocell{SecureEfficient}
& ~  & ~  & ~  & ~  & ~  & ~  & ~
& \ocell{SecureEfficient}
& \ocell{SecureEfficient}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DId.\ ECU FW Hardening}
& ~
& \ocell{EfficientOnly}
& ~  & ~  & ~
& ~
& \ocell{EfficientOnly}
& ~  & ~  & ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayergroup{4}{0.63cm}{CT}
& \dname{\DIa.\ Message\\Authentication}
& ~ & ~ & ~ & ~ & ~
& ~ & ~
& \ocell{SecureEfficient}
& \ocell{SecureEfficient}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIF.\ Victim Resistance}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \ocell{SecureEfficient}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIi.\ Physical IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \ocell{SecureEfficient}
& ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& ~
& ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~  & ~
& \ocell{EfficientOnly}
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\dname{\DIg.\ Unify\\Sample Points}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayergroup{3}{0.44cm}{TW}
& \dname{\DIh.\ Time \& IFS\\Anonymization}
& ~  & ~
& \ocell{EfficientOnly}
& ~  & ~
& ~ & ~ & ~
& \ocell{SecureEfficient}
& \ocell{EfficientOnly}
& ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIj.\ Bit-Banger IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \ocell{SecureEfficient}
& \ocell{SecureEfficient}
& \ocell{EfficientOnly}
& \ocell{SecureEfficient}
& \ocell{SecureEfficient}
& \ocell{EfficientOnly}
& \ocell{SecureEfficient}
& ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIk.\ ECU Guardian}
& ~ & ~ & ~ & ~ & ~
& ~
& \ocell{SecureOnly}
& ~
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& & &
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% AVAILABILITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{5}{0.83cm}{Availability} & \rowlayergroup{4}{0.63cm}{CT} &
  \dname{\DAc. Error Handling IDS}
& ~  & ~
& \ocell{EfficientOnly}
& ~  & ~
& ~ & ~ & ~
& ~
& \ocell{EfficientOnly}
& ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& ~  & ~  & ~
& \ocell{EfficientOnly}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DAd.\ L2 Node Suspension}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& \ocell{EfficientOnly}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\dname{\DAa.\ ID-Priority\\Dissociation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \ocell{Limited}
& \ocell{Limited}
& \ocell{Limited}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DAb.\ One-Shot Mode}
& ~  & ~
& \ocell{EfficientOnly}
& ~  & ~
& ~ & ~ & ~
& ~
& \ocell{EfficientOnly}
& ~  & ~  & ~  & ~
& \ocell{EfficientOnly}
& ~  & ~  & ~
& \ocell{EfficientOnly}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{TW}
& \dname{\DAe.\ Dynamic\\Fragmentation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& ~
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& ~  & ~
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
& \ocell{SecureOnly}
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\multicolumn{25}{|c|}{%
  \makebox[\textwidth][c]{\footnotesize
  \SecureSymbol\ = Secure\quad
  \InsecureSymbol\ = Limited in Security\quad
  \EfficientSymbol\ = Efficient\quad
  \InefficientSymbol\ = Limited in Efficiency\quad}}\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\end{tabular}%
}% end \resizebox
\end{table*}


==> Tables/defense_table3.tex <==
% ================================================================
% PREAMBLE — add all of the following before \begin{document}
% Packages: \usepackage{array, multirow, graphicx, makecell, hhline, amssymb, tikz}
%           \usepackage{diagbox}
%           \usepackage[table]{xcolor}
% ================================================================
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.90,0.70,0.60}
\definecolor{Manhattan}{rgb}{0.7600,0.7955,0.8992}
\definecolor{BurntOrange}{rgb}{0.3373, 0.4353, 0.7216}
\definecolor{Bobo}{RGB}{176,145,122}

% Verdict colors (kept consistent with defense_table.tex).
\definecolor{SecureEfficient}{RGB}{34,139,34}
\definecolor{SecureOnly}{RGB}{140,150,60}
\definecolor{EfficientOnly}{RGB}{255,200,0}
\definecolor{Limited}{RGB}{195,100,210}

% All 22 attack columns use the same wider fixed width.  The slightly
% narrower defense columns leave more horizontal room for the attack grid.
\newcolumntype{D}{>{\centering\arraybackslash}m{0.78cm}}

\newcommand{\datk}[1]{%
  \rotatebox[origin=c]{90}{\parbox{2.2cm}{\centering\footnotesize #1}}}

\newcommand{\tblhead}[1]{{\footnotesize\bfseries #1}}

% A fixed-height label makes every defense row equal, while the tighter
% baseline removes excess white space between two-line defense names.
\newlength{\DefenseRowHeight}
\setlength{\DefenseRowHeight}{0.64cm}
\newcommand{\dname}[1]{%
  \parbox[c][\DefenseRowHeight][c]{2.08cm}{%
    \centering\footnotesize\setlength{\baselineskip}{7.5pt}#1}}

% Explicit centered boxes keep every bold column and row heading centered in
% both directions.  Fixed-width multirow boxes also prevent long rotated
% category labels from shifting within the two narrow label columns.
\newlength{\DefenseColumnHeaderHeight}
\setlength{\DefenseColumnHeaderHeight}{0.36cm}
\newcommand{\columncategory}[1]{%
  \parbox[c][\DefenseColumnHeaderHeight][c]{2.3cm}{\centering\tblhead{#1}}}
\newcommand{\columnlayer}[1]{%
  \parbox[c][\DefenseColumnHeaderHeight][c]{0.55cm}{\centering\tblhead{#1}}}
% #2 compensates for the difference between multirow's array-strut height
% and the actual fixed defense-row height.  multirow treats a positive
% adjustment as upward, so these positive measurements are applied negatively.
\newcommand{\rowcategory}[3]{%
  \multirow[c]{#1}{0.36cm}[-#2]{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#3}}}}
\newcommand{\rowlayergroup}[3]{%
  \multirow[c]{#1}{0.36cm}[-#2]{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#3}}}}
\newcommand{\rowlayer}[1]{%
  \parbox[c][\DefenseRowHeight][c]{0.36cm}{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#1}}}}

\newlength{\DefenseHeaderWidth}
\newlength{\DefenseHeaderHeight}
\newcommand{\defensecorner}{%
  \begin{tikzpicture}[baseline=(current bounding box.center)]
    \path[use as bounding box] (0,0) rectangle
      (\DefenseHeaderWidth,\DefenseHeaderHeight);
    \draw[line width=\arrayrulewidth]
      (0,\DefenseHeaderHeight) -- (\DefenseHeaderWidth,0);
    \node[anchor=west,font=\footnotesize\bfseries]
      at (0.22cm,0.72cm) {Defenses};
    \node[anchor=east,font=\footnotesize\bfseries]
      at (\dimexpr\DefenseHeaderWidth-0.22cm\relax,2.28cm) {Attacks};
  \end{tikzpicture}}

% Six-dimension cell encoding.  The four symbols use fixed quadrants:
%   top-left  = insurance (Ir), top-right = ECU efficiency (Ee),
%   bottom-left = bus performance (Bp), bottom-right = compatibility (Ic).
% Coverage controls the inset outline, validity controls its fill, and the
% original four-class verdict remains visible as the colored outer rim.
\expandafter\def\csname assessment@insurance@P\endcsname{\ensuremath{\mathrm{P}}}
\expandafter\def\csname assessment@insurance@D\endcsname{\ensuremath{\mathrm{D}}}
\expandafter\def\csname assessment@insurance@S\endcsname{\ensuremath{\mathrm{S}}}
\expandafter\def\csname assessment@insurance@DStar\endcsname{\ensuremath{\mathrm{D}^{*}}}
\expandafter\def\csname assessment@insurance@Star\endcsname{\ensuremath{{}^{*}}}
\expandafter\def\csname assessment@insurance@Missing\endcsname{\textendash}

\expandafter\def\csname assessment@level@High\endcsname{\ensuremath{\CIRCLE}}
\expandafter\def\csname assessment@level@Moderate\endcsname{\ensuremath{\LEFTcircle}}
\expandafter\def\csname assessment@level@Low\endcsname{\ensuremath{\Circle}}
\expandafter\def\csname assessment@level@Missing\endcsname{\textendash}

\expandafter\def\csname assessment@validity@Evaluated\endcsname{white}
\expandafter\def\csname assessment@validity@Analyzed\endcsname{black!15}
\expandafter\def\csname assessment@validity@Speculated\endcsname{black!55}

\tikzset{
  assessment coverage/Wide/.style={solid},
  assessment coverage/Restricted/.style={
    dash pattern=on 2.2pt off 1.0pt,
    line cap=butt
  }
}

\newcommand{\AssessmentInsurance}[1]{\csname assessment@insurance@#1\endcsname}
\newcommand{\AssessmentLevel}[1]{\csname assessment@level@#1\endcsname}
\newcommand{\AssessmentValidity}[1]{\csname assessment@validity@#1\endcsname}

\newcommand{\acell}[7]{%
  \cellcolor{#1}% legacy verdict rim
  \parbox[c][\DefenseRowHeight][c]{\linewidth}{%
    \centering
    \begin{tikzpicture}[baseline=(current bounding box.center)]
      \path[use as bounding box] (0,0) rectangle (0.64cm,0.50cm);
      \fill[fill=\AssessmentValidity{#7}]
        (0,0) rectangle (0.64cm,0.50cm);
      \draw[black,line width=0.45pt,assessment coverage/#3]
        (0.012cm,0.012cm) rectangle (0.628cm,0.488cm);
      \node[inner sep=0pt,font=\footnotesize] at (0.17cm,0.365cm)
        {\AssessmentInsurance{#2}};
      \node[inner sep=0pt,font=\footnotesize] at (0.47cm,0.365cm)
        {\AssessmentLevel{#4}};
      \node[inner sep=0pt,font=\footnotesize] at (0.17cm,0.135cm)
        {\AssessmentLevel{#5}};
      \node[inner sep=0pt,font=\footnotesize] at (0.47cm,0.135cm)
        {\AssessmentLevel{#6}};
    \end{tikzpicture}}}

\newcommand{\AssessmentFillSample}[1]{%
  \tikz[baseline=-0.45ex]{\draw[fill=#1,line width=0.3pt]
    (0,0) rectangle (0.20cm,0.12cm);}}
\newcommand{\AssessmentOutlineSample}[1]{%
  \tikz[baseline=-0.45ex]{\draw[line width=0.55pt,assessment coverage/#1]
    (0,0) rectangle (0.24cm,0.13cm);}}
\newcommand{\AssessmentRimSample}[1]{%
  \tikz[baseline=-0.45ex]{\fill[#1] (0,0) rectangle (0.20cm,0.12cm);}}

% ================================================================
\begin{table*}[!t]
\centering
\caption{Overview of CAN Defense Security and Efficiency per Attack Category\\%
  \textbf{HL}: Higher Layer,\quad \textbf{CT}: Controller Layer,\quad \textbf{TW}: Transwire Layer}
\label{tbl:defense_taxonomy}
\label{tbl:bigtable}
\begingroup
\footnotesize
\begin{tabular}{@{}c@{}}
Insurance (\ins, Top-Left): P/D/S = Prevention/Detection/Slowing,
$^{*}$ = Prevention When Combined With Another Approach \\[-0.1ex]
ECU Efficiency (\ecu, Top-Right),
Bus Performance (\bus, Bottom-Left),
Infrastructure Compatibility (\infra, Bottom-Right):
\CIRCLE/\LEFTcircle/\Circle\ = High/Moderate/Low \\[-0.1ex]
Coverage (\cov, Outline): \AssessmentOutlineSample{Wide}\ Wide,
\AssessmentOutlineSample{Restricted}\ Restricted\quad
Validity (\val, Fill): \AssessmentFillSample{white}\ Evaluated,
\AssessmentFillSample{black!15}\ Analyzed,
\AssessmentFillSample{black!55}\ Speculated \\[-0.1ex]
Overall Assessment (Rim):
\AssessmentRimSample{SecureEfficient}\ Secure \& Lightweight,
\AssessmentRimSample{SecureOnly}\ Secure,
\AssessmentRimSample{EfficientOnly}\ Lightweight,
\AssessmentRimSample{Limited}\ Limited
\end{tabular}
\par
\endgroup
\vspace{0.35ex}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{0.60}
\setlength{\DefenseHeaderWidth}{%
  \dimexpr2.92cm+6\tabcolsep+2\arrayrulewidth\relax}
\setlength{\DefenseHeaderHeight}{2.75cm}
\begin{tabular}{%
  |>{\centering\arraybackslash}m{0.36cm}%  col 1
  |>{\centering\arraybackslash}m{0.36cm}%  col 2
  |>{\centering\arraybackslash}m{2.2cm}%col 3
  |D|D|D|D|D%                              C1-C5
  |D|D|D|D|D|D|D|D|D|D%                   I1-I10
  |D|D|D|D|D|D|D|}%                        A1,A2,A3-A6,A8
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 1 : CIA grouping ====
\multicolumn{3}{|@{}c@{}|}{\multirow{3}{*}{\defensecorner}} &
  \multicolumn{5}{c|}{\columncategory{Confidentiality}} &
  \multicolumn{10}{c|}{\columncategory{Integrity}} &
  \multicolumn{7}{c|}{\columncategory{Availability}} \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 2 : Layer grouping ====
\multicolumn{3}{|c|}{} &
  \multicolumn{2}{c|}{\columnlayer{HL}}     &
  \multicolumn{1}{c|}{\columnlayer{CT}}     &
  \multicolumn{2}{c|}{\columnlayer{TW}}     &
  \multicolumn{3}{c|}{\columnlayer{HL}}     &
  \multicolumn{6}{c|}{\columnlayer{CT}}     &
  \multicolumn{1}{c|}{\columnlayer{TW}}     &
  \multicolumn{2}{c|}{\columnlayer{HL}}     &
  \multicolumn{4}{c|}{\columnlayer{CT}}     &
  \multicolumn{1}{c|}{\columnlayer{TW}}     \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 3 : Attack names ====
\multicolumn{3}{|c|}{} &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ca.\ Comm.\ Surveillance}}     &
  \datk{\Cb. Memory Leakage}          &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Cc. Network Reconnaissance}}    &
  \datk{\Cd. HW/Topology Profiling}    &
  \datk{\Ce. EM Emissions}            &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ia. Fake Data Fabrication}}   &
  \datk{\Ib. Mem./FW Manipulation}    &
  \datk{\Ic. Bypass Diag.\ Authentication}     &
  \datk{\cellcolor{Bobo}\Id. Impersonation \& Replay} &
  \datk{\cellcolor{Bobo}\Ie. Frame Hijacking}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\IF. Double Receive}}          &
  \datk{\cellcolor{Manhattan}\Ig. Unorthodox Frames}       &
  \datk{\Ih. Poly-Semantic Frames}    &
  \datk{\Ii. Frame Tampering}         &
  \datk{\cellcolor{Manhattan}\Ij. Physical FP Distortion}   &
  \datk{\Aa. ECU Func.\ Disabling}   &
  \datk{\Ab. Sybil Exhaustion}        &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ac. Error Injection}}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ad. Error State Manipulation}}      &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ae. Bus Access Denial}}       &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Af. Synchronization Disruption}}      &
  \datk{\Ag. Signal Attenuation}      \\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% CONFIDENTIALITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{3}{-0.04cm}{Confidentiality}
& \rowlayer{HL}
& \dname{\DCa.\ Encryption\\\& Obfuscation}
& \acell{Limited}{P}{Restricted}{High}{Low}{Low}{Evaluated}
& ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{CT}
& \dname{\DCb.\ ID Anonymization}
& ~
& ~
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~
& ~ & ~ & ~
& ~
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{TW}
& \dname{\DCc.\ Shielding \&\\Slope Control}
& ~  & ~  & ~  & ~
& \acell{Limited}{Missing}{Restricted}{Missing}{Missing}{Missing}{Speculated}
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% INTEGRITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{10}{1.79cm}{Integrity} & \rowlayergroup{3}{0.44cm}{HL}
& \dname{\DIb.\ Content Inspection}
& ~  & ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{DStar}{Wide}{High}{High}{High}{Evaluated}
& ~
& ~
& ~  & ~  & ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Wide}{Moderate}{High}{High}{Evaluated}
& \acell{EfficientOnly}{D}{Wide}{Moderate}{High}{High}{Evaluated}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIc.\ Patching \&\\Implementation}
& ~
& \acell{SecureEfficient}{P}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~  & ~
& ~
& \acell{SecureEfficient}{P}{Wide}{High}{High}{High}{Evaluated}
& \acell{SecureEfficient}{P}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~  & ~  & ~  & ~  & ~  & ~
& \acell{SecureEfficient}{P}{Wide}{Moderate}{High}{High}{Evaluated}
& \acell{SecureEfficient}{P}{Wide}{Moderate}{High}{High}{Evaluated}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DId.\ ECU FW Hardening}
& ~
& \acell{EfficientOnly}{P}{Restricted}{Moderate}{Moderate}{High}{Analyzed}
& ~  & ~  & ~
& ~
& \acell{EfficientOnly}{P}{Restricted}{Moderate}{Moderate}{High}{Analyzed}
& ~  & ~  & ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayergroup{4}{0.63cm}{CT}
& \dname{\DIa.\ Message\\Authentication}
& ~ & ~ & ~ & ~ & ~
& ~ & ~
& \acell{SecureEfficient}{P}{Wide}{High}{High}{High}{Evaluated}
& \acell{SecureEfficient}{DStar}{Wide}{High}{Moderate}{Moderate}{Evaluated}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIF.\ Victim Resistance}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{P}{Wide}{High}{High}{High}{Analyzed}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIi.\ Physical IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{DStar}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{High}{High}{High}{Evaluated}
& ~
& ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{D}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{Moderate}{High}{High}{Evaluated}
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\dname{\DIg.\ Unify\\Sample Points}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
& \acell{EfficientOnly}{P}{Restricted}{Moderate}{High}{High}{Analyzed}
& \acell{EfficientOnly}{P}{Restricted}{Moderate}{High}{High}{Analyzed}
& ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayergroup{3}{0.44cm}{TW}
& \dname{\DIh.\ Time \& IFS\\Anonymization}
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{High}{Moderate}{Moderate}{Evaluated}
& ~  & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{DStar}{Wide}{High}{Moderate}{Moderate}{Evaluated}
& \acell{EfficientOnly}{P}{Restricted}{High}{Moderate}{Moderate}{Evaluated}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{High}{Moderate}{Moderate}{Evaluated}
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{High}{Moderate}{Moderate}{Evaluated}
& \acell{EfficientOnly}{P}{Restricted}{High}{Moderate}{Moderate}{Evaluated}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIj.\ Bit-Banger IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{DStar}{Wide}{High}{High}{High}{Evaluated}
& \acell{SecureEfficient}{DStar}{Wide}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& \acell{SecureEfficient}{DStar}{Wide}{High}{High}{High}{Evaluated}
& \acell{SecureEfficient}{DStar}{Wide}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{DStar}{Restricted}{High}{High}{High}{Evaluated}
& \acell{SecureEfficient}{DStar}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIk.\ ECU Guardian}
& ~ & ~ & ~ & ~ & ~
& ~
& \acell{SecureOnly}{P}{Wide}{Moderate}{High}{High}{Speculated}
& ~
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{P}{Wide}{High}{High}{High}{Speculated}
& & &
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% AVAILABILITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{5}{0.83cm}{Availability} & \rowlayergroup{4}{0.63cm}{CT} &
  \dname{\DAc. Error Handling IDS}
& ~  & ~
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~
& ~ & ~ & ~
& ~
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~  & ~
& \acell{EfficientOnly}{D}{Wide}{High}{High}{High}{Evaluated}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DAd.\ L2 Node Suspension}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& \acell{EfficientOnly}{P}{Restricted}{High}{High}{High}{Evaluated}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\dname{\DAa.\ ID-Priority\\Dissociation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \acell{Limited}{P}{Restricted}{Moderate}{Moderate}{Low}{Speculated}
& \acell{Limited}{P}{Restricted}{Moderate}{Moderate}{Low}{Speculated}
& \acell{Limited}{P}{Restricted}{Moderate}{Moderate}{Low}{Speculated}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DAb.\ One-Shot Mode}
& ~  & ~
& \acell{EfficientOnly}{S}{Restricted}{High}{High}{Moderate}{Evaluated}
& ~  & ~
& ~ & ~ & ~
& ~
& \acell{EfficientOnly}{S}{Restricted}{High}{High}{Moderate}{Evaluated}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{S}{Restricted}{High}{High}{Moderate}{Evaluated}
& ~  & ~  & ~
& \acell{EfficientOnly}{S}{Restricted}{High}{High}{Moderate}{Evaluated}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{TW}
& \dname{\DAe.\ Dynamic\\Fragmentation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& ~
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
& ~  & ~
& \acell{SecureOnly}{Star}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{High}{High}{High}{Speculated}
& \acell{SecureOnly}{Star}{Wide}{Moderate}{High}{High}{Speculated}
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\end{tabular}%
}% end \resizebox
\end{table*}


==> Tables/defense_table4.tex <==
% ================================================================
% PREAMBLE — add all of the following before \begin{document}
% Packages: \usepackage{array, multirow, graphicx, makecell, hhline, amssymb, tikz}
%           \usepackage{diagbox}
%           \usepackage[table]{xcolor}
% ================================================================
\definecolor{Matrix}{rgb}{0.65,0.301,0.301}
\definecolor{BeautyBush}{rgb}{0.90,0.70,0.60}
\definecolor{Manhattan}{rgb}{0.7600,0.7955,0.8992}
\definecolor{BurntOrange}{rgb}{0.3373, 0.4353, 0.7216}
\definecolor{Bobo}{RGB}{176,145,122}
\usetikzlibrary{patterns}

% Verdict colors (kept consistent with defense_table.tex).
\definecolor{SecureEfficient}{RGB}{34,139,34}
\definecolor{SecureOnly}{RGB}{140,150,60}
\definecolor{EfficientOnly}{RGB}{255,200,0}
\definecolor{Limited}{RGB}{195,100,210}

% All 22 attack columns use the same wider fixed width.  The slightly
% narrower defense columns leave more horizontal room for the attack grid.
\newcolumntype{D}{@{}>{\centering\arraybackslash}m{0.78cm}@{}}

\newcommand{\datk}[1]{%
  \rotatebox[origin=c]{90}{\parbox{2.2cm}{\centering\footnotesize #1}}}

\newcommand{\tblhead}[1]{{\footnotesize\bfseries #1}}

% A fixed-height label makes every defense row equal, while the tighter
% baseline removes excess white space between two-line defense names.
\newlength{\DefenseRowHeight}
\setlength{\DefenseRowHeight}{0.64cm}
\newcommand{\dname}[1]{%
  \parbox[c][\DefenseRowHeight][c]{2.08cm}{%
    \centering\footnotesize\setlength{\baselineskip}{7.5pt}#1}}

% Explicit centered boxes keep every bold column and row heading centered in
% both directions.  Fixed-width multirow boxes also prevent long rotated
% category labels from shifting within the two narrow label columns.
\newlength{\DefenseColumnHeaderHeight}
\setlength{\DefenseColumnHeaderHeight}{0.36cm}
\newcommand{\columncategory}[1]{%
  \parbox[c][\DefenseColumnHeaderHeight][c]{2.3cm}{\centering\tblhead{#1}}}
\newcommand{\columnlayer}[1]{%
  \parbox[c][\DefenseColumnHeaderHeight][c]{0.55cm}{\centering\tblhead{#1}}}
% #2 compensates for the difference between multirow's array-strut height
% and the actual fixed defense-row height.  multirow treats a positive
% adjustment as upward, so these positive measurements are applied negatively.
\newcommand{\rowcategory}[3]{%
  \multirow[c]{#1}{0.36cm}[-#2]{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#3}}}}
\newcommand{\rowlayergroup}[3]{%
  \multirow[c]{#1}{0.36cm}[-#2]{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#3}}}}
\newcommand{\rowlayer}[1]{%
  \parbox[c][\DefenseRowHeight][c]{0.36cm}{%
    \centering\rotatebox[origin=c]{90}{\tblhead{#1}}}}

\newlength{\DefenseHeaderWidth}
\newlength{\DefenseHeaderHeight}
\newcommand{\defensecorner}{%
  \begin{tikzpicture}[baseline=(current bounding box.center)]
    \path[use as bounding box] (0,0) rectangle
      (\DefenseHeaderWidth,\DefenseHeaderHeight);
    \draw[line width=\arrayrulewidth]
      (0,\DefenseHeaderHeight) -- (\DefenseHeaderWidth,0);
    \node[anchor=west,font=\footnotesize\bfseries]
      at (0.22cm,0.72cm) {Defenses};
    \node[anchor=east,font=\footnotesize\bfseries]
      at (\dimexpr\DefenseHeaderWidth-0.22cm\relax,2.28cm) {Attacks};
  \end{tikzpicture}}

% Six-dimension cell encoding. Each populated attack-defense cell is a 1x3
% strip. The symbols report insurance, coverage, and validity, respectively.
% Their backgrounds report ECU efficiency, bus performance, and infrastructure
% compatibility using one shared high/moderate/low color scale. A hatched
% texture marks cells that satisfy the paper's effective-defense threshold.
\expandafter\def\csname assessment@insurance@P\endcsname{\ensuremath{\mathrm{P}}}
\expandafter\def\csname assessment@insurance@D\endcsname{\ensuremath{\mathrm{D}}}
\expandafter\def\csname assessment@insurance@S\endcsname{\ensuremath{\mathrm{S}}}
\expandafter\def\csname assessment@insurance@DStar\endcsname{\scalebox{0.68}{$\mathrm{D}^{*}$}}
\expandafter\def\csname assessment@insurance@Star\endcsname{\scalebox{0.78}{$*$}}
\expandafter\def\csname assessment@insurance@Missing\endcsname{\textendash}

\expandafter\def\csname assessment@coverage@Wide\endcsname{\ensuremath{\CIRCLE}}
\expandafter\def\csname assessment@coverage@Restricted\endcsname{\ensuremath{\LEFTcircle}}
\expandafter\def\csname assessment@coverage@Missing\endcsname{\textendash}

\expandafter\def\csname assessment@validity@Evaluated\endcsname{\ensuremath{\CIRCLE}}
\expandafter\def\csname assessment@validity@Analyzed\endcsname{\ensuremath{\LEFTcircle}}
\expandafter\def\csname assessment@validity@Speculated\endcsname{\ensuremath{\Circle}}
\expandafter\def\csname assessment@validity@Missing\endcsname{\textendash}

\definecolor{AssessmentHigh}{RGB}{198,232,198}
\definecolor{AssessmentModerate}{RGB}{250,221,142}
\definecolor{AssessmentLow}{RGB}{239,183,183}
\definecolor{AssessmentMissing}{RGB}{238,238,238}

\expandafter\def\csname assessment@color@High\endcsname{AssessmentHigh}
\expandafter\def\csname assessment@color@Moderate\endcsname{AssessmentModerate}
\expandafter\def\csname assessment@color@Low\endcsname{AssessmentLow}
\expandafter\def\csname assessment@color@Missing\endcsname{AssessmentMissing}

% Effectiveness is derived from the six criteria rather than from the legacy
% four-class verdict. Prevention (including prevention by combination), wide
% coverage, at least analyzed validity, and at least moderate values for all
% three practical criteria are required.
\expandafter\def\csname assessment@effective@insurance@P\endcsname{}
\expandafter\def\csname assessment@effective@insurance@DStar\endcsname{}
\expandafter\def\csname assessment@effective@insurance@Star\endcsname{}
\expandafter\def\csname assessment@effective@coverage@Wide\endcsname{}
\expandafter\def\csname assessment@effective@level@High\endcsname{}
\expandafter\def\csname assessment@effective@level@Moderate\endcsname{}
\expandafter\def\csname assessment@effective@validity@Evaluated\endcsname{}
\expandafter\def\csname assessment@effective@validity@Analyzed\endcsname{}

\newcommand{\AssessmentInsurance}[1]{\csname assessment@insurance@#1\endcsname}
\newcommand{\AssessmentCoverage}[1]{\csname assessment@coverage@#1\endcsname}
\newcommand{\AssessmentValidity}[1]{\csname assessment@validity@#1\endcsname}
\newcommand{\AssessmentColor}[1]{\csname assessment@color@#1\endcsname}
\newcommand{\AssessmentEffectTexture}[6]{%
  \ifcsname assessment@effective@insurance@#1\endcsname
    \ifcsname assessment@effective@coverage@#2\endcsname
      \ifcsname assessment@effective@level@#3\endcsname
        \ifcsname assessment@effective@level@#4\endcsname
          \ifcsname assessment@effective@level@#5\endcsname
            \ifcsname assessment@effective@validity@#6\endcsname
              \fill[pattern=north east lines,pattern color=black!38]
                (0.02cm,0.02cm) rectangle (0.76cm,0.62cm);
            \fi
          \fi
        \fi
      \fi
    \fi
  \fi}

\newcommand{\acell}[7]{%
  \begin{tikzpicture}[baseline=(current bounding box.center)]
      \path[use as bounding box] (0,0) rectangle (0.78cm,0.64cm);
      \fill[\AssessmentColor{#5}]
        (0.02cm,0.02cm) rectangle (0.2667cm,0.62cm);
      \fill[\AssessmentColor{#6}]
        (0.2667cm,0.02cm) rectangle (0.5133cm,0.62cm);
      \fill[\AssessmentColor{#7}]
        (0.5133cm,0.02cm) rectangle (0.76cm,0.62cm);
      \AssessmentEffectTexture{#2}{#3}{#5}{#6}{#7}{#4}
      \draw[black!55,line width=0.22pt]
        (0.2667cm,0.02cm) -- (0.2667cm,0.62cm);
      \draw[black!55,line width=0.22pt]
        (0.5133cm,0.02cm) -- (0.5133cm,0.62cm);
      \node[inner sep=0pt,font=\tiny] at (0.1433cm,0.32cm)
        {\AssessmentInsurance{#2}};
      \node[inner sep=0pt,font=\tiny] at (0.39cm,0.32cm)
        {\AssessmentCoverage{#3}};
      \node[inner sep=0pt,font=\tiny] at (0.6367cm,0.32cm)
        {\AssessmentValidity{#4}};
  \end{tikzpicture}}

\newcommand{\AssessmentColorSample}[1]{%
  \tikz[baseline=-0.45ex]{\draw[fill=\AssessmentColor{#1},line width=0.3pt]
    (0,0) rectangle (0.20cm,0.12cm);}}
\newcommand{\AssessmentTextureSample}[1]{%
  \tikz[baseline=-0.45ex]{%
    \path[use as bounding box] (0,0) rectangle (0.24cm,0.13cm);
    \ifnum#1=1
      \fill[pattern=north east lines,pattern color=black!38]
        (0,0) rectangle (0.24cm,0.13cm);
    \fi
    \draw[black,line width=0.3pt]
      (0,0) rectangle (0.24cm,0.13cm);}}
\newcommand{\AssessmentTripletSample}{%
  \tikz[baseline=-0.55ex]{%
    \fill[AssessmentHigh] (0,0) rectangle (0.18cm,0.18cm);
    \fill[AssessmentModerate] (0.18cm,0) rectangle (0.36cm,0.18cm);
    \fill[AssessmentLow] (0.36cm,0) rectangle (0.54cm,0.18cm);
    \draw[black,line width=0.25pt] (0.18cm,0)--(0.18cm,0.18cm)
      (0.36cm,0)--(0.36cm,0.18cm);
    \fill[pattern=north east lines,pattern color=black!38]
      (0,0) rectangle (0.54cm,0.18cm);
    \node[font=\tiny,inner sep=0pt] at (0.09cm,0.09cm) {P};
    \node[font=\tiny,inner sep=0pt] at (0.27cm,0.09cm) {$\CIRCLE$};
    \node[font=\tiny,inner sep=0pt] at (0.45cm,0.09cm) {$\LEFTcircle$};}}

% ================================================================
\begin{table*}[!t]
\centering
\caption{Overview of CAN Defense Security and Efficiency per Attack Category\\%
  \textbf{HL}: Higher Layer,\quad \textbf{CT}: Controller Layer,\quad \textbf{TW}: Transwire Layer}
\label{tbl:defense_taxonomy}
\label{tbl:bigtable}
\begingroup
\footnotesize
\begin{tabular}{@{}c@{}}
Cell symbols (left to right):
Insurance (\ins), Coverage (\cov), Validity (\val) \\[-0.1ex]
Insurance: P/D/S = Prevention/Detection/Slowing;
$^{*}$ = Prevention only when combined with another approach \\[-0.1ex]
Coverage: \CIRCLE/\LEFTcircle\ = Wide/Restricted\quad
Validity: \CIRCLE/\LEFTcircle/\Circle\ = Evaluated/Analyzed/Speculated \\[-0.1ex]
Background color (left to right): ECU Efficiency (\ecu),
Bus Performance (\bus), Infrastructure Compatibility (\infra)\\[-0.1ex]
\AssessmentColorSample{High}\ High,
\AssessmentColorSample{Moderate}\ Moderate,
\AssessmentColorSample{Low}\ Low \\[-0.1ex]
Background texture: \AssessmentTextureSample{1}\ Effective Defense,
\AssessmentTextureSample{0}\ Limited
\end{tabular}
\par
\endgroup
\vspace{0.35ex}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{0.60}
\setlength{\DefenseHeaderWidth}{%
  \dimexpr2.92cm+6\tabcolsep+2\arrayrulewidth\relax}
\setlength{\DefenseHeaderHeight}{2.75cm}
\begin{tabular}{%
  |>{\centering\arraybackslash}m{0.36cm}%  col 1
  |>{\centering\arraybackslash}m{0.36cm}%  col 2
  |>{\centering\arraybackslash}m{2.2cm}%col 3
  |D|D|D|D|D%                              C1-C5
  |D|D|D|D|D|D|D|D|D|D%                   I1-I10
  |D|D|D|D|D|D|D|}%                        A1,A2,A3-A6,A8
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 1 : CIA grouping ====
\multicolumn{3}{|@{}c@{}|}{\multirow{3}{*}{\defensecorner}} &
  \multicolumn{5}{c|}{\columncategory{Confidentiality}} &
  \multicolumn{10}{c|}{\columncategory{Integrity}} &
  \multicolumn{7}{c|}{\columncategory{Availability}} \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 2 : Layer grouping ====
\multicolumn{3}{|c|}{} &
  \multicolumn{2}{c|}{\columnlayer{HL}}     &
  \multicolumn{1}{c|}{\columnlayer{CT}}     &
  \multicolumn{2}{c|}{\columnlayer{TW}}     &
  \multicolumn{3}{c|}{\columnlayer{HL}}     &
  \multicolumn{6}{c|}{\columnlayer{CT}}     &
  \multicolumn{1}{c|}{\columnlayer{TW}}     &
  \multicolumn{2}{c|}{\columnlayer{HL}}     &
  \multicolumn{4}{c|}{\columnlayer{CT}}     &
  \multicolumn{1}{c|}{\columnlayer{TW}}     \\
\hhline{|~~~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
%%==== HEADER ROW 3 : Attack names ====
\multicolumn{3}{|c|}{} &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ca.\ Comm.\ Surveillance}}     &
  \datk{\Cb. Memory Leakage}          &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Cc. Network Reconnaissance}}    &
  \datk{\Cd. HW/Topology Profiling}    &
  \datk{\Ce. EM Emissions}            &
  \datk{\cellcolor{Matrix}\textcolor{white}{\Ia. Fake Data Fabrication}}   &
  \datk{\Ib. Mem./FW Manipulation}    &
  \datk{\Ic. Bypass Diag.\ Authentication}     &
  \datk{\cellcolor{Bobo}\Id. Impersonation \& Replay} &
  \datk{\cellcolor{Bobo}\Ie. Frame Hijacking}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\IF. Double Receive}}          &
  \datk{\cellcolor{Manhattan}\Ig. Unorthodox Frames}       &
  \datk{\Ih. Poly-Semantic Frames}    &
  \datk{\Ii. Frame Tampering}         &
  \datk{\cellcolor{Manhattan}\Ij. Physical FP Distortion}   &
  \datk{\Aa. ECU Func.\ Disabling}   &
  \datk{\Ab. Sybil Exhaustion}        &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ac. Error Injection}}         &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ad. Error State Manipulation}}      &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Ae. Bus Access Denial}}       &
  \datk{\cellcolor{BurntOrange}\textcolor{white}{\Af. Synchronization Disruption}}      &
  \datk{\Ag. Signal Attenuation}      \\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% CONFIDENTIALITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{3}{-0.04cm}{Confidentiality}
& \rowlayer{HL}
& \dname{\DCa.\ Encryption\\\& Obfuscation}
& \acell{Limited}{P}{Restricted}{Evaluated}{Low}{Low}{High}
& ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{CT}
& \dname{\DCb.\ ID Anonymization}
& ~
& ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~
& ~ & ~ & ~
& ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{TW}
& \dname{\DCc.\ Shielding \&\\Slope Control}
& ~  & ~  & ~  & ~
& \acell{Limited}{Missing}{Missing}{Missing}{Missing}{Missing}{Low}
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% INTEGRITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{10}{1.79cm}{Integrity} & \rowlayergroup{3}{0.44cm}{HL}
& \dname{\DIb.\ Content Inspection}
& ~  & ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{DStar}{Wide}{Evaluated}{High}{High}{High}
& ~
& ~
& ~  & ~  & ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Wide}{Analyzed}{High}{High}{High}
& \acell{EfficientOnly}{D}{Wide}{Analyzed}{High}{High}{High}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIc.\ Patching \&\\Implementation}
& ~
& \acell{SecureEfficient}{P}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~  & ~
& ~
& \acell{SecureEfficient}{P}{Wide}{Evaluated}{High}{High}{High}
& \acell{SecureEfficient}{P}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~  & ~  & ~  & ~  & ~  & ~
& \acell{SecureEfficient}{P}{Wide}{Analyzed}{High}{High}{High}
& \acell{SecureEfficient}{P}{Wide}{Analyzed}{High}{High}{High}
& ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DId.\ ECU FW Hardening}
& ~
& \acell{EfficientOnly}{P}{Restricted}{Analyzed}{Moderate}{High}{Moderate}
& ~  & ~  & ~
& ~
& \acell{EfficientOnly}{P}{Restricted}{Analyzed}{Moderate}{High}{Moderate}
& ~  & ~  & ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayergroup{4}{0.63cm}{CT}
& \dname{\DIa.\ Message\\Authentication}
& ~ & ~ & ~ & ~ & ~
& ~ & ~
& \acell{SecureEfficient}{P}{Wide}{Evaluated}{High}{High}{High}
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{Moderate}{Moderate}{High}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIF.\ Victim Resistance}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{P}{Wide}{Evaluated}{High}{High}{Moderate}
& ~  & ~  & ~  & ~  & ~  & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIi.\ Physical IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{Evaluated}{High}{High}{High}
& ~
& ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{D}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{Analyzed}{High}{High}{High}
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\dname{\DIg.\ Unify\\Sample Points}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
& \acell{EfficientOnly}{P}{Restricted}{Analyzed}{High}{High}{Moderate}
& \acell{EfficientOnly}{P}{Restricted}{Analyzed}{High}{High}{Moderate}
& ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayergroup{3}{0.44cm}{TW}
& \dname{\DIh.\ Time \& IFS\\Anonymization}
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{Moderate}{Moderate}{High}
& ~  & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{Moderate}{Moderate}{High}
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{Moderate}{Moderate}{High}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{Moderate}{Moderate}{High}
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{Moderate}{Moderate}{High}
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{Moderate}{Moderate}{High}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIj.\ Bit-Banger IDS}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{High}{High}{High}
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{High}{High}{High}
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{DStar}{Restricted}{Evaluated}{High}{High}{High}
& \acell{SecureEfficient}{DStar}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DIk.\ ECU Guardian}
& ~ & ~ & ~ & ~ & ~
& ~
& \acell{SecureOnly}{P}{Wide}{Analyzed}{High}{High}{Low}
& ~
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{P}{Wide}{Evaluated}{High}{High}{Low}
& & &
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}

%%------------------------------------------------------------------------------
%% AVAILABILITY DEFENSES
%%------------------------------------------------------------------------------
\rowcategory{5}{0.83cm}{Availability} & \rowlayergroup{4}{0.63cm}{CT} &
  \dname{\DAc. Error Handling IDS}
& ~  & ~
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~
& ~ & ~ & ~
& ~
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{D}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~  & ~
& \acell{EfficientOnly}{D}{Wide}{Evaluated}{High}{High}{High}
& ~  & ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DAd.\ L2 Node Suspension}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& \acell{EfficientOnly}{P}{Restricted}{Evaluated}{High}{High}{High}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
\dname{\DAa.\ ID-Priority\\Dissociation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~
& ~  & ~
& \acell{Limited}{P}{Restricted}{Analyzed}{Moderate}{Low}{Low}
& \acell{Limited}{P}{Restricted}{Analyzed}{Moderate}{Low}{Low}
& \acell{Limited}{P}{Restricted}{Analyzed}{Moderate}{Low}{Low}
& ~  & ~
\\
\hhline{|~|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& &
  \dname{\DAb.\ One-Shot Mode}
& ~  & ~
& \acell{EfficientOnly}{S}{Restricted}{Evaluated}{High}{Moderate}{High}
& ~  & ~
& ~ & ~ & ~
& ~
& \acell{EfficientOnly}{S}{Restricted}{Evaluated}{High}{Moderate}{High}
& ~  & ~  & ~  & ~
& \acell{EfficientOnly}{S}{Restricted}{Evaluated}{High}{Moderate}{High}
& ~  & ~  & ~
& \acell{EfficientOnly}{S}{Restricted}{Evaluated}{High}{Moderate}{High}
& ~  & ~  & ~
\\
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \rowlayer{TW}
& \dname{\DAe.\ Dynamic\\Fragmentation}
& ~ & ~ & ~ & ~ & ~
& ~ & ~ & ~
& ~
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
& ~  & ~
& \acell{SecureOnly}{Star}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Evaluated}{High}{High}{Low}
& \acell{SecureOnly}{Star}{Wide}{Analyzed}{High}{High}{Low}
\\
\hhline{|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
\end{tabular}%
}% end \resizebox
\end{table*}


==> sec7_GapsRevised.tex <==
\section{Root Cause Analysis}
\label{A:Analysis}
\label{A:ResearchGaps}



In this section, we analyze whether CAN security problems stem from the CAN specifications, are \textit{unique} to them, or neither. We identify a set of shared root causes and map CAN attacks and defense gaps to each of them. For each root cause, we determine whether it is \textit{inherent}, \textit{unique}, or both, and then use that analysis to infer which attacks and gaps are themselves inherent or unique to CAN. Because an attack or gap may have multiple root causes, and a root cause may underlie multiple attacks or gaps, the next two subsections are organized by root cause, with each root cause followed by the attacks or gaps it underlies. 

Tbl. \ref{tbl:root_cause} summarizes these root causes and the attacks or gaps they underlie. Our analysis identifies 9 attack root causes ($\mathcal{R}$) and 3 defense-gap root causes ($\mathcal{DR}$). \textit{By-the-ruler} gaps are highlighted in \textit{red}, and \textit{bit-banger} gaps are highlighted in blue. A \checkmark indicates that a root cause is indispensable to the attack or gap. For attacks, an $\uparrow$ indicates that addressing the root cause provides an effective defense. A root cause may have two non-mutually-exclusive qualities: \textit{1) Inherency (I):} stemming from the CAN standard specification rather than from accidental implementation or deployment choices. \textit{2) Uniqueness (U):} specific to the CAN family of standards.



\subsection{Attack Root Causes}\label{subsec:root_cause}
\label{subsec:attack_rc} 

\kha{revise attack names, numbers and references to tables after changes are settled}



\shortsectionEmph{$\mathcal{R}$1: Attacker Access to Network (I).} The mere access of the attacker to the network, whether physically or remotely, is \textit{inherent} to all of our attacker models (Sec. \ref{subsec:BusAccess}) and all attacks require it. While most attacks require additional root causes with it, it is enough for \textit{fake data fabrication}. It is \textit{not unique}, as any comparison with other communication systems will assume it under any attacker model. 

\shortsectionEmph{$\mathcal{R}$2: Shared Media Properties (I).} Two \textit{inherent} properties that are \textit{not unique} to CAN, but common to all single-channel shared communication media and exploitable by all our attacker models, underlie many attacks. \textit{1) Broadcast promiscuity:} this refers to the ability of a connected malicious node to anonymously monitor bus-wide activity and to have bus-wide reachability, allowing it to act on any observed frame, node, or the medium itself. This directly enables \textit{communication surveillance}, \textit{network reconnaissance}, and \textit{hardware and topology profiling} attacks. It also underlies attacks that interfere with in-flight frames (\Ie, \Ij, and \Ag), attacks that induce errors or manipulate node state (\Ac~and \Ad), attacks that exploit discrepancies among nodes sharing the same bus (\Ih, \Af, \IF, \Id). \textit{2) Mutual exclusion:} because transmission on a single shared channel prevents other nodes from transmitting at the same time, it gives an adversary leverage to deny others bus access or seize transmission opportunities, thereby underlying \textit{bus-access denial} and \textit{frame hijacking}.




\shortsectionEmph{$\mathcal{R}$3: Exploitable Priority System (I).} As described in Sec. \ref{sec:background}, CAN uses a bus-wide priority mechanism, physically prioritizing dominant voltage over recessive. On the controller layer, this is utilized for collision resolution using arbitration, where lower CAN IDs (more leading dominant bits) have higher priority. This enables \textit{bus-access denial}, whether by flooding the bus with low-CAN-ID frames or by continuously asserting dominant voltage. It also enables attacks that transmit past arbitration (\textit{network reconnaissance}, \textit{frame hijacking}, \textit{physical fingerprint distortion}, and \textit{error injection and state manipulation}), whether by matching the ID with victim messages to exploit the simultaneous-transmission technique for by-the-rulers (Sec. \ref{subsubsec:simultaneous}), or by directly flipping recessive voltage to dominant for \textit{bit-bangers}. While this root-cause is \textit{inherent} and exploitable by all attacker models, it is \textit{not unique} as all shared media need priority and media access systems--many of which are exploitable, as shown in Sec. \ref{sec:investigat}.




\shortsectionEmph{$\mathcal{R}$4: Error Handling Properties (IU).} Four \textit{inherent and unique} properties of CAN's error handling mechanism are exploited by attackers: 1) it defines different criteria for frame validity between senders and receivers, allowing attackers to exploit this discrepancy (\IF). 2) the types of errors and their impact, namely halting transmission and raising an error frame, as well as 3) the presence of behaviorally distinct error states, are exploited in attacks that inject errors to push victims into the attacker's desired error state and in attacks that exploit the different behavior of the error-passive state (\Cc, \Ie, \Ij, \Ac, and \Ad). 4) it leaves certain cases of frame non-conformity outside its covered error conditions, allowing attackers to transmit malformed frames without provoking a uniform standard response (\Ig). Paradoxically, some of these properties are used for defense. Specifically, without \textit{frame destruction} (\DIe) as an impact of an active error, \textit{impersonation and replay} would be exposed as gaps (Tbl. \ref{tbl:bigtable}). Similarly, thanks to \textit{error-states and error-types}, fast \textit{layer-II node-suspension} (\DAd) is an effective \textit{bus-access denial} defense, without which it would be exposed as a \textit{by-the-ruler} gap.



\input{Tables/RootCause}


\shortsectionEmph{$\mathcal{R}$5: Physical Signaling (I).}  Several charecterstics of CAN physical signaling are exploitable by attackers ranging from \textit{by-the-rulers} to \textit{down-to-earthers}: 1) despite differential voltage and twisted wires, CAN is still vulnerable to emitting EMI (\Ce) due to lack of shielding and relatively high switching speed. 2) minor electrical differences among nodes using the bus as a shared electrical medium allows \textit{hardware and topology profiling} (\Cd) and \textit{physical fingerprint distortion} (\Ij). 3) using \textit{push-pull signaling} to drive dominant bits and high-impedance for recessive bits, enable attacks that rely on bit-flips and pulses (\Cc, \Ie, \IF, \Ii, \Ac, \Ad, \Ag). 4) dynamic edge synchronization allows \textit{bit-bangers} manipulating edges to disrupt synchronization among nodes (\Af). These features are \textit{inherent} but \textit{not unique}. As will be shown in Sec. \ref{sec:investigat}, many other protocols' physical signaling share them.\looseness-1



\shortsectionEmph{$\mathcal{R}$6: CAN Bit Sampling (IU).} To translate voltage levels into bit values, CAN nodes sense the voltage at specific times called \textit{sample points} whose timing is \textit{configurable}, not the same across nodes, and happens \textit{once per bit}. Exploiting discrepancies between node sample points allows attackers to insert signal transitions between them allows for sending messages that have differing interpretations (\Ih). This is \textit{inherent} and \textit{unique} as other protocols do not combine these sample-point qualities, particularly configurability.\looseness-1    




\shortsectionEmph{$\mathcal{R}$7: Vulnerable Higher-Layer Protocols and Implementation.} Higher-layer protocols and their implementations can introduce exploitable logic and software weaknesses. Vulnerable features, such as request-response exchanges, session mechanisms, and functionality-disabling commands can be abused by by-the-rulers to launch \textit{ECU functionality disabling} (\Aa), and \textit{sybil exhaustion} (\Ab) attacks. At the implementation level, software flaws such as memory-corruption bugs and weaknesses in diagnostic-security handling can be exploited for privileged information exposure and internal-ECU-manipulation attacks (\Cb, \Ib, and \Ic). This is \textit{not inherent} as the CAN standard does not specify or mandate any implementations or higher-layer protocols. It is also \textit{not unique}, as these protocols and implementations could be used with other communication media.





\shortsectionEmph{$\mathcal{R}$8: Layer-II Rule Violation.} The ability of \textit{bit-bangers} to bypass CAN's controller layer rules, placing and reading arbitrary signals on the bus, underlies all \textit{bit-banger} attacks (\IF-\Ii, and \Af-\Ag). It also underlies the \textit{bit-banger} variants of several attacks that could be launched using different methods for \textit{by-the-rulers} (\Cc, \Ie, \Ij, and \Ac-\Ae). By definition, this is \textit{not inherent} to CAN as it does not stem from its rules but from the violation of them, jeopardizing other parts of the standard. It is either an ECU design problem allowing for the bypass or manipulation of the CAN controller, or an access problem, allowing physical installation of non-CAN-conforming devices (Sec. \ref{subsubsec:Dattacker}). 



\shortsectionEmph{$\mathcal{R}$9: Layer-I Rule Bypass.} \textit{Down-to-earthers}' ability to bypass CAN’s physical-layer rules through privileged physical access and specialized equipment allows them to inject or collect physical signal measurements in ways CAN was not designed for. This, along with other root causes, underlies \textit{down-to-earther} attacks such as \textit{hardware and topology intelligence} (\Cd) and \textit{capturing electromagnetic emissions} (\Ce).


\subsection{Defense Gap Root Causes ($\mathcal{DR}$s)}\label{subsec:defense_rc}


\shortsectionEmph{$\mathcal{DR}$1: Cryptography Challenges (I).} Cryptography on CAN faces three challenges. First, \textit{performance}: commercial ECUs often have limited processing budgets, making cryptographic operations costly if applied to all outgoing and incoming messages. Second, \textit{message length}: CAN’s 64-bit maximum payload complicates carrying authentication data. For example, AUTOSAR suggests using 24 authentication bits. If a message carries more than 40 bits of data, little room remains for authentication. If it carries less, authentication data can significantly increase message length and busload. The same length constraint also makes conventional block-cipher encryption cumbersome, since block sizes often exceed the message size. Third, and more fundamentally, CAN faces an \textit{inherent} but not \textit{unique} \textit{shared-media key-management dilemma}. On a broadcast medium, group keys preserve efficiency and can protect against \textit{external attackers} (i.e., an ECU without the group key). However, communication is exposed to \textit{internal attackers} (i.e., a compromised ECU that holds the group key can decrypt all traffic and impersonate any group member). Asymmetric cryptography for general communication is often impractical on resource-constrained ECUs. Pairwise keys between each sender-receiver pair reduce that exposure, but do not fit the broadcast nature of CAN and may impose substantial communication overhead, since the same message may need to be sent multiple times under different keys. While workarounds have been proposed to address \textit{performance} and \textit{message length}, little has been proposed to solve this shared-media key-management dilemma, the main culprit behind the \textit{internal attacker} issue. Fixing the first two challenges mainly improves bus or ECU efficiency, whereas fixing the last fills the \textit{communication surveillance gap} (\Ca) and provides effective defenses against \textit{bypassing diagnostic authentication} (\Ic)~and \textit{impersonation and replay} (\Id). App. \ref{A:CrIssue} discusses the \textit{shared-media key-management dilemma} and some proposed workarounds in more detail.



\shortsectionEmph{$\mathcal{DR}$2: Costly Attacker Signal Filtering and Disabling (I).} On a broadcast bus, availability attacks aimed at disrupting communication (\Ac-\Af) can only be stopped by filtering the attacker's signals or disabling the attacker node, so other nodes have room to communicate. Similarly, attacks that rely on injecting malicious signals into specific parts of a message (\Cc, \IF) can only be prevented this way. The lack of a cheap and effective attacker filtering and disabling approach is the fundamental reason for the \textit{bit-banger} gaps of \Cc, \IF, \Ac-\Af, where defenses cannot simultaneously achieve prevention for all attacker models and good infrastructure compatibility: layer-II node suspension (\DAd) is a cheap form of node disabling but works only against \textit{by-the-ruler}s, leaving the bus vulnerable to other attacker models; addressing stronger attackers by adding guardians (\DIk) or fragmentation mechanisms (\DAe) requires expensive infrastructure changes. Combined with the existing detection approaches, addressing this challenge closes these gaps and provides an effective defense against integrity and availability attacks against the transwire layer (\Ij, \Ag).





\shortsectionEmph{$\mathcal{DR}$3: Difficult Environment Understanding.} Determining whether a message is malicious may be infeasible without understanding the bigger system (\DIb). For example, an attacker compromising the brake ECU and sending fake brake values, without impersonation, the only way to detect this fabrication is to understand how these values relate to the bigger system (e.g., the vehicle), which may involve physical modeling. This $\mathcal{DR}$ is not inherent to CAN but to its environment (e.g., vehicle) and could be solved for open or less complex environments (e.g., an elevator). It is also \textit{not unique}, as it will be present in other communication media operating within the same environment. Addressing this root-cause closes the \textit{fake data fabrication} gap (\Ia) and effectively detects tampering with in-flight frames (\Ie, and \Ii), which could be turned into prevention to provide an effective defense when combined with \textit{frame destruction} (\DIe).\looseness-1  


\begin{tcolorbox}[
  colback=gray!15,
  colframe=gray!60,
  fonttitle=\bfseries,
    boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]
\shortsectionBf{Takeaways on CAN's Insecurity Root Causes} 

\begin{itemize}[leftmargin=*]

\item Most root causes are not unique to CAN. Specifically, 6/9 attack root causes and 2/3 defense-gap root causes are inherent, yet only vulnerable \textit{error handling} ($\mathcal{R}$4) and \textit{bit-sampling} ($\mathcal{R}$6) are unique to the CAN family. This means many weaknesses attributed to CAN actually come from broader shared-media design properties.



\item A high number of inherent root causes does not mean a high number of inherent attacks. An attack usually depends on multiple root causes, and if any required root cause is not inherent, the attack is not inherent. Thus, although 6/9 attack root causes are inherent, only 9/22 attacks are inherent. The unique subset is smaller: only 8/22 attacks are unique, and only 5/22 are both inherent and unique.

\item Among shared-media systems, CAN appears more securable than often assumed. None of the root causes behind the absence of effective defense is unique to CAN. They instead stem from shared single-channel media, vehicular constraints, ECU implementation weaknesses, and access-control assumptions that could recur in any shared-media system under similar conditions. The gap statistics reinforce this interpretation: only 1 gap is inherent, and it is inherent to shared-media communication, not CAN itself. The 4 unique gaps are unique only because their underlying attacks rely on CAN-unique root causes, not because the absence of effective defense is unique. Most importantly, no gap is both inherent and unique.



\end{itemize}

\end{tcolorbox}


\begin{figure}[t]
  \centering
  \includegraphics{figs/root_cause_distribution.pdf}
  \caption{Number of inherent or unique attacks and gaps. \kha{these numbers are wrong. what are the 4 inhent gaps? also i think more unique non inherent}}
  \label{fig:rc_distribution}
\end{figure}

% \section{Root Causes and Transferability of CAN Security Problems}
% \label{sec:Analysis}
% \label{sec:ResearchGaps}

% CAN security problems are often treated as problems of CAN itself. However, this does not distinguish between weaknesses that stem from the CAN standards, weaknesses that are unique to CAN, and weaknesses that instead arise from broader properties of shared in-vehicle buses, ECU implementations, attacker access, or the cyber-physical environment. This distinction is necessary because replacing CAN only eliminates a security problem if the problem is actually CAN-specific.

% We therefore analyze CAN insecurity in two steps. First, we identify the root causes underlying CAN attacks and defense gaps, and determine whether each root cause is \textit{inherent}, \textit{unique}, or both. A root cause is \textit{inherent} if it stems from the CAN specification rather than from accidental implementation or deployment choices. A root cause is \textit{unique} if it is specific to the CAN family of standards. Second, we investigate whether these root causes are also present in emerging in-vehicle bus (IVB) technologies, and use this to assess whether CAN attacks and defense gaps are likely to transfer.

% Tbl. \ref{tbl:root_cause} summarizes both parts of the analysis. It reports the CAN root causes, their inherency and uniqueness, the attacks and gaps they underlie, and their likely presence in CAN FD, CAN XL, and 10BASE-T1S. Detailed attack-by-attack root-cause mappings and IVB standard-review derivations are moved to App. \ref{A:root_cause_details}.

% \subsection{CAN Root Causes}
% \label{subsec:root_cause}
% \label{subsec:attack_rc}

% Our analysis identifies 9 attack root causes ($\mathcal{R}$) and 3 defense-gap root causes ($\mathcal{DR}$). In Tbl. \ref{tbl:root_cause}, a \checkmark indicates that a root cause is indispensable to an attack or gap. For attacks, an $\uparrow$ indicates that addressing the root cause provides an effective defense. \textit{By-the-ruler} gaps are highlighted in \textit{red}, and \textit{bit-banger} gaps are highlighted in blue.

% \shortsectionEmph{$\mathcal{R}$1: Attacker Access to Network (I).} This is the baseline assumption that the attacker has access to the network, either physically or remotely. It is inherent to all considered attacker models and required by all attacks. It is not unique, since comparable analyses of other communication systems also assume attacker access.

% \shortsectionEmph{$\mathcal{R}$2: Shared Media Properties (I).} CAN is a single-channel shared broadcast medium. This gives rise to two general properties: \textit{broadcast promiscuity}, where a connected node can observe bus-wide activity and reach the whole bus, and \textit{mutual exclusion}, where one transmitter can prevent others from transmitting. These properties are inherent to CAN’s bus design but not unique to CAN.

% \shortsectionEmph{$\mathcal{R}$3: Exploitable Priority System (I).} CAN uses a priority system in which dominant voltage overrides recessive voltage and lower CAN IDs receive higher priority. Since CAN IDs are settable by transmitters, this priority system can be exploited by by-the-rulers. This root cause is inherent to CAN but not unique, since shared media generally require some form of priority or media-access control.

% \shortsectionEmph{$\mathcal{R}$4: Error Handling Properties (IU).} CAN error handling includes sender/receiver validity discrepancies, error types and impacts, behaviorally distinct error states, and cases of malformed frames without a uniform standard response. These properties are inherent and unique to the CAN family.

% \shortsectionEmph{$\mathcal{R}$5: Physical Signaling (I).} CAN physical signaling includes exploitable electrical and timing properties, including electromagnetic emissions, node-specific signal characteristics, dominant/recessive signaling behavior, and dynamic edge synchronization. These properties are inherent to CAN’s physical layer but not unique to CAN.

% \shortsectionEmph{$\mathcal{R}$6: CAN Bit Sampling (IU).} CAN nodes sample the bus once per bit at configurable sample points. This allows discrepancies among receivers’ interpretations of the same signal. This root cause is inherent and unique to the CAN family.

% \shortsectionEmph{$\mathcal{R}$7: Vulnerable Higher-Layer Protocols and Implementation.} Higher-layer protocols and ECU implementations can introduce exploitable logic or software weaknesses. This root cause is not inherent to CAN, because CAN does not mandate those protocols or implementations. It is also not unique, because the same weaknesses can appear above other IVBs.

% \shortsectionEmph{$\mathcal{R}$8: Layer-II Rule Violation.} This root cause captures the ability of bit-bangers to bypass CAN controller-layer rules and place arbitrary non-conforming signals on the bus. It is not inherent to CAN, because it violates rather than follows the standard.

% \shortsectionEmph{$\mathcal{R}$9: Layer-I Rule Bypass.} This root cause captures down-to-earthers' ability to bypass normal physical-layer operation through privileged physical access and specialized equipment. It is not inherent to CAN and not unique to CAN.

% \shortsectionEmph{$\mathcal{DR}$1: Cryptography Challenges (I).} CAN cryptography faces performance limits, message-length limits, and a shared-media key-management dilemma. The first two are engineering constraints, while the last is more fundamental: group keys fit broadcast communication but expose traffic to internal attackers, whereas pairwise keys reduce exposure but conflict with efficient broadcast communication. This root cause is inherent to shared-media communication but not unique to CAN.

% \shortsectionEmph{$\mathcal{DR}$2: Costly Attacker Signal Filtering and Disabling (I).} On a shared bus, some attacks can only be prevented by filtering the attacker’s signals or disabling the attacker node. Cheap approaches are limited, while stronger approaches often require infrastructure changes. This root cause is inherent to shared-media buses but not unique to CAN.

% \shortsectionEmph{$\mathcal{DR}$3: Difficult Environment Understanding.} Some malicious messages cannot be identified from bus traffic alone and require understanding the larger cyber-physical environment. This root cause is not inherent to CAN and not unique to CAN, since it stems from the surrounding system rather than the bus standard.

% \input{Tables/RootCause}

% The analysis shows that most root causes are not unique to CAN. Specifically, 6/9 attack root causes and 2/3 defense-gap root causes are inherent, yet only vulnerable \textit{error handling} ($\mathcal{R}$4) and \textit{bit-sampling} ($\mathcal{R}$6) are unique to the CAN family. This means that many weaknesses attributed to CAN actually come from broader shared-media design properties.

% A high number of inherent root causes also does not mean a high number of inherent attacks. An attack usually depends on multiple root causes, and if any required root cause is not inherent, the attack is not inherent. Thus, although 6/9 attack root causes are inherent, only 9/22 attacks are inherent. The unique subset is smaller: only 8/22 attacks are unique, and only 5/22 are both inherent and unique.

% Among shared-media systems, CAN therefore appears more securable than often assumed. None of the root causes behind the absence of effective defense is unique to CAN. They instead stem from shared single-channel media, vehicular constraints, ECU implementation weaknesses, and access-control assumptions that could recur in any shared-media system under similar conditions. The gap statistics reinforce this interpretation: only 1 gap is inherent, and it is inherent to shared-media communication, not CAN itself. The 4 unique gaps are unique only because their underlying attacks rely on CAN-unique root causes, not because the absence of effective defense is unique. Most importantly, no gap is both inherent and unique.

% \begin{tcolorbox}[
%   colback=gray!15,
%   colframe=gray!60,
%   fonttitle=\bfseries,
%   boxsep=0pt,
%   left=2pt,
%   right=2pt,
%   top=2pt,
%   bottom=2pt,
%   before skip=4pt,
%   after skip=4pt,
% ]
% \shortsectionBf{Takeaway on CAN Root Causes.}
% Many CAN security problems are rooted in shared-media and vehicular-system properties, not in CAN-unique mechanisms.
% \end{tcolorbox}

% \begin{figure}[t]
%   \centering
%   \includegraphics{figs/root_cause_distribution.pdf}
%   \caption{Number of inherent or unique attacks and gaps.}
%   \label{fig:rc_distribution}
% \end{figure}


% \subsection{Transferability to Emerging IVBs}
% \label{sec:investigat}

% The previous subsection shows that most root causes of CAN insecurity are not unique to CAN, and that many are broadly inherent to single-channel shared communication media. This naturally raises the question of whether classic CAN security problems transfer to newer IVB technologies, and whether those technologies eliminate them.

% We investigate this question through a targeted standard review centered on the root causes identified above. The goal is a focused transferability analysis, not a broad security review of each IVB. For each IVB, we assess whether the CAN root causes are present in the standard, then extrapolate whether the corresponding CAN attacks and gaps are likely to carry over. The premise is that if an IVB inherits the root-cause patterns of an attack or gap, then the attack or gap is likely to transfer. These findings are only indicative, as confirmation of attack or gap presence in each IVB requires further rigorous research.

% Although point-to-point and switched communication technologies are appearing in vehicles, they require substantially more wiring. Since wiring cost and weight remain major vehicle-design constraints, buses are likely to remain important for in-vehicle communication. We therefore focus on three representative IVBs that are strong candidates to replace classic CAN: CAN FD, CAN XL, and 10BASE-T1S.

% To ensure a fair cross-IVB comparison, we focus only on weaknesses rooted in the standard. Accordingly, we adopt a by-the-ruler attacker model and exclude attacker models that depend on violating, bypassing, or otherwise stepping outside the standard rules. We also assume that vehicle higher-layer protocols running on top of CAN could run on top of any of the considered IVBs. Under these comparison rules, $\mathcal{R}1$ and $\mathcal{R}7$ are satisfied for all IVBs, while $\mathcal{R}8$ and $\mathcal{R}9$, together with the attacks that rely on them, are excluded from the comparison.

% In Tbl. \ref{tbl:root_cause}, IVB rows indicate the likely presence of each root cause: ($\CIRCLE$) means largely present, ($\LEFTcircle$) means somewhat present, and ($\Circle$) means largely absent. IVB columns indicate the likelihood of attacks or gaps under that IVB: ($\CIRCLE$) means \textit{likely}, ($\Circle$) means \textit{unlikely}, and ($-$) means more research is needed. The results should be read only as transferability findings: they identify which CAN security problems are likely to carry over, not the full vulnerability set of each IVB.

% \mysubsub{CAN FD}
% CAN FD shares all the attack and defense-gap root causes with CAN 2.0. Accordingly, all considered attacks and gaps are likely transferable.

% \begin{tcolorbox}[
%   colback=gray!15,
%   colframe=gray!60,
%   fonttitle=\bfseries,
%   boxsep=0pt,
%   left=2pt,
%   right=2pt,
%   top=2pt,
%   bottom=2pt,
%   before skip=4pt,
%   after skip=4pt,
% ]
% \shortsectionBf{CAN FD Standard Review Summary.}
% CAN FD shares all attack and defense-gap root causes with CAN 2.0, making all considered attacks and gaps likely transferable.
% \end{tcolorbox}

% \mysubsub{CAN XL}
% CAN XL has two error-handling settings. When error handling is enabled, it fully shares 9 of the 10 compared root causes and partially shares 1. All 14 attacks and 2 gaps under comparison are likely transferable, and 1 additional attack is likely exposed as a gap.

% When error handling is disabled, CAN XL fully shares 8 of the 10 compared root causes and partially shares 2. Out of the 14 compared attacks and 2 gaps, 11 attacks and all 2 gaps are likely transferable. One attack is unlikely to transfer, 2 require further research, and 1 additional attack is likely exposed as a gap.

% \begin{tcolorbox}[
%   colback=gray!15,
%   colframe=gray!60,
%   fonttitle=\bfseries,
%   boxsep=0pt,
%   left=2pt,
%   right=2pt,
%   top=2pt,
%   bottom=2pt,
%   before skip=4pt,
%   after skip=4pt,
% ]
% \shortsectionBf{CAN XL Standard Review Summary.}
% CAN XL retains most compared CAN root causes under both error-handling settings, making most considered attacks and gaps likely transferable.
% \end{tcolorbox}

% \mysubsub{10BASE-T1S}
% Of the 10 compared root causes, 10BASE-T1S fully shares 7, partially shares 1, and avoids 2. Out of the 14 compared attacks, 10 are likely transferable, 3 need further research, and 1 is unlikely to transfer. All 2 gaps are likely transferable, with 3 additional attacks likely exposed as gaps. As such, the likely decrease in the number of transferable attacks does not necessarily represent an improvement, because it is countered by a likely increase in the number of gaps.

% \begin{tcolorbox}[
%   colback=gray!15,
%   colframe=gray!60,
%   fonttitle=\bfseries,
%   boxsep=0pt,
%   left=2pt,
%   right=2pt,
%   top=2pt,
%   bottom=2pt,
%   before skip=4pt,
%   after skip=4pt,
% ]
% \shortsectionBf{10BASE-T1S Standard Review Summary.}
% 10BASE-T1S avoids some CAN root causes, but most compared attacks remain likely transferable and additional attacks are likely exposed as gaps.
% \end{tcolorbox}

% Across all considered IVBs, most root causes, attacks, and gaps are transferable. This shows that simply transitioning to these IVBs will not eliminate fundamental CAN security issues. These results concern only the CAN security problems considered in our transferability analysis; they do not claim that the listed attacks and gaps exhaust the security problems of CAN FD, CAN XL, or 10BASE-T1S.

% The broader conclusion is that many fundamental CAN security problems are better understood as IVB security problems. While it may be tempting to blame CAN for a great deal of in-vehicle communication insecurity, the analysis shows that the problems lie deeper than CAN. The bulk of CAN's security problems stem from root causes that are inherent to single-channel communication media, or to the cyber-physical environments in which CAN operates. Addressing CAN root causes is therefore not outdated: many of these root causes are likely to outlive CAN and remain present in future IVB generations.

% \begin{tcolorbox}[
%   colback=gray!15,
%   colframe=gray!60,
%   fonttitle=\bfseries,
%   boxsep=0pt,
%   left=2pt,
%   right=2pt,
%   top=2pt,
%   bottom=2pt,
%   before skip=4pt,
%   after skip=4pt,
% ]
% \shortsectionBf{IVB Investigation Takeaway.}
% Most considered CAN security problems are likely transferable to emerging IVBs; replacing CAN alone does not eliminate them.
% \end{tcolorbox}

% \begin{figure}[t]
%   \centering
%   \includegraphics{figs/bar_chart.pdf}
%   \caption{Transferability of CAN 2.0 security problems.}
%   \label{fig:ivb}
% \end{figure}

==> sec8_ComFutureRevised.tex <==


\section{Emerging IVB Root-Cause Investigation}
\label{A:investigat}






A key finding of the previous section was that most root causes of CAN insecurity are not unique to CAN, and that many are broadly inherent to single-channel shared communication media. This naturally raises the question of to what extent classic CAN security problems transfer to newer IVB technologies, and to what extent those technologies eliminate them. We investigate this question through a targeted standard review centered on the root causes identified in Sec. \ref{sec:Analysis}. The goal is therefore a focused transferability analysis, rather than a broad security review of each IVB. For each IVB, we assess whether those root causes are present in the standard, then extrapolate whether the corresponding CAN attacks and gaps are likely to carry over. The premise is that if an IVB inherits the root-cause patterns of an attack or gap, then the attack or gap is likely to transfer. Note that the findings of this investigation are only indicative, as confirmation of attack or gap presence in each IVB requires further rigorous research.

Tbl. \ref{tbl:root_cause} summarizes the findings of this investigation. \textit{By-the-ruler} defense gaps are highlighted in \textit{red}, and excluded attacks and root causes are in \textit{gray}. IVBs appear both as rows and as columns. IVB rows indicate the likely presence of each root cause: ($\CIRCLE$) means largely present, ($\LEFTcircle$) means somewhat present, and ($\Circle$) means largely absent. IVB columns indicate the likelihood attacks or gaps under that IVB: ($\CIRCLE$) means \textit{likely}, ($\Circle$) means \textit{unlikely}, and ($-$) means more research is needed.\looseness-1 
 



\shortsectionBf{IVB Selection.} Although point-to-point \cite{MIPI, ASA} and switched communication technologies \cite{AEth100, AEth1000} are appearing in vehicles, they require substantially more wiring. The wiring harness is already among the vehicle’s most costly components and its third heaviest after the engine and chassis \cite{Wiring2, Wiring}. We therefore expect wiring cost and weight to confine such technologies to essential use cases, with buses continuing to dominate in-vehicle communication. Among the many possible choices, we focus on three representative in-vehicle bus technologies that are strong candidates to replace classic CAN: CAN FD, CAN XL, and Automotive Ethernet (10BASE-T1S) \cite{Bosch2022CANXL,Schaefer2023ArtNetworking}. We select them because manufacturers are most likely to adopt successors built on already established automotive communication ecosystems, namely CAN and Ethernet.

\shortsectionBf{Investigation Methodology.} We investigate the IVBs primarily through a \textit{formal standard review}. Where standard review is insufficient to determine the presence of a root cause, we may use \textit{formal verification}, as with the optional standardized link-layer security mechanisms CANsec and MACsec. To ensure a fair cross-IVB comparison, we focus only on weaknesses rooted in the standard. Accordingly, we adopt a \textit{by-the-rules} attacker model and exclude attacker models that depend on violating, bypassing, or otherwise stepping outside the standard rules. We also assume that vehicle higher-layer protocols running on top of CAN could run on top of any of the considered IVBs. Under these comparison rules, $\mathcal{R}1$ and $\mathcal{R}7$ are satisfied for all IVBs, while $\mathcal{R}8$ and $\mathcal{R}9$, together with the attacks that rely on them, are excluded from the comparison. 










\mysubsub{CAN FD} Reviewing the standard \cite{bosch2012can,ISO1,ISO2}, CAN FD is a shared single-channel broadcast bus and thus shares the same \textit{universal shared media properties} ($\mathcal{R}$2). It uses the same priority system as CAN 2.0 and their priority is settable for \textit{by-the-rulers} ($\mathcal{R}$3). Despite slight modifications, its error-handling mechanism retains the same \textit{different definitions of frame validity}, \textit{error types and impacts}, \textit{behaviorally distinct states}, and \textit{corner cases} ($\mathcal{R}$4). It uses the same physical signaling with \textit{higher switching speeds} than CAN 2.0 and without stipulating shielding as a requirement. Similar to CAN 2.0, only dominant bits are driven by push-pull. Nodes perform \textit{dynamic edge synchronization} ($\mathcal{R}$5). Bits are sampled by reading the voltage level \textit{once at configurable sample points} ($\mathcal{R}$6). It takes no measures to allow \textit{selective attacker signal filtering} ($\mathcal{DR}$2). While its longer payload alleviates a great part of the \textit{performance and length} challenges outlined in $\mathcal{DR}$1, it is still subject to the same \textit{shared media key-management dilemma}. 

\begin{tcolorbox}[
  colback=gray!15,
  colframe=gray!60,
  fonttitle=\bfseries,
    boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]
\shortsectionBf{CAN FD Standard Review Summary:} CAN FD shares all the attack and defense gap root-causes with CAN 2.0, making all considered attacks and gaps likely transferable.

\end{tcolorbox}


\mysubsub{CAN XL}\label{subsub:CXL} Reviewing the standard \cite{CANXL, ISO1, ISO2}, CAN XL is a shared single-channel broadcast bus and thus shares the same \textit{universal shared media properties ($\mathcal{R}$2)}, enabling \textit{communication surveillance} (\Ca), and \textit{impersonation and replay} (\Id). It uses a similar priority system but conventional ID functionalities are split into a \textit{Priority ID} and an \textit{Acceptance Field}, both settable to a \textit{by-the-ruler} ($\mathcal{R}$3), making \textit{bus-access denial} (\Ae) likely. 

Error handling could be enabled or disabled by a \textit{by-the-ruler}. \textbf{When enabled}, it is similar to CAN 2.0, suggesting equivalents of all error-injection-based attacks (\Ac, \Ad, \Cc, \Ie, and \Ij) are possible. \textbf{When disabled}, considerable changes exist, including removing \textit{behaviorally distinct error states} ($\mathcal{R}$4). This likely avoids \textit{error state manipulation} (\Ad). However, this also removes \textit{node suspension} (\DAd) as a possible defense, as a \textit{by-the-ruler} can disable its own error handling, regardless of the victim's setting. Since \textit{node suspension} is an effective defense against many attacks, and the only effective defense against \textit{bus-access denial} (\Ae), it is possibly exposed as a gap for both error handling settings. Both 0s and 1s are driven using push-pull. This still makes equivalents of \textit{error injection} likely. However, the outcome of a 0-1 collision will be less predictable than CAN 2.0, where it would always be 0. Accordingly, the presence of \textit{frame hijacking} (\Ie) and \textit{network reconnaissance} (\Cc) equivalents cannot be determined and needs further research. 

Similar to CAN 2.0, it supports \textit{higher switching speeds}, does not mandate shielding ($\mathcal{R}$5), uses \textit{dynamic edge synchronization}, with bits read \textit{once at configurable sample points} ($\mathcal{R}$6). It is compatible with CANsec \cite{CANsec} and its length is significantly longer, alleviating \textit{performance and length} challenges. To assess if it addresses the \textit{internal attacker} issue ($\mathcal{DR}$1), we formally verified CANsec (details in App. \ref{inv:CANsec}). Our verification shows that as the current in-development version of CANsec stands, it provides authenticity, freshness, and confidentiality only against external attackers but not \textit{internal attackers} ($\mathcal{DR}1$) and hence does not close any open defense gaps.


\begin{tcolorbox}[
  colback=gray!15,
  colframe=gray!60,
  fonttitle=\bfseries,
    boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]
\shortsectionBf{CAN XL Standard Review Summary} 

CAN XL has two error-handling settings:
\begin{itemize}[leftmargin=*] 
\item\shortsectionBf{Enabled:} Of the 10 compared root-causes, it fully shares 9, and partially shares 1. All 14 attacks and 2 gaps under comparison are likely transferable, and 1 additional attack is likely exposed as a gap. 
\item\shortsectionBf{Disabled:} Out of the 10 root-causes under comparison, it fully shares 8, and partially shares 2. Out of the 14 compared attacks and 2 gaps, 11 attacks and all 2 gaps are likely transferable. 1 attack is unlikely to transfer, and 2 require further research to determine. 1 additional attack is likely exposed as a gap.
\end{itemize}

\end{tcolorbox}




\mysubsub{10BASE-T1S} Reviewing the standard \cite{AEth10B}, 10BASE-T1S is a shared half-duplex broadcast bus, with the same \textit{universal shared media properties} ($\mathcal{R}$2), making equivalents of \textit{communication surveillance} (\Ca), and \textit{impersonation and replay} (\Id) possible. Priority is managed by Physical Layer Collision Avoidance (PLCA). Each node's priority is determined by its local ID. Similar to CAN, it is settable for \textit{by-the-rulers} ($\mathcal{R}$3),  making \textit{bus-access denial} (\Ae) possible. 

It has different error handling rules and no error states, likely avoiding error state manipulation (\Ad) but also lacking features that could be used as effective defenses, such as frame destruction (\DIe) or node suspension (\DAd), which in turn is likely to expose \textit{impersonation and replay} (\Id) and \textit{bus access denial} (\Ae) as gaps. \textit{Network reconnaissance} (\Cc) is \textit{likely}, not using errors, but using inherent properties (e.g., node ID). Research on whether it harbors properties allowing equivalents of \textit{error injection} (\Ac), \textit{frame hijacking} (\Ie), and \textit{fingerprint distortion} (\Ij) is needed.



Similar to CAN, it uses differential signaling with \textit{dynamic edge synchronization}, does not stipulate shielding, and supports \textit{higher switching speeds} than CAN 2.0. It uses differential Manchester encoding, where both 0s and 1s are driven using push-pull. This results in the collision outcome of 0 and 1 being unpredictable, unlike CAN, where it is always 0 ($\mathcal{R}$5). Unlike CAN, receivers interpret bits by reading voltage transitions at fixed start and middle of bits, without configurable sample points ($\mathcal{R}$6). 


Like CAN, it takes no measures to facilitate \textit{selective attacker signal filtering} ($\mathcal{DR}$2). It is natively compatible with MACsec, and its maximum length is significantly longer, alleviating the \textit{performance and length} challenges. To assess if it addresses the \textit{internal attacker} issue ($\mathcal{DR}$1), we formally verified MACsec (details in App. \ref{inv:CANsec}). Our verification shows that as the 10BASE-T1S version of MACsec stands, it provides authenticity, freshness, and confidentiality only against external attackers but not \textit{internal attackers} ($\mathcal{DR}1$) and hence does not close any open defense gaps.


\begin{tcolorbox}[
  colback=gray!15,
  colframe=gray!60,
  fonttitle=\bfseries,
    boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]
\shortsectionBf{10BASE-T1S Standard Review Summary} 

Of the 10 compared root-causes, 10BASE-T1S fully shares 7, partially shares 1, and avoids 2. Out of the 14 compared attacks, 10 are likely transferable, 3 need further research, and 1 is unlikely to transfer. All 2 gaps are likely transferable with 3 additional attacks likely exposed as gaps. As such, the likely decrease in the number of transferable attacks does not necessarily represent an improvement as it is countered by a likely increase in the number of gaps.


\end{tcolorbox}

\begin{tcolorbox}[
  colback=gray!15,
  colframe=gray!60,
  fonttitle=\bfseries,
    boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]
\shortsectionBf{IVB Investigation Takeaways}

\begin{itemize}[leftmargin=*]
    
    \item Most of CAN's security problems are transferable to future IVBs. Specifically, for all of the considered IVBs, most of the root causes, attacks, and gaps, were transferable. This shows that simply transitioning into these IVBs will not eliminate fundamental CAN security issues. \kha{we need to rethink what we want to say here}
    \item you need to say somewhere that these are only the transferable things
    \item CAN fundamental security problems are in-vehicle-bus security problems. While it may be enticing to blame CAN for a great deal of in-vehicle communication security issues, our analysis shows that the problems lie deeper than CAN. As has been shown in this section and Sec. \ref{sec:Analysis}, the bulk of CAN's security problems stem from root causes that inherent to single-channel communication media, or to the cyber-physical environments in which CAN operates. (Or maybe addressing CAN root causes of insecurity is not u=outdated as these root causes of insecurity will outlive CAN and will be present in future IVB generations>)
\end{itemize}



\end{tcolorbox}

\begin{figure}[t]
  \centering
  \includegraphics{figs/bar_chart.pdf}
  \caption{Transferability of CAN 2.0 security problems.}
  \label{fig:ivb}
\end{figure}





==> test.tex <==
\section{Root Cause and Transferability Analysis}
\label{sec:Analysis}
\label{sec:ResearchGaps}
\label{sec:investigat}

In this section, we assess whether CAN security problems are fundamentally CAN-specific or likely to persist in other in-vehicle buses (IVBs). We do so through two linked investigations. The first identifies the root causes underlying CAN attacks and defense gaps, classifies each root cause as \textit{inherent}, \textit{unique}, or both, and uses this classification to infer which attacks and gaps are themselves inherent or unique to CAN. The second assesses whether the same root causes appear in alternative IVBs. The premise is that if an IVB inherits the root-cause pattern of an attack or gap, then that attack or gap is likely to transfer. We assess three representative emerging IVBs: CAN FD, CAN XL, and Automotive Ethernet (10BASE-T1S). \MR{6}To separate security problems rooted in bus protocols from those rooted in the surrounding system, we further consider a hypothetical ideal bus that provides secure logical channelization with confidentiality, integrity, and availability, and assess what root causes are present in it. Our investigation is based on standard review, supplemented by formal verification where review alone is inconclusive.



\label{subsec:root_cause}
\label{subsec:attack_rc}

Our analysis identifies 9 attack root causes ($\mathcal{R}$) and 3 defense-gap root causes ($\mathcal{DR}$). Tbl. \ref{tbl:root_cause} summarizes the two investigations detailed in App. \ref{A:Analysis} and App. \ref{A:investigat}. It reports the root causes, their relationship to attacks and gaps, their inherency and uniqueness status, their likely presence in the considered IVBs, and the resulting attack/gap transferability assessment. A \checkmark~indicates that a root cause is indispensable to the attack or gap; for attacks, an $\uparrow$ indicates that addressing the root cause provides an effective defense. IVBs appear both as rows and columns: rows report root-cause presence in each IVB, where ($\CIRCLE$) means largely present, ($\LEFTcircle$) somewhat present, and ($\Circle$) largely absent; columns report attack/gap transferability under each IVB, where ($\CIRCLE$) means likely, ($\Circle$) unlikely, and ($-$) unresolved. {By-the-rules} gaps are highlighted in {red}, {bit-banger} gaps in blue, and excluded attacks and root causes in {gray}. 

To ensure a fair cross-IVB comparison, we focus only on weaknesses rooted in the standard. Accordingly, we adopt a {by-the-rules} attacker model and exclude attacker models that depend on violating, bypassing, or otherwise stepping outside the standard rules. We also assume that vehicle higher-layer protocols running on top of CAN could run on top of any of the considered IVBs. Under these comparison rules, $\mathcal{R}1$ and $\mathcal{R}7$ are satisfied for all IVBs, while $\mathcal{R}8$ and $\mathcal{R}9$, together with the attacks that rely on them, are excluded from the comparison. 

Due to space constraints, we only report the definitions of the root causes and the outcomes of these investigations. The detailed root-cause descriptions, attack-to-root-cause mappings, the reasoning used to classify root causes as inherent or unique, the IVB-selection rationale, and the standard-review analysis are provided in App. \ref{A:Analysis} and App. \ref{A:investigat}.



\shortsectionBf{Attack Root Causes:} 
\input{Tables/RootCause}

\shortsectionEmph{$\mathcal{R}$1: Attacker Access to Network (I).} Access to the bus, whether physical or remote through a compromised ECU, is the baseline condition for all considered attacker models. It is {inherent} to the threat model rather than to a specific CAN feature, and it is assumed to be present in all IVBs under investigation.\looseness-1

\shortsectionEmph{$\mathcal{R}$2: Shared Media Properties (I).} CAN is a single-channel shared broadcast medium. This gives an attacker two broad advantages: \textit{broadcast promiscuity}, meaning that a connected node can observe bus-wide activity and reach all nodes on the bus, and \textit{mutual exclusion}, meaning that one transmitter can prevent others from using the channel. %These properties are inherent to all single-channel shared communication media, including CAN 2.0, CAN FD, CAN XL, and 10BASE-T1S. 


\shortsectionEmph{$\mathcal{R}$3: Exploitable Priority System (I).} CAN resolves bus access through a priority mechanism where dominant bits override recessive bits and lower CAN IDs receive higher priority. Because the CAN ID, and hence message priority, is settable through the higher layer, it is exploitable by {by-the-rules} attackers.\looseness-1 %It is \textit{inherent} to CAN, and was found present in CAN FD, CAN XL, and 10BASE-T1S.

\shortsectionEmph{$\mathcal{R}$4: Error Handling Properties (IU).} CAN error handling contains several exploitable properties: different validity criteria for senders and receivers, specific error types, error behavior that halts transmission and raises error frames, behaviorally distinct error states, and corner cases where malformed frames do not provoke a uniform standard response. These properties are both {inherent} and {unique} only to the CAN family of standards, including CAN 2.0, FD. In CAN XL, it is fully present in one of its operating modes and partially present in the other.\looseness-1

\shortsectionEmph{$\mathcal{R}$5: Physical Signaling (I).} CAN’s physical signaling exposes several attack surfaces, including non-shielded twisted wire differential voltage signaling, node-specific electrical characteristics, push-pull signaling, and dynamic edge synchronization. %These properties are \textit{inherent} to CAN’s physical-layer design but \textit{not unique}, and were found in all IVBs under investigation.

\shortsectionEmph{$\mathcal{R}$6: CAN Bit Sampling (IU).} CAN nodes sample the bus once per bit at configurable sample points. Discrepancies between sample points across nodes can therefore be exploited for inconsistent interpretations of the same signal. %This combination of once-per-bit sampling and configurable sample points is both \textit{inherent} and \textit{unique} to the CAN family: CAN 2.0, CAN FD, and CAN XL, and was not found in 10BASE-T1S.

\shortsectionEmph{$\mathcal{R}$7: Vulnerable Higher-Layer Protocols and Implementations.} Higher-layer protocols and ECU implementations can introduce exploitable logic and software weaknesses. %These weaknesses are \textit{not inherent} to CAN. They are also \textit{not unique}, and could appear over any of the other IVBs.

\shortsectionEmph{$\mathcal{R}$8: Layer-II Rule Violation.} The ability of attackers to bypass CAN controller-layer rules and place arbitrary non-conforming signals on the bus. It is excluded from the IVB comparison. 

% This is \textit{not inherent} to CAN and it is excluded from the IVB comparison. 

\shortsectionEmph{$\mathcal{R}$9: Layer-I Rule Bypass.} The ability of attackers to bypass CAN physical-layer rules (excluded from the IVB comparison).

% This is \textit{not inherent} to CAN and


\shortsectionBf{Defense Gap Root Causes:} 

\shortsectionEmph{$\mathcal{DR}$1: Cryptography Challenges (I).} Cryptography on CAN faces three challenges: the limited processing budget of commercial ECUs, the maximum length of CAN messages, and key-management problems due to its broadcast nature. Since 10BASE-T1S and CAN XL have security add-ons, MACsec and CANsec, we conducted an additional investigation of these two protocols. We summarize the main details of this study later in this section, and explain it at length in App. \ref{inv:CANsec}

% These problems are \textit{inherent} and fully present in CAN 2.0 but are partially present in all single-channel shared-media, including CAN FD, CAN XL, and 10BASE-T1S.

\shortsectionEmph{$\mathcal{DR}$2: Costly Attacker Signal Filtering and Disabling (I).} On a shared bus, preventing some attacks requires filtering attacker signals or disabling their node so legitimate nodes can communicate, usually requiring costly infrastructure changes. %This challenge is \textit{inherent} to all single-channel shared-media, including CAN 2.0, CAN FD, CAN XL, and 10BASE-T1S.

\shortsectionEmph{$\mathcal{DR}$3: Difficult Environment Understanding.} Some malicious messages cannot be identified as malicious based on authentication alone and require understanding the larger cyber-physical environment and the message context within it to determine whether it carries false data. %This is \textit{not inherent} to CAN but to the environment within which it operates. All IVBs under comparison will have it if they operate in the same environment. 

\shortsectionBf{\MR{4}CANsec and MACsec Investigation:} 



\shortsectionEmph{Purpose and Results.} MACsec is a standardized link-layer security protocol for Ethernet, while CANsec is an \textit{in-development} link-layer security protocol for CAN XL modeled after MACsec. As a supplementary check of $\mathcal{DR}$1, we examine whether automotive MACsec and CANsec close the internal-attacker gap. In their automotive configurations, both organize nodes into Connectivity Associations (CAs) whose members share a long-term symmetric Connectivity Association Key (CAK) to authenticate then establish short-term Secure Association Keys (SAK) to protect communication. A shared CAK alone does not determine their insider protection boundary because both protocols employ additional key-agreement and key-establishment mechanisms. These mechanisms could, in principle, introduce per-sender or pairwise keys, node-specific derivation, compromised-member exclusion and rekeying, or other protections. We therefore model the actual automotive/current configurations and verify them against three properties (described below) rather than infer their protection from the shared CAK alone.


Our analysis finds that, despite their key-management and key-establishment machinery, none of the modeled configurations introduces key or privilege separation among members of the same CA or otherwise mechanisms that may protect against the internal attacker. The verified properties hold against the external attacker but not the internal attacker, leaving $\mathcal{DR}$1 open. We additionally test whether idealized revocation closes the gap to motivate future research into practical mechanisms that provide it. The protocol details, models, results, and the revocation experiment are detailed further in App.~\ref{inv:CANsec}.


\shortsectionEmph{Model and Properties.} We use ProVerif~\cite{blanchet2016modeling} to model the protocols assuming a by-the-rules Dolev--Yao attacker in two forms: an external attacker outside the CA and an internal attacker controlling a CA member and possessing its keys. We verify the following properties against both attackers:
$\mathcal{P}_{a}$: An attacker cannot cause an honest CA member to accept spoofed CA messages or SAK distribution as originating from another honest member.
$\mathcal{P}_{f}$: An attacker cannot cause an honest CA member to accept replayed CA messages or SAK distribution as fresh.
$\mathcal{P}_{c}$: An attacker cannot learn protected CA communication exchanged between other members.




\shortsectionEmph{Assumptions.} For MACsec, we model the configuration specified by relevant automotive MKA specifications and AUTOSAR~\cite{automotive_mka,autosarmka}, which assumes a pre-shared CAK with a fixed key server. CANsec is in early development with two current proposals. Both use a pre-shared CAK.


\shortsectionEmph{Scope.} These results apply only to the configurations examined. MACsec supports additional authentication and key-management mechanisms outside the relevant automotive profiles, while CANsec and CKA remain under development.





\shortsectionBf{Observations and Takeaways:} 



\shortsectionEmph{On CAN 2.0 and Root Causes.} 
Most root causes are not unique to CAN. Specifically, only vulnerable {error handling} ($\mathcal{R}$4) and {bit-sampling} ($\mathcal{R}$6) are unique to the CAN family. Interestingly, no defense gap root cause is unique to CAN. 



\begin{tcolorbox}[
 colback=blue!5,
  colframe=black!40,
  fonttitle=\bfseries,
  boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]

CAN fundamental security problems stem from shared single-channel media properties, vehicular constraints, and ECU implementation weaknesses that could recur in any shared-media system under similar conditions.

\end{tcolorbox}

\begin{figure}[t]
  \centering
  \includegraphics{figs/bar_chart.pdf}
  \caption{Transferability of CAN 2.0 security problems to emerging IVBs.}
  \label{fig:ivb}
\end{figure}


\shortsectionEmph{On CAN 2.0 and Attacks and Gaps.} An attack or a gap usually depends on multiple root causes. If any required root cause is not inherent, the attack is not inherent. Conversely, if any of the root causes underlying an attack or a gap is unique, it is unique. Thus, although 6/9 attack root causes are inherent, only 9/22 attacks are inherent, 8/22 attacks are unique, and only 5/22 are both inherent and unique. Relative to gaps, only one is inherent, and it is inherent to shared-media communication, not CAN. The 4 unique gaps are unique only because their underlying attacks rely on CAN-unique root causes, not because the absence of effective defense is unique. Most importantly, no gap is both inherent and unique.



\shortsectionEmph{On IVBs and Root Causes.} Fig. \ref{fig:ivb} summarizes the results of the transferability analysis. As shown, \textbf{CAN FD} shares all compared CAN root causes, making all considered attacks and gaps likely transferable. \textbf{CAN XL} has two error-handling settings. When enabled, it fully shares 9 root causes, and partially shares 1. As such, 14 attacks and 2 gaps under comparison are likely transferable, and 1 additional attack is likely exposed as a gap. When disabled, it fully shares 8 root causes, and partially shares 2. Consequently, 11 attacks and both 2 gaps are likely transferable. 1 attack is unlikely to transfer, and 2 require further research to determine. 1 additional attack is likely exposed as a gap. \textbf{10BASE-T1S} fully shares 7 root causes, partially shares 1, and avoids 2. As such, 10 attacks are likely transferable, 3 need further research, and 1 is unlikely to transfer. Both 2 gaps are likely transferable with 3 additional attacks likely exposed as gaps. \MR{6}Finally, an \textbf{ideal secure bus} fully shares 3 root causes, partially shares 1, and avoids 6. 8 attacks may be avoided and 6 remain, where 1 remains as a gap. This shows that certain problems are rooted in the system surrounding the bus and will reproduce no matter how perfect the bus is unless a new approach to vehicle security is taken, where the entire system is considered as one whole. 

\begin{figure}[t]
  \centering
  \includegraphics{figs/bar_chart.pdf}
  \caption{Transferability of CAN 2.0 security problems to emerging IVBs.}
  \label{fig:ivb}
\end{figure}



\shortsectionEmph{\MR{7}Limitation.} The findings of the transferability analysis were only indicative. The attacks identified as likely transferable were not validated on the respective buses. Such validation could be performed by formally analyzing parts of each bus protocol to determine attack viability, or empirically by setting up a testbed. Of the 14 compared attacks, 5 relied on higher-layer protocols. These attacks would need to be evaluated not only on the respective buses, but with the higher-layer protocols also set up on the ECUs. For CAN variations (CAN FD and CAN XL), most techniques used in CAN 2.0 could be directly utilized. However, for 10BASE-T1S, some techniques would need to be adapted to the specifics of the protocol. For example, instead of achieving bus access denial by faking a high-priority CAN ID, an attacker may need to fake the node ID. Across all buses, attack success could then be measured individually for each attack using the same or adapted metrics the attack authors used (e.g., swiftness and suppression rates for error-state manipulation/bus-off attacks, message loss and delay for bus-access denial attacks, etc.).
 \begin{tcolorbox}[
 colback=blue!5,
  colframe=black!40,
  fonttitle=\bfseries,
  boxsep=0pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt,
  before skip=4pt,
  after skip=4pt,
]
\begin{itemize}[leftmargin=*]


\item Emerging IVBs do not solve CAN's fundamental security problems. Most of CAN security problems likely transfer.
\item CAN is more securable than perceived. Each examined IVB inherits at least as many transferable attacks with defense gaps as CAN, before accounting for IVB-specific risks.\looseness-1
\item Certain CAN security problems can only be solved by securing the system surrounding the bus.
\end{itemize}
\end{tcolorbox}

 
